Editable Concept Bottleneck Models

Concept Bottleneck Models (CBMs) have garnered much attention for their ability to elucidate the prediction process through a humanunderstandable concept layer. However, most previous studies focused on cases where the data, including concepts, are clean. In many scenarios, we often need to remove/insert some training data or new concepts from trained CBMs for reasons such as privacy concerns, data mislabelling, spurious concepts, and concept annotation errors. Thus, deriving efficient editable CBMs without retraining from scratch remains a challenge, particularly in large-scale applications. To address these challenges, we propose Editable Concept Bottleneck Models (ECBMs). Specifically, ECBMs support three different levels of data removal: concept-label-level, concept-level, and data-level. ECBMs enjoy mathematically rigorous closed-form approximations derived from influence functions that obviate the need for retraining. Experimental results demonstrate the efficiency and adaptability of our ECBMs, affirming their practical value in CBMs.

==> ICLR/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says L2L^2 is for function spaces and ℓ2\ell^2 is for vectors
% But then they seem to use L2L^2 for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> ICML_section/accelerate_for_data_level.tex <==
It is worth noting that in theorem \ref{thm:data-level:f}, $H_{\bar{f}^*_{-z_G}}$ serves as an estimate for $H_{\Tilde{f}_{-z_G}}$ which is defined by
\begin{equation*}
    H_{\Tilde{f}_{-z_G}} = \nabla_{\Tilde{f}}\sum_{i\in[n]-G}L_{Y_i}\left(\Tilde{f}_{-z_G}, \hat{g}\right).
\end{equation*}
However, the computation of  $H_{\bar{f}^*_{-z_G}}$ is relatively complex. If the EK-FAC method is further applied to accelerate the process based on this approximation, it will introduce additional errors. Therefore, we can employ a more computationally efficient method with tolerable error to estimate $H_{\Tilde{f}_{-z_G}}$.
% It is worth noting that in theorem, the computation of Hˉf∗−zGH_{\bar{f}^*_{-z_G}} is relatively complex, and the role of Hˉf∗−zGH_{\bar{f}^*_{-z_G}} here is to serve as an estimate of H\Tildef−zGH_{\Tilde{f}_{-z_G}} which is defined by
% \begin{equation*}
%     \nabla_{\Tilde{f}}\sum_{i\in[n]-G}L_{Y_i}\left(\Tilde{f}_{-z_G}, \hat{g}\right).
% \end{equation*}
% If the EK-FAC method is further applied to accelerate the process based on this approximation, it will introduce additional errors. Therefore, considering the high error tolerance when calculating Hˉf∗−zGH_{\bar{f}^*_{-z_G}}, we can employ numerical methods to provide two effective estimates of H\Tildef−zGH_{\Tilde{f}_{-z_G}}.
\begin{theorem}
We can estimate $H_{\Tilde{f}_{-z_G}}$ by the following two ways:
    \begin{align*}
        &H_{\Tilde{f}_{-z_G}} \approx \frac{\|\nabla_{\hat{f}} L_{Y_G}  \| }{\| H_{\hat{f}} \cdot \nabla_{\hat{f}} L_{Y_G} \|} \cdot \left(I - 2 \cdot \frac{C\cdot \nabla_{\hat{f}} L_{Y_G} \cdot {\nabla_{\hat{f}} L_{Y_G}}^{\mathrm{T}} \cdot C }{{\nabla_{\hat{f}} L_{Y_G}}^{\mathrm{T}} \cdot C^2 {\nabla_{\hat{f}} L_{Y_G}}} \right)\\
        &H_{\Tilde{f}_{-z_G}} \approx \nabla_{\hat{f}} L_{Y_G} \cdot {\nabla_{\hat{f}} L_{Y_G}}^{\mathrm{T}} \cdot \left( \nabla_{\hat{f}} L_{Y_G} \cdot {\nabla_{\hat{f}}  L_{Y_G}}^{\mathrm{T}} + \alpha I \right) ^{-1} \cdot H_{\hat{f}},
    \end{align*}
    where $\nabla_{\hat{f}} L_{Y_G}\triangleq\nabla_{\hat{f}} \sum_{r\in G}L_{Y_r} ( \hat{f}, \hat{g})$, and $C\triangleq \frac{H_{\hat{f}}}{\|H_{\hat{f}}\nabla_{\hat{f}} L_{Y_G}\|} - \frac{I}{\|\nabla_{\hat{f}} L_{Y_G}\|}$.
\end{theorem}





\begin{breakablealgorithm}
\caption{Accelerated Data-level ECBM \label{alg:3-1}}
\begin{algorithmic}[1]
    \STATE {\bf Input:} Dataset $\mathcal{D} = \{ (x_i, y_i, c_i) \}_{i=1}^{N}$, original concept predictor $\hat{f}$, label predictor $\hat{g}$, and the to be removed data index set $G$.
    \STATE For $r\in G$, remove the $r$-th data $(x_r, y_r, c_r)$ from $\mathcal{D}$ and define the new dataset as $\mathcal{S}$.
    \STATE Compute the Hessian matrix of the loss function for $\hat{g}$:
    $$H_{\hat{g}} = \nabla^2_{\hat{g}}  \sum_{i,j}  L_{C_j}(\hat{g}^j(x_i),c_i^j).$$
    \STATE Update concept predictor $\Tilde{g}$:
    \begin{equation*}
        \Tilde{g} = \hat{g} + H^{-1}_{\hat{g}} \cdot  \sum_{r\in G}\nabla_{g} L_{C} (\hat{g}(x_r), c_r)
    \end{equation*}
    \STATE Update label predictor $\Tilde{f}$.
    Compute the Hessian matrix of the loss function to $\hat{f}$:
$$H_{\hat{f}} = \nabla^2_{\hat{f}}  \sum_{i=1}^n  L_Y(\hat{f}(\hat{g}(x_i), y_i).$$
\STATE   Compute $A$ as:
    \begin{equation*}
           A =  H^{-1}_{\hat{f}} \cdot  \sum_{i\in [n]-G} \nabla_{\hat{f}} L_{Y}\left(\hat{f}(\hat{g}(x_i)), y_i\right)
    \end{equation*}

\STATE Obtain $\bar{f}$ as 
    \begin{equation*}
        \bar{f} = \hat{f} + A
    \end{equation*}
\STATE Compute the Hessian matrix $H^{\prime}$:

Obtain $$\nabla_{\hat{f}} L_{Y_G}=\nabla_{\hat{f}} \sum_{r\in G}L_Y ( \hat{f} ( \hat{g} (x_r) ), y_r),$$ 
\begin{itemize}
    \item {\bf Method 1}:
    
    Compute $$C=\frac{H_{\hat{f}}}{\|H_{\hat{f}}\nabla_{\hat{f}} L_{Y_G}\|} - \frac{I}{\|\nabla_{\hat{f}} L_{Y_G}\|}$$
    Obtain $H^{\prime}$ as
    \begin{equation*}
        H^{\prime} = \frac{\|\nabla_{\hat{f}} L_{Y_G}  \| }{\| H_{\hat{f}} \cdot \nabla_{\hat{f}} L_{Y_G} \|} \cdot \left(I - 2 \cdot \frac{C\cdot \nabla_{\hat{f}} L_{Y_G} \cdot {\nabla_{\hat{f}} L_{Y_G}}^{\mathrm{T}} \cdot C }{{\nabla_{\hat{f}} L_{Y_G}}^{\mathrm{T}} \cdot C^2 {\nabla_{\hat{f}} L_{Y_G}}} \right)
    \end{equation*}
    \item {\bf Method 2}:

    Obtain $H^{\prime}$ as 
    \begin{equation*}
        H^{\prime} = \nabla_{\hat{f}} L_{Y_G} \cdot {\nabla_{\hat{f}} L_{Y_G}}^{\mathrm{T}} \cdot \left( \nabla_{\hat{f}} L_{Y_G} \cdot {\nabla_{\hat{f}}  L_{Y_G}}^{\mathrm{T}} + \alpha I \right) ^{-1} \cdot H_{\hat{f}}
    \end{equation*}
\end{itemize}


\STATE Compute $B$ as
    \begin{equation*}
        B = -{H^{\prime}}^{-1}\cdot \sum_{i\in [n]-G}\nabla_{\hat{f}}\left(    L_Y(\bar{f}(\Tilde{g}(x_i)), y_i) - L_Y(\bar{f}(\hat{g}(x_i)), y_i)\right)
    \end{equation*}
\STATE Update the label predictor $\Tilde{f}$ as: $\Tilde{f} =  \hat{f} + A + B.$
    \STATE {\bf Return: $\Tilde{f}$, $\Tilde{g}$}.  
\end{algorithmic}
\end{breakablealgorithm}


\begin{lemma}\label{approx:H:1}
\cite{hildebrand1987introduction} If we have an equation $A\cdot x = y$, where $x$ and $y$are known and $A$ is unknown. Then, the solution $A$ will not be unique. We can use a scaled Householder transformation to estimate $A$. If $x$ and $y$ are non-zero vectors with $\hat{x}=\frac{x}{\|x\|}$ and $\hat{y}=\frac{y}{\|y\|}$, then we can take  
\begin{equation*}
A=\left\{\begin{array}{ll}  
\frac{\|y\|}{\|x\|}\cdot\left(I-2 \frac{v v^{T}}{v^{T} v}\right) & \hat{x} \neq \hat{y} \\  
\frac{\|y\|}{\|x\|}\cdot I & \hat{x}=\hat{y}  
\end{array}\right.  
\end{equation*} 
where $v=\hat{x}-\hat{y}$.
\end{lemma}

\begin{proof}
Suppose we are given a unit vector $\hat{x}$ and we want to find a reflection that transforms $\hat{x}$ into a direction parallel to another given vector $\hat{y}$, which is not equal to $\hat{x}$, then the right reflection is through a hyperplane that bisects the angle between $\hat{x}$ and $\hat{y}$, which can be constructed by taking the hyperplane normal to $\|\hat{x} - \hat{y}\|$, that is, letting $v = \hat{x} -\hat{y}$,
\begin{align*}
\left (I - 2 \frac{v \cdot v^{\mathrm{T}}}{v^{\mathrm{T}} v} \right )\cdot \hat{x} - \hat{y} 
= & \frac{\hat{x} - \hat{y}}{\|\hat{x} - \hat{y}\|_{2}^{2}}\left(\|\hat{x} - \hat{y}\|_{2}^{2}-2(\hat{x} - \hat{y})^{t} \hat{x}\right) \\ 
= & \frac{\hat{x} - \hat{y}}{\|\hat{x} - \hat{y}\|_{2}^{2}}\left((\hat{x} - \hat{y})^{t}(\hat{x} - \hat{y})-2(\hat{x} - \hat{y})^{t} \hat{x}\right)  \\ 
= & \frac{\hat{x} - \hat{y}}{\|\hat{x} - \hat{y}\|_{2}^{2}}\left(\hat{x}^{t} \hat{x}-\hat{x}^{t} \hat{y}-\hat{y}^{t} \hat{x}+\hat{y}^{t} \hat{y} -2 \hat{x}^{t} \hat{x}+2 \hat{y}^{t} \hat{x}\right) = 0.
\end{align*}

Denote $\Tilde{A} = I - 2 \frac{v\cdot v^{\mathrm{T}}}{v^{\mathrm{T}} v}$, then we have $\Tilde{A} \hat{x} = \hat{y}$, that is $ \frac{\|y\|}{\|x\|} \cdot \Tilde{A} x = y$. If we choose $A$ to be $\frac{\|y\|}{\|x\|} \cdot \left(I - 2 \frac{v v^{\mathrm{T}}}{v^{\mathrm{T}} v}\right )$, then we have $A x = y$. 

If $x = y$, then we set $\Tilde{A} = I$, and we have $A = \frac{\|y\|}{\|x\|} \cdot I$.
\end{proof}

\begin{lemma}\label{approx:H:2}
\cite{boyd2004convex} If we frame solving equation $A\cdot x = y$ for $A$ as the following optimization problem:
\begin{equation*}
    \min_{A}\frac{1}{2}\|A\cdot x-y\|_{F}^{2}+\frac{\alpha}{2}\|A\|_{F}^{2},
\end{equation*}
where 
\begin{equation*}
    \|A\|_F=\left(\sum_{i=1}^n \sum_{j=1}^n a_{i, j}^2\right)^{\frac{1}{2}}=\operatorname{trace}\left[A^{\top} A\right]^{\frac{1}{2}}
\end{equation*} is the  Frobenius norm, and $\alpha$ is a regularization parameter. Then $A$ can be approximated by
\begin{equation*}
 A = yx^T\left(xx^T + \alpha I\right)^{-1}.
\end{equation*}
\end{lemma}

\begin{proof}
The objective function can be written as 
$$\frac{1}{2}\operatorname{tr}\left[\left(Ax - y\right)^T\left(Ax - y\right)\right] + \frac{\alpha}{2}\operatorname{tr}\left[A^TA\right].$$ 
If $A$ is perturbed in any direction $H$, the derivative of the objective function at $A$ should be zero. That is 
\begin{align*} 
0 &= \frac{d}{dA}\left(\frac{1}{2}\operatorname{tr}\left[\left(Ax -y\right)^T\left(Ax - y\right)\right] + \frac{\alpha}{2}\operatorname{tr}\left[A^TA\right]\right) \cdot H \\ 
&=\operatorname{tr}\left[\left(Hx\right)^T\left(Ax - y\right)\right]+\alpha\operatorname{tr}\left[H^TA\right] \\ 
&= \operatorname{tr}\left[H^T\left(\left(Ax - y\right)x^T + \alpha A\right)\right]. 
\end{align*}
Where $\operatorname{tr}$ is the trace of matrix defined as $\operatorname{tr}(A) = A_{1,1} + A_{2,2} + \cdots + A_{n,n}$.

Since this must hold for all perturbations $H$, we must have $$0 = \left(Ax - y\right)x^T + \alpha A.$$ 
which we may solve to find 
$A = yx^T \left( xx^T + \alpha I \right)^{-1}.$
% Using the Woodbury formula we have 
% (xxT+αI)−1=1α(I−x(αI+xTx)−1xT)\left(xx^T + \alpha I\right)^{-1} = \frac{1}{\alpha}\left( I - x\left(\alpha I + x^Tx\right)^{-1}x^T\right)
% and therefore 
%A=1αyxT−1αyxTx(αI+xTx)−1xT.A = \frac{1}{\alpha}yx^T - \frac{1}{\alpha}yx^T x\left(\alpha I + x^Tx\right)^{-1}x^T.
\end{proof}


\begin{theorem}
    Observing the complexity of computing $H_{\Tilde{f}_{-z_G}}$, we consider the method from lemma \ref{approx:H:1} and \ref{approx:H:2} to approximate the Hessian matrix avoid of iHVP problem. And $H_{\Tilde{f}}$ can be estimated by
    \begin{align*}
        &H_{\Tilde{f}_{-z_G}} \approx \frac{\|\nabla_{\hat{f}} L_{Y_G}  \| }{\| H_{\hat{f}} \cdot \nabla_{\hat{f}} L_{Y_G} \|} \cdot \left(I - 2 \cdot \frac{C\cdot \nabla_{\hat{f}} L_{Y_G} \cdot {\nabla_{\hat{f}} L_{Y_G}}^{\mathrm{T}} \cdot C }{{\nabla_{\hat{f}} L_{Y_G}}^{\mathrm{T}} \cdot C^2 {\nabla_{\hat{f}} L_{Y_G}}} \right)\\
        &H_{\Tilde{f}_{-z_G}} \approx \nabla_{\hat{f}} L_{Y_G} \cdot {\nabla_{\hat{f}} L_{Y_G}}^{\mathrm{T}} \cdot \left( \nabla_{\hat{f}} L_{Y_G} \cdot {\nabla_{\hat{f}}  L_{Y_G}}^{\mathrm{T}} + \alpha I \right) ^{-1} \cdot H_{\hat{f}},
    \end{align*}
    where $\nabla_{\hat{f}} L_{Y_G}\triangleq\nabla_{\hat{f}} \sum_{r\in G}L_Y ( \hat{f} ( \hat{g} (x_r) ), y_r)$, and $C\triangleq \frac{H_{\hat{f}}}{\|H_{\hat{f}}\nabla_{\hat{f}} L_{Y_G}\|} - \frac{I}{\|\nabla_{\hat{f}} L_{Y_G}\|}$.
\end{theorem}
\begin{proof}
The computational complexity of $H_{\Tilde{f}_{-z_G}}$ in theorem \ref{3-esti-f} is relatively high, so we try to estimate it. We rewrite the format of $\Tilde{f}_{-z_G}$ and $\hat{f}$ and define a new symbol $\hat{f}_{\epsilon}$. When $\epsilon \rightarrow 1$, $\hat{f}_{\epsilon} \rightarrow \hat{f}$, When $\epsilon \rightarrow 0$, $\hat{f}_{\epsilon}\rightarrow \Tilde{f}_{-z_G}$.
\begin{equation*}
\left \{
\begin{aligned}
 \Tilde{f}_{-z_G} = \argmin_f \sum_{i \in S}^{n} L_Y \left(  f \left(  \hat{g} (x_i) \right),y_i  \right) \quad \text{ \textcircled{1} } \\
\hat{f}_{\epsilon} = \argmin_f \sum_{i \in S}^{n} L_Y \left(  f (\hat{g}(x_i)), y_i  \right) +  \epsilon \cdot \sum_{r\in G}L_Y \left( f ( \hat{g} (x_r) ) , y_r   \right) \quad \text{ \textcircled{2} }
\end{aligned}
\right.
\end{equation*}

For the \textcircled{2} equation, we use Taylor expansion:
\begin{equation*}
    \nabla_{\hat{f}_{\epsilon}} \sum_{i \in S }^{n} L_Y \left(  \hat{f}_{\epsilon} (\hat{g}(x_i)), y_i  \right) +  \epsilon \cdot \nabla_{\hat{f}_{\epsilon}} \sum_{r\in G}L_Y \left( \hat{f}_{\epsilon} ( \hat{g} (x_r) ) , y_r   \right) = 0.
\end{equation*}

If we expand in $\Tilde{f}_{-z_G}$, then we have,
\begin{align*}
&   \nabla_{\Tilde{f}_{-z_G}} \sum_{i\in S}^{n} L_Y \left(  \Tilde{f}_{-z_G} (\hat{g}(x_i)), y_i  \right) +  \epsilon \cdot \nabla_{\Tilde{f}_{-z_G}}\sum_{r\in G} L_Y \left( \Tilde{f}_{-z_G} ( \hat{g} (x_r) ) , y_r   \right)  \\
& + \left[ \nabla^{2}_{\Tilde{f}_{-z_G}} \sum_{i\in S}^{n} L_Y \left(  \Tilde{f}_{-z_G} (\hat{g}(x_i)), y_i  \right) +  \epsilon \cdot \nabla^{2}_{\Tilde{f}_{-z_G}}\sum_{r\in G} L_Y \left( \Tilde{f}_{-z_G} ( \hat{g} (x_r) ) , y_r   \right) \right] ( \hat{f}_{\epsilon} - \Tilde{f}_{-z_G} ) = 0.
\end{align*}

We know that $\nabla_{\Tilde{f}_{-z_G}} \sum_{i\in S}^{n} L_Y \left(  \Tilde{f}_{-z_G} (\hat{g}(x_i)), y_i  \right) = 0$, and $\nabla^{2}_{\Tilde{f}_{-z_G}} \sum_{i\in S}^{n} L_Y \left(  \Tilde{f}_{-z_G} (\hat{g}(x_i)), y_i  \right)$ is the $H_{\Tilde{f}_{-z_G}}$ which we want to estimate. 

Then, we expand $\nabla_{\Tilde{f}_{-z_G}} \sum_{r\in G}L_Y \left( \Tilde{f}_{-z_G} ( \hat{g} (x_r) ) , y_r   \right)$ in the $\hat{f}_{\epsilon}$, we have,
\begin{equation*}
   H_{\Tilde{f}_{-z_G}} \cdot \left[ \hat{f}_{\epsilon} - \Tilde{f}_{-z_G}   \right] 
 = -\epsilon \cdot \nabla_{\Tilde{f}_{-z_G}}\sum_{r\in G} L_Y ( \Tilde{f}_{-z_G} ( \hat{g} (x_r) ), y_r ).
\end{equation*}

\begin{equation*}
    \Rightarrow
   H_{\Tilde{f}_{-z_G}} \cdot \frac{   \left[ \hat{f}_{\epsilon} - \Tilde{f}_{-z_G}   \right] } {\epsilon}
 = (-1) \sum_{r\in G}\cdot \left[ \nabla_{\hat{f}_{\epsilon}} L_Y ( \hat{f}_{\epsilon} ( \hat{g} (x_r) ), y_r )     + \nabla^{2}_{\hat{f}_{\epsilon}}  L_Y ( \hat{f}_{\epsilon} ( \hat{g} (x_r) ), y_r ) \cdot ( \Tilde{f}_{-z_G} - \hat{f}  )   \right].
\end{equation*}
\begin{equation*}
    \Rightarrow
   H_{\Tilde{f}_{-z_G}} \cdot \frac{   \left[ \hat{f}_{\epsilon} - \Tilde{f}_{-z_G}   \right] } {\epsilon}
 \approx (-1)\sum_{r\in G} \cdot \nabla_{\hat{f}_{\epsilon}} L_Y ( \hat{f}_{\epsilon} ( \hat{g} (x_r) ), y_r ).  
\end{equation*}

We estimate it using the value $\epsilon = 1$,
\begin{equation*}\label{approxH}
 H_{\Tilde{f}_{-z_G}} \cdot ( \hat{f} - \Tilde{f}_{-z_G} ) 
\approx (-1) \sum_{r\in G}\cdot \nabla_{\hat{f}} L_Y ( \hat{f} ( \hat{g} (x_r) ), y_r).
\end{equation*}

Substituting equation \ref{ap:approx:f_piao} into the above equation and we have
\begin{equation}\label{app:aprox:H_piao}
    H_{\Tilde{f}_{-z_G}} \cdot \left (H_{\hat{f}} \cdot \nabla_{\hat{f}} \sum_{r\in G}L_Y ( \hat{f} ( \hat{g} (x_r) ), y_r )  \right )= \nabla_{\hat{f}} \sum_{r\in G}L_Y ( \hat{f} ( \hat{g} (x_r) ), y_r ).  
\end{equation}

Estimating $H_{\Tilde{f}_{-z_G}}$ from the above equation is an ill-posed problem, and we give an estimation by directly substituting \eqref{app:aprox:H_piao} into lemma \ref{approx:H:1} and \ref{approx:H:2}:
\begin{align*}
        &H_{\Tilde{f}_{-z_G}} = \frac{\|\nabla_{\hat{f}} L_{Y_G}  \| }{\| H_{\hat{f}} \cdot \nabla_{\hat{f}} L_{Y_G} \|} \cdot \left(I - 2 \cdot \frac{C\cdot \nabla_{\hat{f}} L_{Y_G} \cdot {\nabla_{\hat{f}} L_{Y_G}}^{\mathrm{T}} \cdot C }{{\nabla_{\hat{f}} L_{Y_G}}^{\mathrm{T}} \cdot C^2 {\nabla_{\hat{f}} L_{Y_G}}} \right)\\
        &H_{\Tilde{f}_{-z_G}} = \nabla_{\hat{f}} L_{Y_G} \cdot {\nabla_{\hat{f}} L_{Y_G}}^{\mathrm{T}} \cdot \left( \nabla_{\hat{f}} L_{Y_G} \cdot {\nabla_{\hat{f}}  L_{Y_G}}^{\mathrm{T}} + \alpha I \right) ^{-1} \cdot H_{\hat{f}},
    \end{align*}
    where $\nabla_{\hat{f}} L_{Y_G}\triangleq\nabla_{\hat{f}} \sum_{r\in G}L_Y ( \hat{f} ( \hat{g} (x_r) ), y_r)$, and $C\triangleq \frac{H_{\hat{f}}}{\|H_{\hat{f}}\nabla_{\hat{f}} L_{Y_G}\|} - \frac{I}{\|\nabla_{\hat{f}} L_{Y_G}\|}$.
\end{proof}




==> ICML_section/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}
\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our main claims made in the abstract and introduction accurately reflect the paper's contributions and scope. See in Section \ref{sec:intro} and Abstract.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Section \ref{sec:limitation}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide the full set of assumptions and a complete (and correct) proof. See Section \ref{sec:further}, Section \ref{sec:appendix:b}, Section \ref{sec:appendix:c}, and Section \ref{sec:appendix:d} in the Appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Section \ref{sec:exp} and Section \ref{sec:appendix:exp}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, we will provide the code.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Section \ref{sec:exp} and Section \ref{sec:appendix:exp}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Section \ref{sec:exp} and Section \ref{sec:appendix:exp}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Section \ref{sec:exp} and Section \ref{sec:appendix:exp}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Section \ref{sec:impacts}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected. See Section \ref{sec:exp} and Section \ref{sec:appendix:exp}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}


==> ICML_section/extra_stuff.tex <==
%\section{More Related Work}
%\label{sec:app:related work}
%\paragraph{Concept Bottleneck Models.} 
%CBM \cite{koh2020concept} stands out as an innovative deep-learning approach for image classification and visual reasoning. It introduces a concept bottleneck layer into deep neural networks, enhancing model generalization and interpretability by learning specific concepts. However, CBM faces two primary challenges: its performance often lags behind that of original models lacking the concept bottleneck layer, attributed to incomplete information extraction from the original data to bottleneck features. Additionally, CBM relies on laborious dataset annotation. Researchers have explored solutions to these challenges. \cite{chauhan2023interactive} extend CBM into interactive prediction settings, introducing an interaction policy to determine which concepts to label, thereby improving final predictions. \cite{oikarinen2023label} address CBM limitations and propose a novel framework called Label-free CBM. This innovative approach enables the transformation of any neural network into an interpretable CBM without requiring labeled concept data, all while maintaining high accuracy. Post-hoc Concept Bottleneck models \cite{yuksekgonul2022post} can be applied to various neural networks without compromising model performance, preserving interpretability advantages. CBMs work on the image field also includes \cite{havasi2022addressing,kim2023probabilistic,keser2023interpretable,sawada2022concept,sheth2023auxiliary}. For the graph concept field, \cite{magister2021gcexplainer} provides a global interpretation for Graph Neural Networks (GNN). They begin by mapping graphs into a concept space through clustering and subsequently offer a human-in-the-loop evaluation. \cite{xuanyuan2023global, Barbiero2023interpretable} extends this approach by incorporating global and local explanations. For local explanations, they define a concept set, with each neuron represented as a vector with Boolean values indicating concept activation. 

%Despite many works on CBMs, we are the first to investigate the interactive influence between concepts through influence functions. Our research endeavors to bridge this gap by utilizing influence functions in CBMs, thereby deciphering the interaction of concept models and providing an adaptive solution to concept editing.

%\noindent {\bf Influence Function.} The influence function, initially a staple in robust statistics \cite{cook2000detection,cook1980characterizations}, has seen extensive adoption within machine learning since \cite{koh2017understanding} introduced it to the field. Its versatility spans various applications, including detecting mislabeled data, interpreting models, addressing model bias, and facilitating machine unlearning tasks. In the domain of machine unlearning, several studies leverage influence functions for approximate unlearning, offering closed-form updates of model parameters and tracing the impact of unlearning on recalled data samples. Notable works in this area encompass unlearning features and labels \cite{warnecke2021machine}, minimax unlearning \cite{liu2024certified}, forgetting a subset of image data for training deep neural networks \cite{golatkar2020eternal,golatkar2021mixed}, graph unlearning involving nodes, edges, and features. Recent advancements, such as the LiSSA method \cite{agarwal2017second,kwon2023datainf} and kNN-based techniques \cite{guo2021fastif}, have been proposed to enhance computational efficiency. These methods enable faster computation of the inverse Hessian in influence functions, facilitating the identification of influential examples and mislabeled data in large-scale models. Various studies have applied influence functions to interpret models across different domains, including natural language processing \cite{han2020explaining} and image classification \cite{basu2021influence}, while also addressing biases in classification models \cite{wang2019repairing}, word embeddings \cite{brunet2019understanding}, and finetuned models \cite{chen2020multi}. 

%Despite numerous studies on influence functions, we are the first to utilize them to construct the editable CBM. This offers valuable insights into removing mislabeled concepts and interpreting data influence within CBMs. Moreover, compared to traditional neural networks, CBMs are more complicated in their influence function. Because we only need to change the predicted output in the traditional influence function. While in CBMs, we should first remove the true concept, then we need to approximate the predicted concept in order to approximate the output. Bridging the gap between the true and predicted concepts poses a significant theoretical challenge in our proof.








#######  Extra stuff ######

We then introduce an important lemma across all three scenarios,
\begin{lemma}
    For the concept bottleneck model, if the bottleneck layer C\mathcal{C} utilize linear transformations of the θTc\theta^{T} c, then we have θ∗pj=0\theta^{*}_{p_j=0} = θ∗−pj\theta^{*}_{-p_j}. 
\end{lemma}

\begin{proof}
It is evident that for the dot product, θTc\theta^{T} c is irrelevant whether a dimension of cc is missing or equals zero in the linear transformation
\begin{equation*}
    \sum_{k:k \neq j} \theta[k] c[k] = \sum_k \theta[j] \mathbb{I} \{ k \notin j \} c[k].
\end{equation*}
Thus, the loss ℓ(z,θ)=ℓ(θTˆc,y;θ)\ell (z,\theta) = \ell(\theta^T \hat{c}, y; \theta) of both models is the same for every sample in the second stage. Thus, L(θ;D)L(\theta;\mathcal{D}) is also equal for both models with the same model parameters.
\end{proof}




\noindent{\bf Second Stage.} 
We first focus on the difference between ˆf\hat{f} and ˆfpr=0\hat{f}_{p_r=0}. The influence function can be defined as :
\begin{equation*}
\mathcal{I}(z) \stackrel{\text { def }}{=} \frac{d \hat{\theta}_{\epsilon, z}}{d \epsilon}|_{\epsilon=0}=-H_{\hat{\theta}}^{-1} \nabla_{\hat{\theta}} L(z, \hat{\theta}),  
\end{equation*}

We can linearly approximate the parameter change by the following equation,

\begin{equation}
\label{eq:1}
    \hat{f}_{p_r=0} = -H_{\hat{f}}^{-1} \cdot  \left( \nabla_{\hat{f}} \sum_{i=1}^n \ell \left( \hat{f}\left(\hat{g}\left(x_{i}\right), y_{i}\right)\right)-\nabla_{\hat{f}} \sum_{i=1}^n\ell\left(\hat{f}\left(\hat{g}_{-p_r}^{*}\left(x_{i}\right), y_{i}\right)\right)\right).
\end{equation}

Because $\hat{f}$ is the minimizer of the label loss of the original dataset, the first term in the above equation equals zero.

\noindent{\bf First Stage.}
Now, we come to the problem of approximating ˆg∗−pr∈T0={wfinal=0}⊆T\hat{g}^{*}_{-p_r} \in T_0 = \{ w_{\text{final}} = 0 \}  \subseteq T, where wfinalw_{\text{final}} is the parameter of the final layer of neural network. And ˆg∈T\hat{g} \in T. We use ˆgϵ\hat{g}_{\epsilon} to approximate ˆg∗−pr\hat{g}^{*}_{-p_r}. Similar to the original idea of defining the influence function, we define the following:
\begin{equation}
    \hat{g}_{-p_r}^{*}=\underset{g \in \Gamma_0}\argmin \sum_{\substack{j=1, j \neq p_r}}^{k}\sum_{i=1}^{n} \ell\left(g^j\left(x_{i}\right), c^{j}_i\right).
\end{equation}
\begin{equation}
    \hat{g}=\underset{g \in T}\argmin \sum_{\substack{j=1, j \neq p_r}}^{k} \sum_{i=1}^{n} \ell\left(g^{j}\left(x_{i}\right), c_i^j\right)
    +\sum_{i=1}^n \ell\left(g^p_r(x_i), c_i^{p_r}\right).
\end{equation}
\begin{equation}
    \hat{g}_{\epsilon} \triangleq \underset{g \in T}\argmin \sum_{\substack{j=1, j \neq p_r}}^{k} \sum_{i=1}^{n}\ell\left(g^{j}\left(x_{i}\right), c^{j}_i\right)+\epsilon \cdot \sum_{i=1}^{n} \ell\left(g^{p_r}\left(x_{i}\right), c^{p_r}_i\right).
\end{equation}
When ϵ→0\epsilon \rightarrow 0, ˆgϵ→ˆg∗−pr\hat{g}_{\epsilon} \rightarrow \hat{g}_{-p_r}^{*}, by the condition of the minimizer, we can obtain:
\begin{equation}
    \nabla_{g}\sum_{\substack{j=1, j \neq p_r}}^{k} \sum_{i=1}^{n} \ell\left(\hat{g}_{-p_r}^{*j}\left(x_{i}\right), c^{j}_i\right)=0
\end{equation}
Perform a Taylor expansion of the above equation at ˆgϵ\hat{g}_{\epsilon}, we can obtain

\begin{equation*}
    \nabla_{\hat{f}} \sum_{i=1}^{n} \ell ( \hat{f}( \hat{g}^{*}_{-p_r} (x_{i})), y_{i})
= -\nabla_{\hat{f}} \sum_{i=1}^{n} \ell \left( \hat{f} \left( \hat{g} (x_i) - H^{-1}_{\hat{g}} \cdot \nabla_{\hat{g}} \sum_{j=1, j \neq r}^{k} \sum_{i=1}^{n} \ell ( \hat{g}_{j} (x_i), c_j) \right) , y_i \right).
\end{equation*}

Substitute $\nabla_{\hat{f}} \sum_{i=1}^{n} \ell ( \hat{f}( \hat{g}^{*}_{-p_r} (x_{i})), y_{i})$ to equation \ref{eq:1}, we get the final closed-form influence function:

\begin{equation}
    \hat{f}_{-p_r}
= -H_{\hat{f}}^{-1} \cdot   \nabla_{\hat{f}} \sum_{i=1}^{n} \ell \left( \hat{f} \left( \hat{g} (x_i) - H^{-1}_{\hat{g}} \cdot \nabla_{\hat{g}} \sum_{j=1, j \neq r}^{k} \sum_{i=1}^{n} \ell ( \hat{g}_{j} (x_i), c_j) \right) , y_i \right).
\end{equation}

\noindent{\bf First Stage.}
To obtain the approximation of the parameters change. Motivated by \cite{koh2017understanding}, we do a derivation and definition of the influence function.
\begin{equation}
    \hat{g}_{\epsilon, -z_r} = \argmin \sum_{i \neq r} \ell(g(x_i), c_i) + \epsilon \cdot \ell\left(g(x_r), c_r\right).
\end{equation}
Then, when $\epsilon \to 0$, $\hat{g}_{\epsilon, -z_r} \to \hat{g}$.
\begin{equation}
    \mathcal{I}(z_r) \stackrel{\text { def }}{=} \frac{d \hat{g}_{\epsilon, -z_r}}{d \epsilon}|_{\epsilon=0}=-H_{\hat{g}}^{-1} \nabla_{\hat{g}} \sum \ell\left(\hat{g}(x_i),c_i\right),  
\end{equation}
Then, we can linearly approximate $\hat{g}_{-z_r}$ by computing $\hat{g} - 1 \cdot \mathcal{I}(z_r)$.

\noindent{\bf Second Stage.} Now we approximate $\hat{f}_{-z_r}$.
\begin{equation}
    \hat{f}_{-z_r} = \argmin_{f}\sum_{\substack{i = 1}}^{n} \ell(f\left(\hat{g}_{-z_r}(x_{i})\right), y_{i}) - \ell\left(f(\hat{g}_{-z_r}(x_r)), y_r\right)
\end{equation}
\begin{equation}
    \hat{f}_{-z_r}^* = \argmin_{f}\sum_{\substack{i = 1}}^{n} \ell(f\left(\hat{g}(x_{i})\right), y_{i})- \ell\left(f(\hat{g}(x_r)), y_r\right)
\end{equation}
We can evaluate the difference between $\hat{f}^*_{-z_r}$ and $\hat{f}$, and then approximate $\hat{f}_{-z_r} - \hat{f}^*_{-z_r}$ use the method similar to Appendix \ref{ap1}. Finally, we get the closed-form solution,

\begin{align*}
&\hat{f}_{-z_r} = \hat{f} + H^{-1}_{\hat{f}}  \left(  
\nabla_{\hat{f}} \sum_{i=1}^{n} \ell \left(   \hat{f} ( \hat{g} (x_i) ) , y_i   \right) \right) \\
& \cdot \left(  1  -  \left( \nabla_{\hat{f}} \ell \left( 
\hat{f} ( \hat{g} (x_r) ),y_r \right) \cdot \left( 
\nabla_{\hat{f}} \sum_{i=1,i \neq r}^{n} \ell \left(   \hat{f} ( \hat{g} (x_i) ) , y_i   \right)  -  \nabla_{\hat{f}} \sum_{i=1, i \neq r }^{n} \ell \left( 
\hat{f} ( \hat{g} (x_i) ),y_i \right) \right) \right) \right).
\end{align*}

Similar to previous practice, we approximate the retrained concept predicting model first and obtain the approximation of $\hat{g}_{c_w^r = 0}$ as 
\begin{equation}\label{4.4-1}
    \hat{g}_{c^r_w=0} \approx \hat{g} -H^{-1}_{\hat{g}} \cdot \nabla_g \sum_{j=1}^k \sum_{i=1}^n  \ell ( \hat{g}^j(x_i), c^j_i)
\end{equation}
On the other hand, we estimate $\hat{f}_{c_w^r = 0}$ as:
\begin{equation}\label{4.4-2}
    \hat{f}_{c_w^r = 0} \approx \hat{f}  -H^{-1}_{\hat{f}}\cdot\sum_{i=1}^n\nabla_f  \left( \ell \left( \hat{f} \left( \hat{g}_{\epsilon, c^r_w=0} \left(x_{i} \right) \right), y_{i}\right)-  \ell \left(  \hat{f}\left(\hat{g}\left(x_{i} \right) \right), y_{i} \right) \right),
\end{equation}
Substituting equation \ref{4.4-2} into equation \ref{4.4-1}, we have
\begin{align}
     \hat{f}_{c_w^r = 0} &= \hat{f} + H^{-1}_{\hat{f}} \cdot \nabla_f \sum_{i=1}^n \ell \left(   \hat{f} \left( \hat{g} ( x_{i} ) 
 \right) , y_{i} \right) \notag \\
     & - H^{-1}_{\hat{f}} \cdot \nabla_f \sum_{i=1}^n \left( \ell \left( \hat{f} \left( \hat{g} (x_{i} )
    - H^{-1}_{\hat{g}} \cdot \nabla_g \sum_{j=1}^k\sum_{i=1}^n \ell ( \hat{g}^j(x_i), c^j_i) ( x_i ) \right) , y_{i_c} \right) \right).
\end{align}

\begin{algorithm}[h]
\caption{Concept-level ECBM \label{alg:2}}
\begin{algorithmic}[1]
    \State {\bf Input:} Dataset $\mathcal{D} = \{ (x_i, y_i, c_i) \}_{i=1}^{N}$, original concept predictor $\hat{f}$, and label predictor $\hat{g}$.
    \State Set $p_r = 0$ for all $\mathcal{D}$.
    \For {$i=1,\cdots, k$} \quad \quad \quad   \# Update concept predictor
    \If {$i=r$}
        \State Update $\Tilde{g}^{r}$:
    \begin{equation*}
        \Tilde{g}^{r} \approx \hat{g} (x_i) - H^{-1}_{\hat{g}} \cdot \nabla_{\hat{g}} \sum_{j=1, j \neq r}^{k} \sum_{i=1}^{n} \ell ( \hat{g}_{j} (x_i), c_j).
    \end{equation*}
    \Else
        \State Update other concept predictors:
        $\Tilde{g}^i=\hat{g}^i$.
    \EndIf
    \EndFor 
    \State Update label predictor $\Tilde{f}$:
    \begin{equation*}
    \hat{f}_{-p_r}
    \approx \hat{f}-H_{\hat{f}}^{-1} \cdot   \nabla_{\hat{f}} \sum_{i=1}^{n} \ell \left( \hat{f} \left( \hat{g} (x_i) - H^{-1}_{\hat{g}} \cdot \nabla_{\hat{g}} \sum_{j=1, j \neq r}^{k} \sum_{i=1}^{n} \ell ( \hat{g}_{j} (x_i), c_j) \right) , y_i \right).
    \end{equation*}
    \State {\bf Return: $\Tilde{f}$, $\Tilde{g}$}.  
\end{algorithmic}
\end{algorithm}





% The gradients on parameters θl=(W,b)\theta_{l} = \left(W, b \right) is 
% \begin{equation*}
%     \nabla_{\theta} = \frac{\partial L}{\partial \theta} = \mathrm{vec}\left(h \delta^{\mathrm{T}}\right).  
% \end{equation*}
% The Kronecker factored approximation of corresponding $G^{l}$ is 
% \begin{align*}
% G^{l}  = & \mathbb{E} \left[ \nabla_{\theta} \nabla_{\theta}^{\mathrm{T}} \right]\\
% \approx &  \mathbb{E} \left[h h^{\mathrm{T}} \right] \otimes \mathbb{E} \left[ \delta \delta^{\mathrm{T}}\right]
% \end{align*}
% Plugging the notation for convolution layer, we have 
% \begin{equation*}
%     {G^{(l)}} \approx {A} \otimes {B} 
% \end{equation*}
% where
% \begin{align*}
% A=\mathbb{E}\left[\sum_{t, t^{\prime}\in\mathcal{T} } h^{t} h^{t^{\prime} \top}\right], B=\mathbb{E}\left[\sum_{t, t^{\prime}\in \mathcal{T}} \delta^{t} \delta^{t^{\prime} \top}\right] 
% \end{align*}
% and hth^{t} is flattened input subtensor (receptive field) at position tt, δt\delta^{t} is the gradient of LL w.r.t. output of filter at position tt.



% \begin{array}{l}  
 
% A=\mathbb{E}\left[\sum_{\left(s, s^{\prime}\right)} h^{s} h^{s^{\prime} \top}\right], B=\mathbb{E}\left[\sum_{\left(s, s^{\prime}\right)} \delta^{s} \delta^{s^{\prime} \top}\right] \\  
% \end{array}  
% $$  
% $s \in \mathcal{S}, s^{\prime} \in \mathcal{S}$ : spatial positions iterated over by the filter $h^{s}$ : flattened input subtensor (receptive field) at position $s$ $\delta^{s}$ : gradient of $\ell$ w.r.t. output of filter at position $s$

% $\underset{\left(n_{\text {in }} n_{\text {out }} k_{w} k_{h}\right)^{2}}$
% $\underset{\left(n_{\text {in }} k_{w} k_{h}\right)^{2}}$


% And this layer is parameterized by a set of weights $w_{i, j, \delta}$ and biases $b_{i}$, where $i \in\{1, \ldots, I\}$ indexes the output map, $j$ indexes the input map, and $\delta \in \Delta$ indexes the spatial offset (from the center of the filter). If the filters are of size $(2 R+1) \times(2 R+1)$, then we would have $\Delta=\{-R, \ldots, R\} \times\{-R, \ldots, R\}$. We denote the numbers of spatial locations and spatial offsets as $|\mathcal{T}|$ and $|\Delta|$, respectively. The convolution layer computes a set of pre-activations $\left\{s_{i, t}\right\}$ as follows:  




% To this end, consider the $l$-th layer of $\hat{g}$ which takes $\left\{a_{j, t}\right\}$ as input. And this layer is parameterized by a set of weights $w_{i, j, \delta}$ and biases $b_{i}$, where $i \in\{1, \ldots, I\}$ indexes the output map, $j$ indexes the input map, and $\delta \in \Delta$ indexes the spatial offset (from the center of the filter). If the filters are of size $(2 R+1) \times(2 R+1)$, then we would have $\Delta=\{-R, \ldots, R\} \times\{-R, \ldots, R\}$. We denote the numbers of spatial locations and spatial offsets as $|\mathcal{T}|$ and $|\Delta|$, respectively. The convolution layer computes a set of pre-activations $\left\{s_{i, t}\right\}$ as follows:  
% $$  
% s_{i, t}=\sum_{\delta \in \Delta} w_{i, j, \delta} a_{j, t+\delta}+b_{i},  
% $$  


% %----------------
% $$  
% \begin{array}{l}  
% \underset{\left(n_{\text {in }} n_{\text {out }} k_{w} k_{h}\right)^{2}}{G^{(l)}} \approx \underset{\left(n_{\text {in }} k_{w} k_{h}\right)^{2}}{A} \otimes \underset{\left(n_{\text {out }}\right)^{2}}{B} \\  
% A=\mathbb{E}\left[\sum_{\left(s, s^{\prime}\right)} h^{s} h^{s^{\prime} \top}\right], B=\mathbb{E}\left[\sum_{\left(s, s^{\prime}\right)} \delta^{s} \delta^{s^{\prime} \top}\right] \\  
% \end{array}  
% $$  
% $s \in \mathcal{S}, s^{\prime} \in \mathcal{S}$ : spatial positions iterated over by the filter $h^{s}$ : flattened input subtensor (receptive field) at position $s$ $\delta^{s}$ : gradient of $\ell$ w.r.t. output of filter at position $s$

% %----------------



% the parameters $\theta_{l}$ for $l$-th layer includes input, weights, bias and outputs are denoted a layer of activation $\left\{a_{j, t}\right\}$, where $j \in\{1, \ldots, J\}$ indexes the input map and $t \in \mathcal{T}$ indexes the spatial location which is typically a 2-D grid. Assume convolution is performed with a stride of 1 and padding equal to $R$, so that the set of spatial locations is shared between the input and output feature maps.


% where $b_{i}$ denotes the bias parameter. The activations are defined to take the value 0 outside of $\mathcal{T}$. The pre-activations are passed through a nonlinearity such as ReLU to compute the output layer activations, but we have no need to refer to this explicitly when analyzing a single layer. (For simplicity, we assume operations such as pooling and response normalization are implemented as separate layers.)  
  
% Pre-activation derivatives $\mathcal{D} s_{i, t}$ are computed during backpropagation. One then computes weight derivatives as:  
% \begin{equation}\label{con_layer}
%     \mathcal{D} w_{i, j, \delta}=\sum_{t \in \mathcal{T}} a_{j, t+\delta} \mathcal{D} s_{i, t}.
% \end{equation}






% \section{EK-FAC acceleration}
% Noting that all the theorems in our work requires computing an inverse-Hessian-vector product(IHVP), i.e., $H^{-1}v$ for some vector $v$. 
% This is a computational bottleneck for large models, since each dimension of this matrix, $H$, is equal to the number of model parameters phases. 
% In this section, we utilize Eigenvalue Kronecker-Factored Approximate Curvature(EK-FAC) method to the Fisher information matrix(FIM) to approximate IHVP.
% And the FIM is defined as follows:
% \begin{equation*}
%     F = \mathbb{E}_{x \sim p_{\text{data}}, y \sim P_{y \mid x}(\theta)} \left[ \nabla_{{\theta}} \log p (y \mid \theta, x) {\nabla_{{\theta}} \log p (y \mid \theta, x)}^{\mathrm{T}}\right].
% \end{equation*}
% where $p_{\text{data}}$ is the data distribution and $P_{y \mid x}(\theta)$ is the model's output distribution over $y$. And $y$ is sampled from the output distribution, we use the training labels instead yields the empirical Fisher matrix as an alternative.
% \subsection{EK-FAC for Convolution Layer}
% In our CBM model, the label predictor is a single linear layer and the cost for Hessian computing is affordable. However, the concept predictor is based on Resnet-18, which has much more parameters. Therefore, we perform a EK-FAC for $\hat{g}$.
% \begin{equation*}
%     \hat{g} = \argmin_g \sum_{j=1}^{k}  L_{C_j} = \argmin_g \sum_{j=1}^k\sum_{i=1}^n \ell(g^j(x_i),c_i^j),
% \end{equation*}
% we define $H_{\hat{g}} = \nabla^2_{\hat{g}}L_{C_j}$ as the Hessian matrix of the loss function with respect to the parameters. The Gauss-Newton Hessian (GNH),  serves as an estimate of $H$ that approximates the linearization of the parameter-output relationship of the network around its current parameters(\cite{martens2020new}), and is denoted as 
% \begin{equation*}
%     G=\mathbb{E}\left[J^{\top} H_{y} J\right]
% \end{equation*}
% where $J = \frac{\mathrm{d}y}{\mathrm{d}{\hat{g}}}$, $H_{y} = \nabla_{y}^2 L_{C_j}$ is the Hessian of the loss with respect to the network’s outputs, and the expectation is with respect to the empirical distribution.
% %index ref{martens2020new}

% \cite{martens2020new} shows that there is quite general equivalence between FIM and GNH, especially for several common loss functions like cross-entropy and squared error. Therefore, we can use FIM instead of GNH as an estimate of $H_{\hat{g}}$.

% % On the other hand, EK-FAC method provides a parameterized estimate of FIM for a neural network, facilitating efficient inversion. Although initially developed for optimization tasks with considerations like step size selection, our attention here is solely on the fundamental FIM approximation. 
% We provide the EK-FAC method for approximating the Hessian matrix for the concept predictor here.


% \subsection{Convolution layer}
% The block-diagonal version of K-FAC is based on two approximations to F which together make it tractable to invert. Firstly, it is assumed that the weight derivatives in various layers are independent, leading to the block diagonal structure of F, where each layer corresponds to a separate block:
% \begin{equation*}
%     F \approx\left(\begin{array}{ccc}E\left[\operatorname{vec}\left(\mathcal{D} \overline{W}_{1}\right) \operatorname{vec}\left(\mathcal{D} \overline{W}_{1}\right)^{\top}\right] & & \mathbf{0} \\ & \ddots & \\ \mathbf{0} & & \mathbb{E}\left[\operatorname{vec}\left(\mathcal{D} \overline{W}_{L}\right) \operatorname{vec}\left(\mathcal{D} \overline{W}_{L}\right)^{\top}\right]\end{array}\right)
% \end{equation*}
% This approximation alone is inadequate, as each of the blocks could still be significantly large. We perform the second approximation in the following part.

% Consider the ll-th layer of ˆg\hat{g} which takes as input 
% input, weights, bias and outputs are denoted a layer of activations $\left\{a_{j, t}\right\}$, where $j \in\{1, \ldots, J\}$ indexes the input map and $t \in \mathcal{T}$ indexes the spatial location which is typically a 2-D grid. Assume convolution is performed with a stride of 1 and padding equal to $R$, so that the set of spatial locations is shared between the input and output feature maps.
% This layer is parameterized by a set of weights $w_{i, j, \delta}$ and biases $b_{i}$, where $i \in\{1, \ldots, I\}$ indexes the output map, $j$ indexes the input map, and $\delta \in \Delta$ indexes the spatial offset (from the center of the filter). If the filters are of size $(2 R+1) \times(2 R+1)$, then we would have $\Delta=\{-R, \ldots, R\} \times\{-R, \ldots, R\}$. We denote the numbers of spatial locations and spatial offsets as $|\mathcal{T}|$ and $|\Delta|$, respectively. The convolution layer computes a set of pre-activations $\left\{s_{i, t}\right\}$ as follows:  
% $$  
% s_{i, t}=\sum_{\delta \in \Delta} w_{i, j, \delta} a_{j, t+\delta}+b_{i},  
% $$  
% where $b_{i}$ denotes the bias parameter. The activations are defined to take the value 0 outside of $\mathcal{T}$. The pre-activations are passed through a nonlinearity such as ReLU to compute the output layer activations, but we have no need to refer to this explicitly when analyzing a single layer. (For simplicity, we assume operations such as pooling and response normalization are implemented as separate layers.)  
  
% Pre-activation derivatives $\mathcal{D} s_{i, t}$ are computed during backpropagation. One then computes weight derivatives as:  
% \begin{equation}\label{con_layer}
%     \mathcal{D} w_{i, j, \delta}=\sum_{t \in \mathcal{T}} a_{j, t+\delta} \mathcal{D} s_{i, t}.
% \end{equation}

% \subsection{K-FAC for convolution layer}
% Recall the definition of FIM and plug equation \ref{con_layer} in, then we have
% \begin{equation*}
%     \mathbb{E}\left[\mathcal{D} w_{i, j, \delta} \mathcal{D} w_{i^{\prime}, j^{\prime}, \delta^{\prime}}\right]=\mathbb{E}\left[\left(\sum_{t \in \mathcal{T}} a_{j, t+\delta} \mathcal{D} s_{i, t}\right)\left(\sum_{t^{\prime} \in \mathcal{T}} a_{j^{\prime}, t^{\prime}+\delta^{\prime}} \mathcal{D} s_{i^{\prime}, t^{\prime}}\right)\right]
% \end{equation*}
% Before the approximation, we need to recall the following three assumptions proposed in \cite{grosse2016kronecker}:
% \begin{itemize}
% \item Independent activations and derivatives (IAD). The activations are independent of the pre-activation derivatives, i.e. $\left\{a_{j, t}\right\}\perp\left\{\mathcal{D} s_{i, t^{\prime}}\right\}$. 
% \item Spatial homogeneity (SH). The first-order statistics of the activations are independent of spatial location. The second-order statistics of the activations and pre-activation derivatives at any two spatial locations $t$ and $t^{\prime}$ depend only on $t^{\prime}-t$. This implies there are functions $M, \Omega$ and $\Gamma$ such that:  
% $$  
% \begin{aligned}  
% \mathbb{E}\left[a_{j, t}\right] & =M(j) \\  
% \mathbb{E}\left[a_{j, t} a_{j^{\prime}, t^{\prime}}\right] & =\Omega\left(j, j^{\prime}, t^{\prime}-t\right) \\  
% \mathbb{E}\left[\mathcal{D} s_{i, t} \mathcal{D} s_{i^{\prime}, t^{\prime}}\right] & =\Gamma\left(i, i^{\prime}, t^{\prime}-t\right) .  
% \end{aligned}  
% $$  
% Note that $\mathbb{E}\left[\mathcal{D} s_{i, t}\right]=0$ under the model's distribution, so 
% \begin{equation*}
% \operatorname{Cov}\left(\mathcal{D} s_{i, t}, \mathcal{D} s_{i^{\prime}, t^{\prime}}\right)=\mathbb{E}\left[\mathcal{D} s_{i, t} \mathcal{D} s_{i^{\prime}, t^{\prime}}\right].
% \end{equation*}
% \item Spatially uncorrelated derivatives (SUD). The pre-activation derivatives at any two distinct spatial locations are uncorrelated, i.e. $\Gamma\left(i, i^{\prime}, \delta\right)=0$ for $\delta \neq 0$.
% \end{itemize}
% Let $\hat{F_{\ell}} \approx \mathbb{E}\left[\operatorname{vec}\left(\mathcal{D} \overline{W}_{\ell}\right) \operatorname{vec}\left(\mathcal{D} \overline{W}_{\ell}\right)^{\top}\right]$ denote the block of the approximate Fisher for layer $\ell$. Because the data are two-dimensional, the offsets can be parameterized with indices $\delta=\left(\delta_{1}, \delta_{2}\right)$ and $\delta^{\prime}=\left(\delta_{1}^{\prime}, \delta_{2}^{\prime}\right)$, and denote the dimensions of the activations map as $\left(T_{1}, T_{2}\right)$. 
% Theorem 1 in \cite{grosse2016kronecker} yields our KFC factorization of $\hat{{F}}_{\ell}$ into a Kronecker product of smaller factors:
% \begin{equation*}
% \hat{F}_{\ell}={\Omega}_{\ell-1} \otimes {\Gamma}_{\ell}
% \end{equation*}
% where
% \begin{equation*}
%     \begin{aligned} 
% {\left[{\Omega}_{\ell-1}\right]_{j|\Delta|+\delta, j^{\prime}|\Delta|+\delta^{\prime}} } & \triangleq \beta\left(\delta, \delta^{\prime}\right) \Omega\left(j, j^{\prime}, \delta^{\prime}-\delta\right) \\ {\left[{\Omega}_{\ell-1}\right]_{j|\Delta|+\delta, 0}=\left[{\Omega}_{\ell-1}\right]_{0, j|\Delta|+\delta} } & \triangleq \beta(\delta) M(j) \\ {\left[{\Omega}_{\ell-1}\right]_{0,0} } & \triangleq|\mathcal{T}| \\ {\left[{\Gamma}_{\ell}\right]_{i, i^{\prime}} } & \triangleq \Gamma\left(i, i^{\prime}, 0\right) .
% \end{aligned}
% \end{equation*}
% and
% \begin{equation*}
% \begin{aligned} 
% \beta(\delta) & \triangleq\left(T_{1}-\left|\delta_{1}\right|\right)\left(T_{2}-\left|\delta_{2}\right|\right) \\
% \beta\left(\delta, \delta^{\prime}\right) & \triangleq\left(T_{1}-\max \left(\delta_{1}, \delta_{1}^{\prime}, 0\right)+\min \left(\delta_{1}, \delta_{1}^{\prime}, 0\right)\right) \cdot\left(T_{2}-\max \left(\delta_{2}, \delta_{2}^{\prime}, 0\right)+\min \left(\delta_{2}, \delta_{2}^{\prime}, 0\right)\right)
% \end{aligned}
% \end{equation*}
% Recall the Theorem 2 in \cite{grosse2016kronecker}, Under assumption SH, we estimate each $\Omega$ and $\Gamma$ directly by the following fact:
% \begin{equation}
%     \begin{aligned}  
% {\Omega}_{\ell} & =\mathbb{E}\left[ \llbracket {{A}}_{\ell} \rrbracket_{H}^{\mathrm{T}} \llbracket {{A}}_{\ell} \rrbracket_{H} \right] \\  
% {\Gamma}_{\ell} & =\frac{1}{|\mathcal{T}|} \mathbb{E}\left[\mathcal{D} {S}_{\ell}^{\top} \mathcal{D} {S}_{\ell}\right]  
% \end{aligned} 
% \end{equation}
% where  $\llbracket \tilde{\mathbf{A}}_{\ell} \rrbracket$ is the expanded activation as
% \begin{equation}\label{expand_op}
%     \llbracket \tilde{\mathbf{A}}_{\ell} \rrbracket_{t M+m, j|\Delta|+\delta}=[\tilde{\mathbf{A}}_{\ell}]_{(t+\delta) M+m, j}=a_{j, t+\delta}^{(m)},
% \end{equation}
% for all entries such that t+δ∈Tt+\delta \in \mathcal{T}. All other entries are defined to be 0 . Here, mm indexes the data instance within the mini-batch.

% The extension operators is an operator used to overcome the problem of poor convolutional memory localisation and thus efficiently implemented, denoted as \llbracket⋅\rrbracket\llbracket\cdot\rrbracket, which extracts patches around each spatial location and flattens them into vectors, and these vectors become the rows of a matrix. For instance, M×|T|×JM \times|\mathcal{T}| \times J array ˜Aℓ\tilde{{A}}_{\ell}, where MM is the mini-batch size, |T||\mathcal{T}| is the number of spatial locations, and JJ is the number of feature maps. Then, \llbracket˜Aℓ\rrbracket\llbracket \tilde{\mathbf{A}}_{\ell} \rrbracket is a M|T|×J|Δ|M |\mathcal{T}| \times J |\Delta| matrix, defined as equation ???\ref{expand_op}.

% Using this result, we define the empirical statistics for a given mini-batch:  
% $$  
% \begin{aligned}  
% \hat{{\Omega}}_{\ell-1} & =\frac{1}{M} \llbracket \tilde{{A}}_{\ell-1} \rrbracket_{H}^{\top} \llbracket \tilde{{A}}_{\ell-1} \rrbracket_{H} \\  
% \hat{{\Gamma}}_{\ell} & =\frac{1}{M|\mathcal{T}|} \mathcal{D} \tilde{{S}}_{\ell}^{\top} \mathcal{D} \tilde{{S}}_{\ell}  
% \end{aligned}  
% $$
% Since subsequent inverse operations are required and the current approximation for FIM or GNH  is PSD, we actually use a damped version for FIM as ˆF=F+γI\hat{F} = F + \gamma I, 

% \subsection{EK-FAC for convolution layer}
% In this part, for the sake of simplicity, we drop the layer subscript and aproxiamate hat.

% The K-FAC approximation also allows for efficient computation of eigendecomposition. In particular, eigendecomposition can be distributed across Kronecker products. That is, if ˆΩ\mathbf{\hat{\Omega}} and ˆΓ\mathbf{\hat{\Gamma}} have eigendecomposition 
% \mathbf{Q}_{\mathbf{\Omega}} \boldsymbol{\Lambda}_{\mathbf{\Omega}} \mathbf{Q}_{\mathbf{\Omega}}^{\top}\mathbf{Q}_{\mathbf{\Omega}} \boldsymbol{\Lambda}_{\mathbf{\Omega}} \mathbf{Q}_{\mathbf{\Omega}}^{\top}\mathbf{Q}_{\mathbf{\Omega}} \boldsymbol{\Lambda}_{\mathbf{\Omega}} \mathbf{Q}_{\mathbf{\Omega}}^{\top}\mathbf{Q}_{\mathbf{\Omega}} \boldsymbol{\Lambda}_{\mathbf{\Omega}} \mathbf{Q}_{\mathbf{\Omega}}^{\top} and \mathbf{Q}_{\mathbf{\Gamma}} \boldsymbol{\Lambda}_{\mathbf{\Gamma}} \mathbf{Q}_{\mathbf{\Gamma}}^{\top}\mathbf{Q}_{\mathbf{\Gamma}} \boldsymbol{\Lambda}_{\mathbf{\Gamma}} \mathbf{Q}_{\mathbf{\Gamma}}^{\top}\mathbf{Q}_{\mathbf{\Gamma}} \boldsymbol{\Lambda}_{\mathbf{\Gamma}} \mathbf{Q}_{\mathbf{\Gamma}}^{\top}\mathbf{Q}_{\mathbf{\Gamma}} \boldsymbol{\Lambda}_{\mathbf{\Gamma}} \mathbf{Q}_{\mathbf{\Gamma}}^{\top}, respectively, then the eigendecomposition of \mathbf{\Omega} \otimes \mathbf{\Gamma}\mathbf{\Omega} \otimes \mathbf{\Gamma} can be written as: 
% $$  
% \begin{aligned}  
% \mathbf{\Omega} \otimes \mathbf{\Gamma} & =\mathbf{Q}_{\mathbf{\Omega}} \boldsymbol{\Lambda}_{\mathbf{\Omega}} \mathbf{Q}_{\mathbf{\Omega}}^{\top} \otimes \mathbf{Q}_{\mathbf{\Gamma}} \boldsymbol{\Lambda}_{\mathbf{\Gamma}} \mathbf{Q}_{\mathbf{\Gamma}}^{\top} \\  
% & =\left(\mathbf{Q}_{\mathbf{\Omega}} \otimes \mathbf{Q}_{\mathbf{\Gamma}}\right)\left(\boldsymbol{\Lambda}_{\mathbf{\Omega}} \otimes \mathbf{\Lambda}_{\mathbf{\Gamma}}\right)\left(\mathbf{Q}_{\mathbf{\Omega}} \otimes \mathbf{Q}_{\mathbf{\Gamma}}\right)^{\top}  
% \end{aligned}  
% $$



% %_-------------

% 2.2.3 Eigenvalue-Corrected Kronecker-Factored Approximate Curvature  
  
% The K-FAC approximation admits not only efficient IHVP computation but also efficient eigendecomposition. Specifically, eigendecompositions distribute over Kronecker products, so if the factors A\mathbf{A} and S\mathbf{S} (we drop the layer subscripts to avoid clutter) have eigendecomposition \mathbf{Q}_{\mathbf{A}} \boldsymbol{\Lambda}_{\mathbf{A}} \mathbf{Q}_{\mathbf{A}}^{\top}\mathbf{Q}_{\mathbf{A}} \boldsymbol{\Lambda}_{\mathbf{A}} \mathbf{Q}_{\mathbf{A}}^{\top} and \mathbf{Q}_{\mathbf{S}} \boldsymbol{\Lambda}_{\mathbf{S}} \mathbf{Q}_{\mathbf{S}}^{\top}\mathbf{Q}_{\mathbf{S}} \boldsymbol{\Lambda}_{\mathbf{S}} \mathbf{Q}_{\mathbf{S}}^{\top}, respectively, then the eigendecomposition of \mathbf{A} \otimes \mathbf{S}\mathbf{A} \otimes \mathbf{S} can be written as:  
% $$  
% \begin{aligned}  
% \mathbf{A} \otimes \mathbf{S} & =\mathbf{Q}_{\mathbf{A}} \boldsymbol{\Lambda}_{\mathbf{A}} \mathbf{Q}_{\mathbf{A}}^{\top} \otimes \mathbf{Q}_{\mathbf{S}} \boldsymbol{\Lambda}_{\mathbf{S}} \mathbf{Q}_{\mathbf{S}}^{\top} \\  
% & =\left(\mathbf{Q}_{\mathbf{A}} \otimes \mathbf{Q}_{\mathbf{S}}\right)\left(\boldsymbol{\Lambda}_{\mathbf{A}} \otimes \mathbf{\Lambda}_{\mathbf{S}}\right)\left(\mathbf{Q}_{\mathbf{A}} \otimes \mathbf{Q}_{\mathbf{S}}\right)^{\top}  
% \end{aligned}  
% $$
  
% Observe that \boldsymbol{\Lambda}_{\mathbf{A}}\boldsymbol{\Lambda}_{\mathbf{A}} and \boldsymbol{\Lambda}_{\mathbf{S}}\boldsymbol{\Lambda}_{\mathbf{S}} are (M+1) \times(M+1)(M+1) \times(M+1) and P \times PP \times P diagonal matrices, and their Kronecker product is a (M+1) P \times(M+1) P(M+1) P \times(M+1) P diagonal matrix. Because this larger diagonal matrix \boldsymbol{\Lambda}_{\mathbf{A}} \otimes \boldsymbol{\Lambda}_{\mathbf{S}}\boldsymbol{\Lambda}_{\mathbf{A}} \otimes \boldsymbol{\Lambda}_{\mathbf{S}} has only (M+1) P(M+1) P entries, we can afford to fit and store the diagonal entries individually rather than assuming the Kronecker structure.  
  
% The Eigenvalue-corrected K-FAC (EK-FAC) (George et al., 2018) approximation does exactly this. After computing the eigendecomposition of the original Kronecker factors, it fits a more accurate GNH approximation such that:  
% $$  
% \mathbf{G} \approx\left(\mathbf{Q}_{\mathbf{A}} \otimes \mathbf{Q}_{\mathbf{s}}\right) \mathbf{\Lambda}\left(\mathbf{Q}_{\mathbf{A}} \otimes \mathbf{Q}_{\mathbf{s}}\right)^{\top}  
% $$  
% where \boldsymbol{\Lambda}\boldsymbol{\Lambda} is diagonal matrix of dimension (M+1) P(M+1) P defined as:  
% $$  
% \boldsymbol{\Lambda}_{i i}=\mathbb{E}\left[\left(\left(\mathbf{Q}_{\mathbf{A}} \otimes \mathbf{Q}_{\mathbf{S}}\right) \mathcal{D} \boldsymbol{\theta}\right)_{i}^{2}\right]  
% $$



==> ICML_section/rebuttal.tex <==
\section{Additional Experiment}

\subsection{Improvement via Harmful Data Removal}

We conducted addition experiments on CUB datasets with synthetically introduced noisy concepts or labels. Firstly, we introduce noises under three levels. In concept level, we choose 10\% of the concepts and flip these concept labels for a portion of the data. In data level, we choose 10\% of the data and flip their labels. In concept-label level, we choose 10\% of the total concepts and flip them. Then we conduct the following experiments.

We introduce noises into the three levels and train the model. After that, we remove the noise and obtain the retrained mdoel, which is the ground truth(gt) of this harmful data removal task. In contrast, we use ECBM to remove the harmful data. 
\begin{figure}[ht]
    \centering
    \begin{tabular}{c}
        \includegraphics[width=0.95\linewidth]{images/harmful_removal.png} 
    \end{tabular}
    \caption{Model performance after the removal of harmful data.}
    \label{hramful_removal}
\end{figure}

From figure \ref{hramful_removal}, it can be observed that the model performance improves across all three settings after noise removal and subsequent retraining or ECBM editing. This confirms that the performance of ECBM is nearly equivalent to retraining in various experimental scenarios, further providing evidence of the robustness of our method.


\noindent {\bf Model Unlearning.} 
Model unlearning has gained significant attention in recent years, with various methods~\citep{bourtoule2021machine,brophy2021machine,cao2015towards, chen2022recommendation,chen2022graph} proposed to efficiently remove the influence of certain data from trained machine learning models. Existing approaches can be broadly categorized into exact and approximate unlearning methods. Exact unlearning methods aim to replicate the results of retraining by selectively updating only a portion of the dataset, thereby avoiding the computational expense of retraining on the entire dataset~\citep{sekhari2021remember, chowdhury2024towards}. Approximate unlearning methods, on the other hand, seek to adjust model parameters to approximately satisfy the optimality condition of the objective function on the remaining data~\citep{golatkar2020eternal,guo2019certified,izzo2021approximate}. These methods are further divided into three subcategories: (1) Newton step-based updates that leverage Hessian-related terms [22, 26, 31, 34, 40, 43, 49], often incorporating Gaussian noise to mitigate residual data influence. To reduce computational costs, some works approximate the Hessian using the Fisher information matrix~\citep{golatkar2020eternal} or small Hessian blocks~\citep{mehta2022deep}. (2) Neural tangent kernel (NTK)-based unlearning approximates training as a linear process, either by treating it as a single linear change~\citep{golatkar2020forgetting}. (3) SGD path tracking methods, such as DeltaGrad~\citep{wu2020deltagrad} and unrollSGD~\citep{thudi2022unrolling}, reverse the optimization trajectory of stochastic gradient descent during training. 
Despite their advancements, these methods fail to handle the special architecture of CBMs. Moreover, given the high cost of obtaining data, we sometimes prefer to correct the data rather than remove it, which model unlearning is unable to achieve.

==> figs/figRT.tex <==
\vspace{-7pt}
\begin{figure}[ht]
    \centering
\begin{tabular}{ccc}
\includegraphics[width=0.3\linewidth]{images/Concept-label-level.pdf}     & 
\includegraphics[width=0.3\linewidth]{images/Concept-level.pdf} & 
\includegraphics[width=0.3\linewidth]{images/Data-level.pdf} 
\end{tabular}
\caption{Running Time(RT) of different edition ratios on three settings on CUB dataset. \label{fig:rt}}
\vspace{-12pt}
\end{figure}

==> section/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}
Modern deep learning models, such as large language models~\citep{zhao2023survey,yang2024moral,yang2024human,xu2023llm,yang2024dialectical} and large multimodal~\citep{yin2023survey,ali2024prompt,cheng2024multi}, often exhibit intricate non-linear architectures, posing challenges for end-users seeking to comprehend and trust their decisions. This lack of interpretability presents a significant barrier to adoption, particularly in critical domains such as healthcare~\citep{ahmad2018interpretable,yu2018artificial} and finance \citep{cao2022ai}, where transparency is paramount. To address this demand, explainable artificial intelligence (XAI) models~\citep{das2020opportunities,hu2023seat,hu2023improving} have emerged, offering explanations for their behavior and insights into their internal mechanisms. Among these, Concept Bottleneck Models (CBMs) \citep{koh2020concept} have gained prominence for explaining the prediction process of end-to-end AI models. CBMs add a bottleneck layer for placing human-understandable concepts. In the prediction process, CBMs first predict the concept labels using the original input and then predict the final classification label using the predicted concept in the bottleneck layer, which provides a self-explained decision to users. 

%However, deriving efficient editable CBMs remains a critical concern, particularly in large-scale applications characterized by challenges such as model complexity, data mislabelling, and concept annotation errors. For example, consider scenarios where a physician annotates data with erroneous concepts or where a newly discovered concept significantly impacts prediction. Discarding mislabeled data or retraining models in such cases proves prohibitively expensive, especially in domains like medicine or chemistry, where data annotation is costly. Additionally, retraining large models is both resource-intensive and time-consuming. Therefore, the development of an efficient method to approximate prediction changes becomes paramount. Providing users with an adaptive approach to utilize such explainable models is crucial and pressing.

\input{figs/fig1}
Existing research on CBMs predominantly addresses two primary concerns: Firstly, CBMs heavily rely on laborious dataset annotation. Researchers have explored solutions to these challenges in unlabeled settings~\citep{oikarinen2023label,yuksekgonul2022post,lai2023faithful}. Secondly, the performance of CBMs often lags behind that of original models lacking the concept bottleneck layer, attributed to incomplete information extraction from original data to bottleneck features. Researchers aim to bridge this utility gap~\citep{NEURIPS2023_555479a2, yuksekgonul2022post, NEURIPS2022_867c0682}. However, few of them considered the adaptivity or editability of CBMs, crucial aspects encompassing annotation errors, data privacy considerations, or concept updates. Actually, these demands are increasingly pertinent in the era of large models. We delineate the editable setting into three key aspects (illustrated in Figure \ref{fig:intro}):
\begin{itemize}
    \item \emph{Concept-label-level:} 
    In most scenarios, concept labels 
    are annotated by humans or experts. Thus, it is unavoidable that there are some annotation errors, indicating that there is a need to correct some concept labels in a trained CBM. 
    \item \emph{Concept-level:} 
    In CBMs, the concept set is pre-defined by LLMs or experts. However, in many cases, evolving situations demand concept updates, as evidenced by discoveries such as chronic obstructive pulmonary disease as a risk factor for lung cancer, and doctors have the requirements to add related concepts. For another example, recent research found a new factor, obesity~\citep{sattar2020obesity} are risky for severe COVID-19 and factors (e.g., older age, male gender, Asian race) are risk associated with COVID-19 infection~\citep{rozenfeld2020model}. 
    On the other hand, one may also want to remove some spurious or unrelated concepts for the task. This demand is even more urgent in some rapidly evolving domains like the pandemic. 
    \item \emph{Data-level:}
    Data issues can arise in CBMs when training data is erroneous or poisoned. For example, if a doctor identifies a case as erroneous or poisoned, this data sample becomes unsuitable for training. Therefore, it is essential to have the capability to completely delete such data from the \rebuttal{learned} models. We need such an editable model that can interact effectively with doctors.
    %Data privacy issues arise as training data in CBMs always involves sensitive individual information. Specifically, according to regulations such as the General Data Protection Regulation (GDPR) \cite{paul2017gdpr}, and the California Consumer Privacy \cite{pardau2018california}. Patients and users have the right to revoke their sensitive data. Thus, one must have the ability to remove data lineage from learning models fully.
\end{itemize}
The most direct way to address the above three problems is retraining from scratch on the data after correction. However, retraining models in such cases prove prohibitively expensive, especially in large models, which is resource-intensive and time-consuming. Therefore, developing an efficient method to approximate prediction changes becomes paramount. Providing users with an adaptive and editable CBM is both crucial and urgent.

We propose Editable Concept Bottleneck Models (ECBMs) to tackle these challenges. Specifically, compared to retraining, ECBMs provide a mathematically rigorous closed-form approximation for the above three settings to address editability within CBMs efficiently. Leveraging the influence function~\citep{cook2000detection,cook1980characterizations}, we quantify the impact of individual data points, individual concept labels, and the concept for all data on model parameters. 
Despite the growing attention and utility of influence functions in machine learning~\citep{koh2017understanding}, their application in CBMs remains largely unexplored due to their composite structure, i.e., the intermediate representation layer.

To the best of our knowledge, we are the first to work to fill this gap by demonstrating the effectiveness of influence functions in elucidating the behavior of CBMs, especially in identifying mislabeled data and discerning the data influence. Comprehensive experiments on benchmark datasets show that our ECBMs are efficient and effective. Our contributions are summarized as follows.
\begin{itemize}
    \item We delineate three different settings that need various levels of data or concept removal in CBMs: concept-label-level, concept-level, and data-level. To the best of our knowledge, our research marks the first exploration of data removal issues within CBMs.
    \item To make CBMs able to remove data or concept influence without retraining, 
    we propose the Editable Concept Bottleneck Models (ECBMs).  Our approach in ECBMs offers a mathematically rigorous closed-form approximation. Furthermore, to improve computational efficiency, we present streamlined versions integrating Eigenvalue-corrected Kronecker-Factored Approximate Curvature (EK-FAC). 
    \item To showcase the effectiveness and efficiency of our ECBMs, we conduct comprehensive experiments across various benchmark datasets to demonstrate our superior performance.
\end{itemize}

==> section/2_related_work.tex <==
\section{Related Work}\label{sec:related work}
\noindent{\bf Concept Bottleneck Models.}
CBM~\citep{koh2020concept} stands out as an innovative deep-learning approach for image classification and visual reasoning. It introduces a concept bottleneck layer into deep neural networks, enhancing model generalization and interpretability by learning specific concepts. However, CBM faces two primary challenges: its performance often lags behind that of original models lacking the concept bottleneck layer, attributed to incomplete information extraction from the original data to bottleneck features. Additionally, CBM relies on laborious dataset annotation. Researchers have explored solutions to these challenges. \citet{chauhan2023interactive} extend CBM into interactive prediction settings, introducing an interaction policy to determine which concepts to label, thereby improving final predictions. \citet{oikarinen2023label} address CBM limitations and propose a novel framework called Label-free CBM. This innovative approach enables the transformation of any neural network into an interpretable CBM without requiring labeled concept data, all while maintaining high accuracy. Post-hoc Concept Bottleneck models \citep{yuksekgonul2022post} can be applied to various neural networks without compromising model performance, preserving interpretability advantages. CBMs work on the image field also includes \rebuttal{the works of} \citet{havasi2022addressing},\citet{kim2023probabilistic},\citet{keser2023interpretable},\citet{sawada2022concept} and \citet{sheth2023auxiliary}. Despite many works on CBMs, we are the first to investigate the interactive influence between concepts through influence functions. Our research endeavors to bridge this gap by utilizing influence functions in CBMs, thereby deciphering the interaction of concept models and providing an adaptive solution to concept editing. For more related work, please refer to Appendix \ref{app:sec:more_related}.


%Influence function, initially a staple in robust statistics for linear regression estimation \cite{cook2000detection,cook1980characterizations}, has seen extensive adoption within machine learning since \cite{koh2017understanding}. \cite{koh2017understanding} was the first to introduce influence functions to the machine learning domain, employing linear approximation to trace model predictions. This technique proves invaluable for model debugging, even in non-convex scenarios, despite potentially challenging its theoretical foundations. Its versatility spans various applications, including detecting mislabeled data, interpreting models, addressing model bias, and facilitating machine unlearning tasks. 

%In the realm of machine unlearning tasks, certain studies concentrate on approximate unlearning by employing influence functions to trace the impact of unlearning when recalling a data sample and providing closed-form updates of model parameters. Notable works in this area encompass unlearning features and labels \cite{warnecke2021machine}, minimax unlearning \cite{liu2024certified}, forgetting a subset of image data for training deep neural networks \cite{golatkar2020eternal,golatkar2021mixed}, graph unlearning involving nodes, edges, and features, as well as unlearning unusable data from users in recommendation systems \cite{zhang2023recommendation}.
%Typical applications include mislabeled data detection \cite{koh2017understanding}, model interpretation \cite{kwon2023datainf,guo2021fastif,aamir2023interpreting,han2020explaining,basu2021influence}, model bias \cite{wang2019repairing,kong2021resolving,brunet2019understanding,chen2020multi}, and machine unlearning \cite{warnecke2021machine,wu2023gif,zhang2023recommendation,golatkar2021mixed,golatkar2020eternal}. 
%To speed up the inverse Hessian, \cite{kwon2023datainf} applies an iterative LiSSA method to compute inverse Hessian in influence function and applies it to the large models like Llama and stable-diffusion to identify the most influential fine-tuning examples and mislabeled data detection. \cite{guo2021fastif} propose FASTIF, which uses kNN to reduce candidate points and fast estimate the inverse Hessian-vector. Besides, for layer-wise interpretation, \cite{aamir2023interpreting} propose a bi-directional approach including influence function and Shapley values to interpret contribution to class prediction. \cite{han2020explaining} interpreting BERT for natural language predictions. \cite{basu2021influence} explored the successes and failures of the influence function in image classification. For model bias, reduce the disparate impact of a fixed classification model \cite{wang2019repairing}, relabel training samples \cite{kong2021resolving}, bias in word embedding \cite{brunet2019understanding}, track predictions from finetuned model to pertaining data\cite{chen2020multi}.

==> section/3_preliminary.tex <==
\section{Preliminaries}
\label{sec:preliminary}
\noindent{\bf Concept Bottleneck Models.} In this paper, we consider the original CBM, and we adopt the notations used by \citet{koh2020concept}. We consider a classification task with a concept set denoted as $\bm{c}=\{p_1, \cdots, p_k\}$ with each $p_i$ is a concept given by experts or LLMs, and a training dataset represented as $\mathcal{D} = \{ z_i\}_{i=1}^{n}$, where $z_i = (x_i, y_i, c_i)$. Here, for $i\in [n]$, $x_i\in \mathbb{R}^m$ represents the feature vector, $y_i\in \mathbb{R}^{d_z}$ denotes the label (with $d_z$ corresponding to the number of classes), and $c_i=(c_i^1, \cdots, c_i^k) \in \mathbb{R}^k$ represents the concept vector. In this context, $c_i^j$ represents the weight of the concept $p_j$. In CBMs, our goal is to learn two representations: one called concept predictor that transforms the input space to the concept space, denoted as $g: \mathbb{R}^m \to \mathbb{R}^k$, and another called label predictor that maps the concept space to the prediction space, denoted as $f: \mathbb{R}^k \to \mathbb{R}^{d_z}$. Usually, here the map $f$ is linear.  For each training sample $z_i = (x_i, y_i, c_i)$, we consider two empirical loss functions: one is from the input space to concept space, and the other is from concept space to output space:
\begin{align}
  & \label{eq:hatg} \hat{g} = %\argmin_g \sum_{j=1}^{k}  L_{C_j} = 
    \argmin_g \sum_{j=1}^k\sum_{i=1}^n L_{C}(g^j(x_i),c_i^j)=\argmin_g \sum_{j=1}^k\sum_{i=1}^n L_{C_j}(g(x_i),c_i), \\
  & \label{eq:hatf} \hat{f} = %\argmin_f \sum_{i=1}^{n} L_{Y} = 
    \argmin_f \sum_{i=1}^nL_{Y}(f(\hat{g}(x_i)), y_i)=\argmin_f \sum_{i=1}^nL_{Y_i}(f, \hat{g}),
\end{align}
where $g^j(x_i)$ is the $j$-th concept predictor with $x_i$, $L_{C}$ and $L_{Y}$ are loss functions\rebuttal{See the notation table in Appendix~\ref{tab:notation}.}. We treat $g$ as a collection of $k$ concept predictors and separate different columns as a vector $g^j(x_i)$ for simplicity. Furthermore, in this paper, we primarily focus on the scenarios where the label predictor $f$ is a linear transformation. %Actually, the neural network gets gg as a whole. Besides, the objective ˆf\hat{f} and ˆg\hat{g} are different in the following three settings.

For any input $x$, we aim to ensure that its predicted concept vector $\hat{c}=g(x)$ and prediction $\hat{y}=f(\hat{g}(x))$ are close to their underlying counterparts, thus capturing the essence of the original CBMs.

\noindent {\bf Influence function.} The influence function is a measure of the dependence of the estimator on the value of any one of the points in the sample. Consider a neural network $\hat{\theta}=\arg\min_\theta \sum_{i=1}^n \ell(z_i;\theta)$ with loss function $\ell$ and dataset $D=\{z_i\}_{i=1}^n$. If we remove a point $z_m$ from the training dataset, the parameters become $\hat{\theta}_{-z_m} = \arg\min_\theta \sum_{i\neq m} \ell(z_i; \theta)$. Influence function gives us an efficient approximation for $\hat{\theta}_{-z_m}$ by defining a response function as $\hat{\theta}_{\epsilon, -z_m} = \underset{\theta \in \Theta}{\operatorname{argmin}} \frac{1}{n} \sum_{i=1}^{n} L(z_{i} ; \theta) + \epsilon L(z_m ; \theta).$ Perform first-order Taylor expansion on the gradient of the objective function corresponding to the $\argmin$ process of the response function, we can obtain the influence function defined by 
\begin{equation*}
    \mathcal{I}_{\hat{\theta}} \left( z_m \right)\triangleq \left.\frac{\mathrm{d} {\hat{\theta}_{\epsilon,-z_m}} }{\mathrm{d}\epsilon}\right|_{\epsilon = 0} = -H^{-1}_{\hat{\theta}} \cdot \nabla_{\theta} \ell (z_m; {\hat{\theta}}),
\end{equation*}
which can evaluate the influence of $z_m$ on the parameters.
% Removing a point zmz_m, the model change is denoted as ˆθ−zm−ˆθ\hat{\theta}_{-z_m} - \hat{\theta}, where ˆθ−zm≜\argminθ∑i≠mℓ(zi,θ)\hat{\theta}_{-z_m} \triangleq \argmin_{\theta} \sum_{i \neq m}\ell\left(z_{i}, \theta\right). Influence function gives us an efficient approximation for ˆθ−zm−ˆθ\hat{\theta}_{-z_m} - \hat{\theta} by parameterizing the training set using the weight ϵ\epsilon assigned to the new sample and observing consequent changes in the optimal parameters ˆθ−zm(ϵ)=\argminθ∑i≠mℓ(zi,θ)+ϵ⋅ℓ(zm,θ)\hat{\theta}_{-z_m} (\epsilon)= \argmin_{\theta} \sum_{i\neq m}\ell (z_i, \theta) + \epsilon \cdot \ell(z_m, \theta).
% Subsequently, our focus shifts to elucidating the influence of the sample zmz_m on the parameter θ{\theta}. The response function is defined as the first-order Taylor approximation evaluated at ϵ=0\epsilon=0 to capture this effect, that is Iˆθ(zm)≜dˆθdϵ|ϵ=0=−H−1ˆθ⋅∇θℓ(zm,ˆθ)\mathcal{I}_{\hat{\theta}} \left( z_m \right)\triangleq \left.\frac{\mathrm{d} {\hat{\theta}} }{\mathrm{d}\epsilon}\right|_{\epsilon = 0} = -H^{-1}_{\hat{\theta}} \cdot \nabla_{\theta} \ell (z_m, {\hat{\theta}}),
% where H−1ˆθ=∇2θ∑ni=1ℓ(zi,ˆθ)H^{-1}_{{\hat{\theta}}} = \nabla^2_{\theta} \sum_{i=1}^n \ell(z_i, {\hat{\theta}}) is the Hessian matrix of the loss function on the original training dataset with respect to ˆθ{\hat{\theta}}.
% Then, a quadratic approximation is created for the empirical risk centered at ˆθ\hat{\theta}. By taking a single Newton step with a step length of 1, we can estimate the change in parameters resulting from the exclusion of zmz_m without the need to retrain the model. This estimation is obtained by computing ˆθ−zm−ˆθ≈−Iˆθ(zm)\hat{\theta}_{-z_m}-\hat{\theta} \approx-\mathcal{I}_{{\hat{\theta}}}(z_m). 
When the loss function $\ell$ is twice-differentiable and strongly convex in $\theta$, the Hessian $H_{{\hat{\theta}}}$ is positive definite and thus the influence function is well-defined.  For non-convex loss, \citet{bartlett1953approximate} proposed that the Hessian $H_{{\hat{\theta}}}$ can be replaced by $\hat{H} =G_{\hat{\theta}} + \lambda I$
where $G_{\hat{\theta}}$ is the Fisher information matrix defined by $n^{-1}\sum_{i = 1}^n \nabla_{\theta}\ell(z_i; \theta)\nabla_{\theta}\ell(z_i; \theta)^{\mathrm{T}}$, $\lambda$ is a small damping term used to ensure the positive definiteness of $\hat{H}$. We can employ the Eigenvalue-corrected Kronecker-Factored Approximate Curvature (EK-FAC) method to further accelerate the computation. See Appendix \ref{sec:further} for details. 

%We mainly consider three settings: concept label-level, concept-level, and data-level for editable CBMs, which corrects the wrong concept for one data point, removes or introduces some concept for all the data, removes or introduces a new data, respectively. And we want to understand the influence of editing the CBM in the above level and the edited model's behavior on a new test data point. Among the many metrics that can be used to describe a model's behaviour, in this study we focus on the model parameters and the results of the model's inference at the test data point.



==> section/4_method.tex <==
\section{Editable Concept Bottleneck Models}
\label{sec:method}
In this section, we introduce our EBCMs for the three settings mentioned in the introduction by leveraging the influence function. Specifically, for the concept-label level, we will calculate the influence of a set of data sample's different concept labels; for the concept level, we will calculate the influence of several concepts; for the data level, we will calculate the influence of several samples. 


\vspace{-7pt}
\subsection{Concept Label-level Editable CBM}
\vspace{-7pt}
In many cases, several data samples possess erroneous annotations for certain concepts, \rebuttal{yet} we may opt to preserve their other information, particularly considering the high cost associated with acquiring data in specific domains like medical imaging.
In such scenarios, it is common practice to correct such erroneous concepts instead of removing the whole data point from the dataset. Estimating the changes in the parameters of the retraining model holds significance in this context. 
We name this case as concept label-level editable CBM.
%we choose to correct such erroneous concepts instead of removing the whole data point from the dataset due to the expensive annotation for some medical data. We denote this concept of single concept label data level influence as a concept label-level influence.

Mathematically, we have a set of erroneous data $D_e$ and its associated index set $S_e\subseteq [n]\times [k]$ such that for each $(w, r)\in S_e$, we have $(x_w, y_w, c_w)\in D_e$ with $c_w^r$ is mislabeled and $\tilde{c}_w^r$ is its corrected concept label. Thus, our goal is to approximate the new CBM without retraining. The retrained concept predictor \rebuttal{and} label predictor will be represented in the following manner. 
%We denote the erroneous data as (xir,yir,cir){(x_{i_r},y_{i_r},c_{i_r})}, where ir∈Sr⊂{1,2,⋯,n}≜[n]i_r\in S_r \subset \{1,2,\cdots,n\}\triangleq [n]. For some data (xw,yw,cw)(x_w, y_w, c_w),  w∈Srw\in S_r, the rr-th concept is mislabeled as crwc_w^r, we correct it to crw′{c_w^r}^{\prime}. Then the retrained concept predictor ˆgcrw\hat{g}_{c^r_w} with the revised dataset becomes:
\begin{align}
    &   \hat{g}_{e} = \argmin_{g} \left[ \sum_{(i, j) \notin S_e} L_{C}\left(g^j(x_i),c_i^j\right) +\sum_{(i, j) \in S_e} L_{C}\left(g^j(x_i), \tilde{c}_i^j \right) \right], \label{concept-label:g} \\
 & \label{concept-label:f}
    \hat{f}_{e} = \argmin_{f} \sum_{i=1}^n L_{Y} \left(f\left(\hat{g}_{e}\left(x_i\right)\right), y_i\right). 
\end{align}
For simple neural networks, we can use the influence function approach directly to estimate the retrained model. However, for CBM architecture, if we intervene with the true concepts, the concept predictor $\hat{g}$ fluctuates to $\hat{g}_e$ accordingly. Observing that the input data of the label predictor is the output of the concept predictor, which is also changing. Therefore, we need to adopt a two-stage \rebuttal{editing} approach. Here we consider the influence function for \eqref{concept-label:g} and \eqref{concept-label:f} separately. We first edit the concept predictor from $\hat{g}$ to $\bar{g}_{e}$, and then edit from $\hat{f}$ to $\bar{f}_e$ based on our approximated concept predictor, by the following two theorems.
\begin{theorem}\label{th:concept-label:g}
The retrained concept predictor $\hat{g}_{e}$ defined by (\ref{concept-label:g}) can be approximated by: 
\begin{equation}
    \hat{g}_{e} \approx \bar{g}_{e}  \triangleq \hat{g} -H^{-1}_{\hat{g}}  \cdot \sum_{(w,r)\in S_e} \left(\nabla_{\hat{g}}L_C\left(\hat{g}^r(x_w),\tilde{c}_w^r\right) - \nabla_{\hat{g}}L_C\left(\hat{g}^r(x_w),c_w^r\right) \right),
\end{equation}
where $H_{\hat{g}} = \nabla^2_{\hat{g}}  \sum_{i,j}  L_{C}(\hat{g}^j(x_i),c_i^j)$ is the Hessian matrix of the loss function with respect to $\hat{g}$.
\end{theorem}

\begin{theorem}
The retrained label predictor $\hat{f}_{e}$ defined by \eqref{concept-label:f} can be approximated by: 
\begin{align*}
     \hat{f}_{e} &\approx  \bar{f}_{e}=\hat{f} + H^{-1}_{\hat{f}} \cdot \nabla_f \sum_{i=1}^n L_{Y_i} \left(   \hat{f}, \hat{g}
 \right) - H^{-1}_{\hat{f}} \cdot \nabla_f \sum_{i=1}^n  L_{Y_i} \left( \hat{f}, \bar{g}_{e} \right),
   \end{align*}
where $H_{\hat{f}} = \nabla^2_{\hat{f}}\sum_{i=1}^n L_{Y_i}(\hat{f}, \hat{g})$ is the Hessian matrix of the loss function with respect to $\hat{f}$, $L_{Y_i}(\hat{f},\hat{g}) \triangleq L_{Y}(\hat{f}(\hat{g}(x_i)), y_i)$, and $\bar{g}_{e}$ is given in Theorem \ref{th:concept-label:g}.
\end{theorem}

\noindent {\bf Difference with test-time intervention.} 
The ability to intervene in CBMs enables human users to interact with the model in the prediction process, for example, a medical expert can substitute the erroneous predicted concept value $\hat{c}$ directly, and then observe its effect on the final prediction $\hat{y}$. However, the fundamental flaws in the concept predictor have not been thoroughly rectified, and similar errors may persist when applied to new test data. While under the editable CBM framework, not only can test-time intervention be performed, but the concept predictor of the CBM can also undergo secondary editing based on the test data that repeatedly yields errors. This process extends the rectification from the data level to the model level.

%For example, if a doctor needs to remove some mislabeled concepts or introduce new ones, this poses a challenge as modifying one concept disrupts the entire training dataset.
\subsection{Concept-level Editable CBM}
In this case, a set of concepts is removed due to incorrect attribution or spurious concepts, termed concept-level edit. \footnote{For convenience, in this paper, we only consider concept removal; our method can directly extend to concept insertion.}Specifically, for the concept set, denote the erroneous concept index set as $M\subset [k]$, we aim to delete these concept labels in all training samples. We aim to investigate the impact of updating the concept set within the training data on the model's predictions.  
It is notable that compared to the above concept label case,  the dimension of output (input) of the retrained concept predictor (label predictor) will change. If we delete $t$ concepts from the dataset, then ${g}$ becomes ${g}^{\prime}:\mathbb{R}^{m}\rightarrow\mathbb{R}^{k-t}$ and ${f}$ becomes ${f}^{\prime}:\mathbb{R}^{k-t}\rightarrow\mathbb{R}^{d_z}$.
More specifically, if we retrain the CBM with the revised dataset, the corresponding concept predictor becomes:
\begin{equation}\label{concept-level:g}
\hat{g}_{-p_M} = \argmin_{g^{\prime}}\sum_{j\notin M}  L_{C_j} = \argmin_{g'} \sum_{j\notin M}\sum_{i=1}^n L_{C}({g'}^j(x_i),c_i^j). 
\end{equation}
The variation of the parameters in dimension renders the application of influence function-based editing challenging for the concept predictor. This is because the influence function implements the editorial predictor by approximate parameter change from the original base after $\epsilon$-weighting the corresponding loss for a given sample, and thus, it is unable to deal with changes in parameter dimensions.

To overcome the challenge, our strategy is to develop some transformations that need to be performed on $\hat{g}_{-p_M}$ to align its dimension with $\hat{g}$ so that we can apply the influence function to edit the CBM. We achieve this by mapping $\hat{g}_{-p_M}$ to $\hat{g}^{*}_{-p_M} \triangleq \mathrm{P}(\hat{g}_{-p_M})$, which has the same amount of parameters as $\hat{g}$ and has the same predicted concepts $\hat{g}^{*}_{-p_M}(j)$ as $\hat{g}_{-p_M}(j)$ for all $j\in [k]-M$. We achieve this effect by inserting a zero row vector into the $r$-th row of the matrix in the final layer of $\hat{g}_{-p_M}$ for $r\in M$. Thus, we can see that the mapping $P$ is one-to-one. Moreover, assume the parameter space of $\hat{g}$ is $T$ and that of $\hat{g}^{*}_{-p_M}$, $T_0$ is \rebuttal{the subset of} $T$. Noting that $\hat{g}^{*}_{-p_M}$ is the optimal model of the following objective function:
\begin{equation}\label{concept-level:g^*}
\hat{g}^{*}_{-p_M} = \argmin_{g^{\prime} \in T_0} \sum_{j \notin M}^{k} \sum_{i=1}^{n} L_{C_j} ( g'^{j}(x_i), c_i^j), 
\end{equation}
i.e., it is the optimal model of the concept predictor loss on the remaining concepts under the constraint $T_0$.  Now we can apply the influence function to edit $\hat{g}$ to approximate $\hat{g}^{*}_{-p_M}$ with the restriction on the value of 0 for rows indexed by MM with the last layer of the neural network, denoted as $\bar{g}^*_{-p_M}$. After that, we remove from $\bar{g}^*_{-p_M}$ the parameters initially inserted to fill in the dimensional difference, which always equals 0 because of the restriction we applied in the editing stage, thus approximating the true edited concept predictor $\hat{g}_{-p_M}$. We now detail the editing process from $\hat{g}$ to $\hat{g}^{*}_{-p_M}$ using the following theorem. 
\begin{theorem}\label{thm:4.3}
For the retrained concept predictor $\hat{g}_{-p_M}$ defined in \eqref{concept-level:g}, we map it to $\hat{g}^{*}_{-p_M}$ as \eqref{concept-level:g^*}. And we can edit the initial $\hat{g}$ to $\hat{g}^*_{-p_M}$ as:
%For dataset D\mathcal{D}, we delete pr,r∈Mp_r, r \in M for all training samples. The retrained concept predictor is defined by equation ref{concept-level:g}. We can edit the initial ˆg\hat{g} to a fixed equivalent version of ˆg−pM\hat{g}_{-p_M} denoted by ˆg∗−pM\hat{g}^*_{-p_M} as:
% \begin{equation*}
% \hat{g}^*_{-p_M} = \argmin_{g}\sum_{j\notin M}L_{C_j} = \argmin_{g} \sum_{j\notin M}\sum_{i=1}^n L_{C_j}({g}^j(x_i),c_i^j),
% \end{equation*}
\begin{equation*}
    \hat{g}^*_{-p_M} \approx \bar{g}^*_{-p_M}\triangleq \hat{g}  - H^{-1}_{\hat{g}} \cdot \nabla_{\hat{g}} \sum_{j\notin M} \sum_{i=1}^{n} L_{C_j} ( \hat{g} (x_i), c_i),
\end{equation*}
where $H_{\hat{g}} = \nabla^2_{g} \sum_{j\notin M} \sum_{i=1}^{n} L_{C_j} ( \hat{g} (x_i), c_i)$.
Then, by removing all zero rows inserted during the mapping phase, we can naturally approximate $\hat{g}_{-p_M}\approx  \mathrm{P}^{-1}(\hat{g}^{*}_{-p_M})$.
\end{theorem}


For the second stage of training, assume we aim to remove concept $p_r$ for $r\in M$ and the new optimal model is $\hat{f}_{-p_M}$.
% defined by:
% \begin{equation}
% \hat{f}_{-p_M}=\argmin_{f^{\prime}\in\Theta^{\prime}} \sum_{i=1}^{n} L_{Y}=\argmin_{f'\in\Theta^{\prime}}\sum_{i=1}^{n} \ell(f^{\prime}(\hat{g}_{-p_M}(x_{i})), y_{i}).
% \end{equation}
We will encounter the same difficulty as in the first stage, i.e., the number of parameters of the label predictor will change. To address the issue, our key observation is that in the existing literature on CBMs, we always use linear transformation for the label predictor, meaning that the dimensions of the input with values of $0$ will have no contribution to the final prediction. 
To leverage this property, we fill the missing values in the input of the updated predictor with $0$, that is, replacing $\hat{g}_{-p_M}$ with $\hat{g}^*_{-p_M}$ and consider $\hat{f}_{p_M = 0}$ defined by
\begin{equation}\label{concept-level:f^*}
    \hat{f}_{p_M=0} = \argmin_{f} \sum_{i = 1}^n L_{Y_i} \left(f, \hat{g}^*_{-p_M}\right).
\end{equation}
%If we set the rr-th concept to zero for r∈Mr\in M and train again, we obtain another optimal model ˆf∗pM=0\hat{f}_{p_M=0}^*. Compared with ˆf−pM\hat{f}_{-p_M}, ˆfpM=0\hat{f}_{p_M = 0} has the same input in the rr-th dimension, r∈[k]−Mr\in[k]-M, and has 00 as input in dimension index in MM.
In total, we have the following lemma:
\begin{lemma}\label{method:lm:1}
In the CBM, \rebuttal{if} the label predictor utilizes linear transformations of the form $\hat{f} \cdot c$ with input $c$, \rebuttal{then, for each $r\in M$,} we remove the $r$-th concept from c and denote the new input as $c^{\prime}$; set the $r$-th concept to $0$ and denote the new input as $c^0$. Then we have $\hat{f}_{-p_M} \cdot c^{\prime} = \hat{f}_{p_M=0} \cdot c^0$ for any input $c$. 
\end{lemma}
Lemma \ref{method:lm:1} demonstrates that the retrained $\hat{f}_{-p_M}$ and $\hat{f}_{p_M=0}$, when given inputs $\hat{g}_{-p_M}(x)$ and $\hat{g}^*_{-p_M}(x)$ respectively, yield identical outputs. Consequently, we can utilize $\hat{f}_{p_M=0}$ as the editing target in place of $\hat{f}_{-p_M}$.
\begin{theorem}
For the revised retrained label predictor $\hat{f}_{p_M=0}$ defined by \eqref{concept-level:f^*}, we can edit the initial label predictor $\hat{f}$ to $\bar{f}_{p_M=0}$ by the following equation as a substitute for $\hat{f}_{p_M=0}$:
\begin{equation*}
    \hat{f}_{p_M=0} \approx \bar{f}_{p_M=0} \triangleq\hat{f}-H_{\hat{f}}^{-1} \cdot   \nabla_{\hat{f}} \sum_{l=1}^{n} L_{Y_l} \left( \hat{f}, \bar{g}^*_{-p_M} \right), 
\end{equation*}
where $H_{\hat{f}} = \nabla^2_{\hat{f}}\sum_{i=1}^n L_{Y_i}(\hat{f}, \hat{g})$. Deleting the $r$-th dimension of $\bar{f}_{p_M=0}$ for $r\in M$, then we can map it to $\bar{f}_{-p_M}$, which is the approximation of the final edited label predictor $\hat{f}_{-p_M}$ under concept level.
\end{theorem}

\subsection{Data-level Editable CBM}
In this scenario, we are more concerned about fully removing the influence of data samples on CBMs due to different reasons, such as the training data involving poisoned or erroneous issues. Specifically, we have a set of samples to be removed $\{(x_i, y_i, c_i)\}_{i\in G}$ with $G\subset [n]$. Then, we define the retrained concept predictor as
\begin{equation}\label{data-level:defg}
    \hat{g}_{-z_G} = \argmin_{g}\sum_{j=1}^k\sum_{i\in [n]-G}L_{C_j}(g(x_i), c_i)
\end{equation}
which can be evaluated by the following theorem:
\begin{theorem}\label{data-level:g}
For dataset $\mathcal{D} = \{ (x_i, y_i, c_i) \}_{i=1}^{n}$, given a set of data $z_r = (x_r, y_r, c_r)$, $r\in G$ to be removed. Suppose the updated concept predictor $\hat{g}_{-z_G}$ is defined by \eqref{data-level:defg}, then we have the following approximation for $\hat{g}_{-z_G}$
\begin{equation}
\hat{g}_{-z_G} \approx \bar{g}_{-z_G} \triangleq\hat{g} + H^{-1}_{\hat{g}} \cdot \sum_{r\in G}\nabla_{g} L_{C_r} (\hat{g}(x_r), c_r), 
\end{equation}
where $H_{\hat{g}} = \nabla^2_{\hat{g}}  \sum_{i,j}  L_{C_j}(\hat{g}^j(x_i),c_i^j)$ is the Hessian matrix of the loss function \rebuttal{with} respect to $\hat{g}$.
\end{theorem}

Based on $\hat{g}_{-z_G}$, the label predictor becomes $\hat{f}_{-z_G}$ which is defined by 
\begin{equation}\label{data-level:f}
    \hat{f}_{-z_G} = \argmin_{f}\sum_{i\in [n]-G} L_{Y_i}(f, \hat{g}_{-z_G}).
\end{equation}
%Noting that we do not know the specific value of the parameters in ˆg−zG\hat{g}_{-z_G}, we employ theorem  to approximate it actually. And the retrained label predictor is replaced by  
%ˆf−zG=\argminf∑i∈[n]−GLYi(f,ˉg−zG)\hat{f}_{-z_G} = \argmin_{f}\sum_{i\in [n]-G} L_{Y_i}(f, \bar{g}_{-z_G})
Compared with the original loss before unlearning 
in \eqref{eq:hatf}, we can observe two changes in \eqref{data-level:f}. First, we remove $|G|$ data points in the loss function $L_Y$. Secondly,  the input for the loss is also changed from $\hat{g}(x_i)$ to $\hat{g}_{-z_G}$. Therefore, it is difficult to estimate directly with an influence function. Here we introduce an intermediate label predictor as 
\begin{equation}\label{data-levl:tilde-f}
    \Tilde{f}_{-z_G} = \argmin \sum_{i\in [n]-G} L_{Y_i}(f, \hat{g}),
\end{equation}
and split the estimate of $\hat{f}_{-z_G}-\hat{f}$ into $\hat{f}_{-z_G}- \Tilde{f}_{-z_G}$ and $\Tilde{f}_{-z_G} - \hat{f}$. 
%The following result gives us the estimate for each term. 
\begin{theorem}\label{thm:data-level:f}
For dataset $\mathcal{D} = \{ (x_i, y_i, c_i) \}_{i=1}^{n}$, given a set of data $z_r = (x_r, y_r, c_r)$, $r\in G$ to be removed. The intermediate label predictor $\Tilde{f}_{-z_G}$ is defined in \eqref{data-levl:tilde-f}. Then we have
\begin{equation*}
%\label{method:approx:f_piao}
\Tilde{f}_{ -z_G} -\hat{f}  \approx H^{-1}_{\hat{f}} \cdot \sum_{i\in[n]-G}\nabla_{\hat{f}}L_{Y_i}(\hat{f},\hat{g}) \triangleq A_G.
\end{equation*}
We denote the edited version of $\Tilde{f}_{-z_G}$ as $\bar{f}^*_{-z_G} \triangleq \hat{f} + A_G$. 
Define $B_G$ as
\begin{equation*}
\hat{f}_{-z_G}-\Tilde{f}_{-z_G}\approx  -H^{-1}_{\bar{f}^*_{-z_G}} \cdot \nabla_{\hat{f}} \sum_{i\in [n]-G}\left(L_{Y_i} \left(\bar{f}^*_{-z_G}, \bar{g}_{-z_G}\right) - L_{Y_i} \left( \bar{f}^*_{-z_G}, \hat{g}\right)\right) \triangleq B_G,
\end{equation*}
where $H_{\bar{f}^*_{-z_G}} = \nabla_{\bar{f}}\sum_{i\in[n]-G}L_{Y_i}\left(  \bar{f}^*_{-z_G}, \hat{g}\right)$ is the Hessian matrix concerning $\bar{f}^*_{-z_G}$. 
Combining the above two-stage approximation, then, the final edited label predictor $\bar{f}_{-z_G}$ can be obtained by
\begin{equation}
    \bar{f}_{-z_G} = \bar{f}^*_{-z_G} + B_G = \hat{f} + A_G + B_G. 
\end{equation}
\end{theorem}
% \begin{equation}\label{method:approx:hat_f}
% \begin{split}
%  \hat{f}_{-z_G} - \Tilde{f}_{-z_G}\approx & -H^{-1}_{\bar{f}^*_{-z_G}} \cdot \left(\nabla_{\hat{f}} \sum_{i\in [n]-G}L_{Y_i} \left(\bar{f}^*_{-z_G}, \bar{g}_{-z_G}\right) -\nabla_{\hat{f}} \sum_{i\in [n]-G} L_{Y_i} \left( \bar{f}^*_{-z_G}, \hat{g}\right)\right)
%  \triangleq B_G, 
% \end{split}
% \end{equation}
%\approx & -H^{-1}_{\Tilde{f}_{-z_G}} \cdot \nabla_{\hat{f}} \sum_{i\in [n]-G}L_{Y_i} \left(\Tilde{f}_{-z_G}, \hat{g}_{-z_G}\right) + H^{-1}_{\Tilde{f}_{-z_G}} \cdot\nabla_{\hat{f}} \sum_{i\in [n]-G} L_{Y_i} \left(  \Tilde{f}_{-z_G}, \hat{g}\right)\\
%where Hˉf∗−zG=∇ˉf∑i∈[n]−GLYi(ˉf∗−zG,ˆg)H_{\bar{f}^*_{-z_G}} = \nabla_{\bar{f}}\sum_{i\in[n]-G}L_{Y_i}\left(  \bar{f}^*_{-z_G}, \hat{g}\right) is the Hessian matrix of the loss function on the intermediate dataset concerning \Tildef−zG\Tilde{f}_{-z_G}. 
%Observing that the computational complexity of this matrix is quite high. And we will estimate it using an optimization method in the theorem below. 
%Besides, we denote this approximation as BGB_G. 
\noindent {\bf Acceleration via EK-FAC.} As we mentioned in Section \ref{sec:preliminary}, as the loss function in CBMs is non-convex, the Hessian matrices in all our theorems may not be well-defined. We can use the EK-FAC approach, i.e., using $\hat{H}_{\theta} =G_{\theta} + \lambda I$ to approximate the Hessian, 
where $G_{\theta}$ is the Fisher information matrix of model ${\theta}$, and $\lambda$ is a small damping term used to ensure the positive definiteness. See Appendix \ref{sec:FAC_CBM} for using EK-FAC to CBMs. Also, see Algorithm \ref{alg:4}-\ref{alg:6} in the Appendix for the detailed EK-FAC-based algorithms for our three levels, whose original (Hessian) versions are in  Algorithm \ref{alg:1}-\ref{alg:3}, respectively. 
% Based on theorem subscribe AGA_G into BGB_G and use two methods to accelerate the calculation of H\Tildef−zGH_{\Tilde{f}_{-z_G}} we have the following approximation for the data-level edited label predictor in CBM.
% \begin{theorem}
% For dataset D={(xi,yi,ci)}ni=1\mathcal{D} = \{ (x_i, y_i, c_i) \}_{i=1}^{n}, we delete a set of data zr=(xr,yr,cr)z_r = (x_r, y_r, c_r), r∈Gr\in G. Suppose the retrained label predictor ˆf−zG\hat{f}_{-z_G} is defined by . The intermediate label predictor is defined by equation  
% Then, we have the following approximation for ˆf−zG\hat{f}_{-z_G},
% \begin{align*}
%  \hat{f}_{-z_G} - \hat{f} \approx & A_G + B_G
% \end{align*}
% AGA_G and BGB_G is defined in lemma ?????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{lem:data-level:f}.
% \end{theorem}
% And there are these two methods to estimate H−1\Tildef−zGH^{-1}_{\Tilde{f}_{-z_G}} in BGB_G:
% \begin{equation*}
%   H_{\Tilde{f}_{-z_G}} = \frac{\|\nabla_{\hat{f}} \ell_r  \| }{\| H_{\hat{f}} \cdot \nabla_{\hat{f}} \ell_r \|} \cdot \left(I - 2 \cdot \frac{C\cdot \nabla_{\hat{f}} \ell_r \cdot {\nabla_{\hat{f}} \ell_r}^{\mathrm{T}} \cdot C }{{\nabla_{\hat{f}} \ell_r}^{\mathrm{T}} \cdot C^2 {\nabla_{\hat{f}} \ell_r}} \right)
% \end{equation*}
% \begin{equation*}
%     H_{\Tilde{f}_{-z_r}} = \nabla_{\hat{f}} \ell_r \cdot {\nabla_{\hat{f}} \ell_r}^{\mathrm{T}} \cdot \left( \nabla_{\hat{f}} \ell_r \cdot {\nabla_{\hat{f}} \ell_r}^{\mathrm{T}} + \alpha I \right) ^{-1} \cdot H_{\hat{f}}
% \end{equation*}

% \begin{align*}
%  \hat{f}_{-z_G} - \hat{f}
%   =& \underbrace{H^{-1}_{\Tilde{f}_{-z_G}} \cdot  \nabla_{\hat{f}} \sum_{i\in S}\ell \left(  \Tilde{f}_{-z_r}(\hat{g}_{-z_r}(x_{i})), y_{i}  \right)}_{A} - \underbrace{H^{-1}_{\Tilde{f}_{-z_r}} \cdot \nabla_{\hat{f}} \sum_{i\in S} \ell \left(  \Tilde{f}_{-z_r}(\hat{g}(x_{i})), y_{i}  \right)}_{B}  \\
% +& H^{-1}_{\hat{f}} \cdot \nabla_{\hat{f}}\ell \left(\hat{f} ( \hat{g} (x_r) ) , y_r   \right),
% \end{align*}
% where
% \begin{align*}
% A = & H^{-1}_{\Tilde{f}_{-z_r}} \cdot \left[ \nabla_{\hat{f}} \sum_{i\in S}\ell \left(  \hat{f}\left(\hat{g}(x_{i}) + {x_{i}}^{\mathrm{T}}\cdot H^{-1}_{\hat{g}} \cdot \nabla_{g} \ell (\hat{g}(x_r), c_r)  \right) \right.\right.\\ 
% + &\left.\left.  \left( \hat{g}(x_{i}) + x_{i}^{\mathrm{T}}\cdot H^{-1}_{\hat{g}} \cdot \nabla_{g} \ell (\hat{g}(x_r), c_r) \right)^{\mathrm{T}}\cdot H^{-1}_{\hat{f}} \cdot \nabla_{\hat{f}}\ell \left(\hat{f} ( \hat{g} (x_r) ) , y_r\right), y_{i}\right)\right].
% \end{align*}
% \begin{align*}
% B = & H^{-1}_{\Tilde{f}_{-z_r}} \cdot  \nabla_{\hat{f}} \left [ \sum_{i\in S}\ell \left(  \hat{f}\left(\hat{g}(x_{i})\right ) + (\hat{g}(x_{i}))^{\mathrm{T}}\cdot H^{-1}_{\hat{f}} \cdot \nabla_{\hat{f}}\ell \left(\hat{f} ( \hat{g} (x_r) ) , y_r   \right), y_{i}\right)\right].
% \end{align*}

%For simplicity, we consider setting pM=0p_M=0 for all data points and get another optimal model ˆfpM=0\hat{f}_{p_M=0}, which has the same dimension of parameters as ˆf\hat{f}. Then, derived from the linearity of ff, this predictor is equivalent to ˆf−pM\hat{f}_{-p_M}. 
%Then, for the label predicting stage, the following is equivalent.


%To address this problem, let us first consider the second stage of training. Assume we remove concept prp_r and retrain again to get a new optimal model ˆf−pM\hat{f}_{-p_M}. For simplicity, we consider setting pM=0p_M=0 for all data points and get another optimal model ˆfpM=0\hat{f}_{p_M=0}, which has the same dimension of parameters as ˆf\hat{f}. Then, derived from the linearity of ff, this predictor is equivalent to ˆf−pM\hat{f}_{-p_M}. 
%On the other hand, we project ˆg\hat{g} to P(ˆg)=ˆg∗−pM\mathrm{P}(\hat{g}) = \hat{g}^{*}_{-p_M}, which has the same amount of parameters as ˆg\hat{g} and have the same predicted concepts ˆg∗j−pM\hat{g}^{*j}_{-p_M}, as ˆgj−pM\hat{g}^{j}_{-p_M}, where j∈[k]−Mj\in [k]-M. We achieve this effect by inserting a zero row vector into the rr-th row of the matrix in the final layer of ˆg−pM\hat{g}_{-p_M} for r∈Mr\in M. Then, for the label predicting stage, the following is equivalent.
% \begin{equation*}
% \hat{f}_{p_M=0}=\argmin_{f} \sum_{i=1}^{n} L_{Y}\left(f,\hat{g}_{-p_r}^{*}\right).
% \end{equation*}
% \begin{equation*}
% \hat{f}_{-p_r}=\argmin_{f^{\prime}} \sum_{i=1}^{n} L_{Y ;_i} \left(f^{\prime}, \hat{g}_{-p_r}\right).
% \end{equation*}
























% We design the influence function under three scenarios for editable CBM: 
% \begin{enumerate}
%     \item Concept label-level. In some cases, if several data sample (xir,yir,cir){(x_{i_r},y_{i_r},c_{i_r})} possesses erroneous annotations for certain concept pr∈cip_r \in c_i, we choose to delete such erroneous pr∈cip_r \in c_i due to the expensive annotation for some medical data. We denote this concept of single data level influence as a single-level influence.
%     \item Concept-level Editable CBM. In this case, one concept is removed due to incorrect attribution, termed concept-level influence. Specifically, for dataset D={(xi,yi,ci)}Ni=1\mathcal{D} = \{ (x_i, y_i, c_i) \}_{i=1}^{N}, we delete pr∈\bmcp_r \in \bm{c} for all training samples {(xi,yi,ci)}Ni=1\{ (x_i, y_i, c_i) \}_{i=1}^{N}.
%     \item Data-level Editable CBM. In this case, we address situations where a data sample (xi,yi,ci)(x_i,y_i,c_i) possesses erroneous annotations for certain concepts. We choose to remove such data, referred to as data-level influence, i.e., for such sample (xi,yi,ci)(x_i, y_i, c_i), pr∈cip_r \in c_i is erroneous, then, we remove the data (xi,yi,ci)(x_i, y_i, c_i).
% \end{enumerate}
% \subsection{Concept Label-level Influence}
% In instances where only one concept of a particular data is mislabeled, we may opt to preserve its other information, particularly considering the high cost associated with acquiring data in specific domains like medical imaging. In such scenarios, it is common practice to set the value of 0 to this mislabeled concept. Estimating the changes in the parameters of the retraining model holds significance in this context.

% Assume the rr-th concept of the ww-th data is wrong, then the retrained concept predictor ˆgcrw\hat{g}_{c^r_w} with crwc^r_w corrected to crw′{c_w^r}^{\prime} are changed to:
% \begin{equation}\label{concept-label:g}
%        \hat{g}_{c^r_w} = \argmin \left[\sum_{(i, j)\neq(w, r)} L_{C_j}\left(g^j(x_i),c_i^j\right) +L_{C_j}\left(g^r(x_w),{c_w^r}^{\prime} \right)\right],
% \end{equation}
% Then, without the need of retraining the model, the following theorem deduces an approximation for ˆgcrw\hat{g}_{c^r_w}.
% \begin{theorem}
% On the other hand, the retrained concept predictor ˆgcrw\hat{g}_{c^r_w} defined by equation ???????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{concept-label:g} can be approximated by: 
% \begin{equation}
%     \hat{g}_{c^r_w} \triangleq \bar{g}_{c^r_w}\approx   \hat{g} -H^{-1}_{\hat{g}}  \cdot  \left(\nabla_{\hat{g}}\ell\left(\hat{g}^r(x_w),{c_w^r}^{\prime}\right) - \nabla_{\hat{g}}\ell\left(\hat{g}^r(x_w),c_w^r\right) \right),
% \end{equation}
% where Hˆg=∇2ˆg∑i,jLCj(ˆgj(xi),cji)H_{\hat{g}} = \nabla^2_{\hat{g}}  \sum_{i,j}  L_{C_j}\left(\hat{g}^j(x_i),c_i^j\right) is the Hessian matrix of the loss function respect to ˆg\hat{g}.
% \end{theorem}
% The retrained label predictor accordingly defined by
% \begin{equation}\label{concept-label:f}
%     \hat{f}_{c^r_w} = \argmin \sum_{i=1}^n L_{Y} \left(f\left(\hat{g}_{c^r_w}\left(x_i\right)\right), y_i\right)
% \end{equation}
% We can see that all the sample in the training set has changed, we need the retrained concept model to evaluate, however, theorem ?????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{th:concept-label:g} enables us to estimate the change exactly.
% \begin{theorem}
% The retrained label predictor ˆfcrw\hat{f}_{c^r_w} defined by equation ????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{concept-label:f} can be approximated by: 
% \begin{align*}
%      \hat{f}_{c_w^r} &= \hat{f} + H^{-1}_{\hat{f}} \cdot \nabla_f \sum_{i=1}^n L_Y \left(   \hat{f} \left( \hat{g} ( x_{i} ) 
%  \right) , y_{i} \right) - H^{-1}_{\hat{f}} \cdot \nabla_f \sum_{l=1}^n \left( L_Y \left( \hat{f} \left( \bar{g}_{c^r_w}(x_l) \right) , y_{l} \right) \right).
%    \end{align*}
% Where H−1ˆf=∇2ˆf∑ni=1LY(ˆf(ˆg(xi)),yi)H^{-1}_{\hat{f}} = \nabla^2_{\hat{f}}\sum_{i=1}^n L_Y\left(\hat{f}\left(\hat{g}\left(x_i\right)\right), y_i\right) is the Hessian matrix of the loss function respect to ˆf\hat{f}, ˉgcrw\bar{g}_{c^r_w} is given in theorem ????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{th:concept-label:g}.
% \end{theorem}

% \paragraph{Discussion:} Difference with test-time intervention.

% \subsection{Concept-level Influence}
% Our goal is to investigate the impact of updating the concept set within the training data on the model's predictions. For example, if a doctor needs to remove a mislabeled concept or introduce a new one, this poses a challenge as modifying one concept disrupts the entire training dataset. Let us consider the influence of model parameters by removing a concept prp_r from the training set. That is, if we retrain the CBM with the revised dataset, corresponding predictors become:
% \begin{equation}
% \hat{g}_{-p_r} = \argmin_{g^{\prime}}\sum_{j=1, j\neq r}^{k}  L_{C_j} = \argmin_{g'} \sum_{j=1, j \neq r}^k\sum_{i=1}^n \ell({g'}^j(x_i),c_i^j),
% \end{equation}
% \begin{equation}
% \hat{f}_{-p_r}=\argmin_{f^{\prime}} \sum_{i=1}^{n} L_{Y}=\argmin_{f'} \sum_{i=1}^{n} \ell(f^{\prime}(\hat{g}_{-p_r}(x_{i})), y_{i}).
% \end{equation}
% % However, retraining the model is costly and is not practical. We need a computing-efficient method to quantify changes in parameters. Let us re-consider the concept bottleneck models. In CBMs, our goal is to learn two representations: one that transforms the input space to the concept space, denoted as g:Rd→Rkg: \mathbb{R}^d \to \mathbb{R}^k, and another that maps the concept space to the prediction space, denoted as f:Rk→Rdzf: \mathbb{R}^k \to \mathbb{R}^{d_z}. By the way, if we remove the prp_r concept from all the data, the output dimension of gg and the input dimension of ff will decrease to k−1k-1. 
% % To address this problem, let us first consider the second stage of training. Assume we remove concept prp_r and retrain again to get a new optimal model ˆf−pr\hat{f}_{-p_r}. For simplicity, we consider setting pr=0p_r=0 for all data points and get another optimal model ˆfpr=0\hat{f}_{p_r=0}, which has the same dimension of parameters as ˆf\hat{f}. Then, derived from the linearity of ff, this predictor is equivalent to ˆf−pr\hat{f}_{-p_r}. On the other hand, we project ˆg\hat{g} to P(ˆg)=ˆg∗−pr\mathrm{P}(\hat{g}) = \hat{g}^{*}_{-p_r}, which has the same amount of parameters as ˆg\hat{g} and have the same predicted concepts ˆg∗j−pr\hat{g}^{*j}_{-p_r}, as ˆgj−pr\hat{g}^{j}_{-p_r}, where j=1,⋯,r−1,r+1,⋯,kj=1,\cdots,r-1,r+1,\cdots,k. We achieve this effect by inserting a zero row vector into the rr-th row of the matrix in the final layer of ˆg−pr\hat{g}_{-p_r}. Then, for the label predicting stage, the following is equivalent.
% \begin{equation*}
% \hat{f}_{p_r=0}=\argmin_{f} \sum_{i=1}^{n} \ell\left(f\left(\hat{g}_{-p_r}^{*}\left(x_{i}\right), y_{i}\right)\right).
% \end{equation*}
% \begin{equation*}
% \hat{f}_{-p_r}=\argmin_{f^{\prime}} \sum_{i=1}^{n} \ell \left(f^{\prime} \left(\hat{g}_{-p_r}\left(x_{i}\right), y_{i}\right)\right).
% \end{equation*}
% \begin{theorem}
% For dataset D={(xi,yi,ci)}Ni=1\mathcal{D} = \{ (x_i, y_i, c_i) \}_{i=1}^{N}, we delete pr∈\bmcp_r \in \bm{c} for all training samples {(xi,yi,ci)}Ni=1\{ (x_i, y_i, c_i) \}_{i=1}^{N}. Suppose the concept predictor ˆg\hat{g} is defined by equation ????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{eq:hatg}. Denote ˆg−pr\hat{g}_{-p_r} as the the updated ˆg\hat{g} under this scenario. If we define ˆg−pr\hat{g}_{-p_r} as
% \begin{equation*}
% \hat{g}_{-p_r} = \argmin_{g^{\prime}}\sum_{j=1, j\neq r}^{k}  L_{C_j} = \argmin_{g'} \sum_{j=1, j \neq r}^k\sum_{i=1}^n \ell({g'}^j(x_i),c_i^j),
% \end{equation*}
% Then, we define an equivalent concept predictor ˆg∗−pr\hat{g}^*_{-p_r} and have the following approximation for ˆg∗−pr\hat{g}^*_{-p_r}, 
% \begin{equation*}
%     \hat{g}^*_{-p_r} \approx \hat{g}  - H^{-1}_{\hat{g}} \cdot \nabla_{\hat{g}} \sum_{j=1, j \neq r}^{k} \sum_{i=1}^{n} \ell ( \hat{g}^{j} (x_i), c
%     ^j_i),
% \end{equation*}
% where Hˆg=∇2g∑kj=1,j≠r∑ni=1ℓ(ˆgj(xi),cji)H_{\hat{g}} = \nabla^2_{g} \sum_{j=1, j \neq r}^{k} \sum_{i=1}^{n} \ell ( \hat{g}^{j} (x_i), c^j_i).
% \end{theorem}


% \begin{theorem}
% For dataset D={(xi,yi,ci)}Ni=1\mathcal{D} = \{ (x_i, y_i, c_i) \}_{i=1}^{N}, we delete pr∈\bmcp_r \in \bm{c} for all training samples {(xi,yi,ci)}Ni=1\{ (x_i, y_i, c_i) \}_{i=1}^{N}. Suppose the label predictor ˆf\hat{f} is defined by equation ???????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{eq:hatf}. Denote ˆf−pr\hat{f}_{-p_r} as the the updated ˆf\hat{f} under this scenario. If we define ˆf−pr\hat{f}_{-p_r} as
% \begin{equation*}
% \hat{f}_{-p_r}=\argmin_{f^{\prime}} \sum_{i=1}^{n} L_{Y}=\argmin_{f'} \sum_{i=1}^{n} \ell(f^{\prime}(\hat{g}_{-p_r}(x_{i})), y_{i}),
% \end{equation*}
% Then, we have the following approximation for ˆf−pr\hat{f}_{-p_r}, 
% \begin{equation*}
%     \hat{f}_{-p_r} \approx \hat{f}-H_{\hat{f}}^{-1} \cdot   \nabla_{\hat{f}} \sum_{l=1}^{n} \ell \left( \hat{f} \left( \hat{g} (x_l) - x_l^{\mathrm{T}} \cdot H^{-1}_{\hat{g}} \cdot \nabla_{\hat{g}} \sum_{j=1, j \neq r}^{k} \sum_{i=1}^{n} \ell ( \hat{g}^{j} (x_i), c^j_i) \right)  , y_l \right).
% \end{equation*}
% \end{theorem}



% \subsection{Data-level Influence}
% In practical application scenarios, if we find that a certain data zr=(xr,yr,cr)z_r = (x_r, y_r, c_r) has information that is wrong, the usual practice is that we will choose to remove this data, and ˆf\hat{f} and ˆg\hat{g} accordingly become: 
% \begin{equation}
%     \hat{g}_{-z_r} = \argmin_{g}\sum_{\substack{i=1, i \neq r}}^{n} \ell(\hat{g}(x_{i}), c_{i})
% \end{equation}
% \begin{equation}
%     \hat{f}_{-z_r} = \argmin_{f}\sum_{\substack{i=1, i \neq r}}^{n} \ell(f\left(\hat{g}_{-z_r}(x_{i})\right), y_{i})
% \end{equation}

% \begin{theorem}
% For dataset D={(xi,yi,ci)}Ni=1\mathcal{D} = \{ (x_i, y_i, c_i) \}_{i=1}^{N}, we delete one sample zr=(xr,yr,cr)z_r = (x_r, y_r, c_r). Suppose the concept predictor ˆg\hat{g} is defined by equation ???????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{eq:hatg}. Denote ˆg−zr\hat{g}_{-z_r} as the the updated ˆg\hat{g} under this scenario. If we define ˆg−zr\hat{g}_{-z_r} as
% \begin{equation*}
%     \hat{g}_{-z_r} = \argmin_{g}\sum_{\substack{i=1, i \neq r}}^{n} \ell(g(x_{i}), c_{i}),
% \end{equation*}
% Then, we have the following approximation for ˆg−zr\hat{g}_{-z_r}, 
% \begin{equation}
% \hat{g}_{-z_r} \approx \hat{g} + H^{-1}_{\hat{g}} \cdot \nabla_{g} \ell (\hat{g}(x_r), c_r).
% \end{equation}
% \end{theorem}

% \begin{theorem}
% For dataset D={(xi,yi,ci)}Ni=1\mathcal{D} = \{ (x_i, y_i, c_i) \}_{i=1}^{N}, we delete one sample zr=(xr,yr,cr)z_r = (x_r, y_r, c_r). Suppose the label predictor ˆf\hat{f} is defined by equation ???????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{eq:hatf}. Denote ˆf−zr\hat{f}_{-z_r} as the the updated ˆf\hat{f} under this scenario. If we define ˆf−zr\hat{f}_{-z_r} as
% \begin{equation*}
%     \hat{f}_{-z_r} = \argmin_{f}\sum_{\substack{i=1, i \neq r}}^{n} \ell(f\left(\hat{g}_{-z_r}(x_{i})\right), y_{i}),
% \end{equation*}
% Then, we have the following approximation for ˆf−zr\hat{f}_{-z_r},
% \begin{align*}
%  \hat{f}_{-z_r} - \hat{f}
%   =& \underbrace{H^{-1}_{\Tilde{f}_{-z_r}} \cdot  \nabla_{\hat{f}} \sum_{i\in S}\ell \left(  \Tilde{f}_{-z_r}(\hat{g}_{-z_r}(x_{i})), y_{i}  \right)}_{A} - \underbrace{H^{-1}_{\Tilde{f}_{-z_r}} \cdot \nabla_{\hat{f}} \sum_{i\in S} \ell \left(  \Tilde{f}_{-z_r}(\hat{g}(x_{i})), y_{i}  \right)}_{B}  \\
% +& H^{-1}_{\hat{f}} \cdot \nabla_{\hat{f}}\ell \left(\hat{f} ( \hat{g} (x_r) ) , y_r   \right),
% \end{align*}
% where
% \begin{align*}
% A = & H^{-1}_{\Tilde{f}_{-z_r}} \cdot \left[ \nabla_{\hat{f}} \sum_{i\in S}\ell \left(  \hat{f}\left(\hat{g}(x_{i}) + {x_{i}}^{\mathrm{T}}\cdot H^{-1}_{\hat{g}} \cdot \nabla_{g} \ell (\hat{g}(x_r), c_r)  \right) \right.\right.\\ 
% + &\left.\left.  \left( \hat{g}(x_{i}) + x_{i}^{\mathrm{T}}\cdot H^{-1}_{\hat{g}} \cdot \nabla_{g} \ell (\hat{g}(x_r), c_r) \right)^{\mathrm{T}}\cdot H^{-1}_{\hat{f}} \cdot \nabla_{\hat{f}}\ell \left(\hat{f} ( \hat{g} (x_r) ) , y_r\right), y_{i}\right)\right].
% \end{align*}
% \begin{align*}
% B = & H^{-1}_{\Tilde{f}_{-z_r}} \cdot  \nabla_{\hat{f}} \left [ \sum_{i\in S}\ell \left(  \hat{f}\left(\hat{g}(x_{i})\right ) + (\hat{g}(x_{i}))^{\mathrm{T}}\cdot H^{-1}_{\hat{f}} \cdot \nabla_{\hat{f}}\ell \left(\hat{f} ( \hat{g} (x_r) ) , y_r   \right), y_{i}\right)\right].
% \end{align*}
% And there are these two methods to estimate H−1\Tildef−zrH^{-1}_{\Tilde{f}_{-z_r}}:
% \begin{equation*}
%   H_{\Tilde{f}_{-z_r}} = \frac{\|\nabla_{\hat{f}} \ell_r  \| }{\| H_{\hat{f}} \cdot \nabla_{\hat{f}} \ell_r \|} \cdot \left(I - 2 \cdot \frac{C\cdot \nabla_{\hat{f}} \ell_r \cdot {\nabla_{\hat{f}} \ell_r}^{\mathrm{T}} \cdot C }{{\nabla_{\hat{f}} \ell_r}^{\mathrm{T}} \cdot C^2 {\nabla_{\hat{f}} \ell_r}} \right)
% \end{equation*}
% \begin{equation*}
%     H_{\Tilde{f}_{-z_r}} = \nabla_{\hat{f}} \ell_r \cdot {\nabla_{\hat{f}} \ell_r}^{\mathrm{T}} \cdot \left( \nabla_{\hat{f}} \ell_r \cdot {\nabla_{\hat{f}} \ell_r}^{\mathrm{T}} + \alpha I \right) ^{-1} \cdot H_{\hat{f}}
% \end{equation*}
% \end{theorem}


==> section/5_experiment.tex <==
\section{Experiments}
\label{sec:exp}
In this section, we demonstrate our main experimental results on utility evaluation, edition efficiency, and interpretability evaluation. Details and additional results are in Appendix \ref{sec:appendix:exp} due to space limit.

\subsection{Experimental Settings}
\noindent{\bf Dataset.} We utilize three datasets: \textit{X-ray grading (OAI)}~\citep{nevitt2006osteoarthritis}, \textit{Bird identification (CUB)}~\citep{wah2011caltech} and \textit{Large-scale CelebFaces Attributes dataset (CelebA)}~\citep{liu2015deep}. OAI is a multi-center observational study of knee osteoarthritis, which comprises 36,369 data points. Specifically, we configure n=10 concepts that characterize crucial osteoarthritis indicators such as joint space narrowing, osteophytes, and calcification. Bird identification (CUB)\footnote{\rebuttal{The original dataset is processed. Detailed explanation can be found in \ref{sec:appendix:exp}.}} consists of 11,788 data points, which belong to 200 classes and include 112 binary attributes to describe detailed visual features of birds. CelebA comprises \rebuttal{202,599} celebrity images, each annotated with 40 binary attributes that detail facial features, such as hair color, eyeglasses, and smiling. As the dataset lacks predefined classification tasks, following~\cite{NEURIPS2022_867c0682}, we designate 8 attributes as labels and the remaining 32 attributes as concepts. For all the above datasets, we follow the same network architecture and settings outlined in~\cite{koh2020concept}.

\noindent{\bf \rebuttal{Ground Truth} and Baselines.} \rebuttal{We use retrain as the ground truth method.} \textit{Retrain}: We retrain the CBM from scratch by removing the samples, concept labels, or concepts from the training set. We employ two baseline methods: CBM-IF, and ECBM. \textit{CBM-IF}: This method is a direct implementation of our previous theorems of model updates in the three settings. See Algorithms \ref{alg:1}-\ref{alg:3} in Appendix for details. \textit{ECBM}:  
As we discussed above, all of our model updates can be further accelerated via EK-FAC, ECBM corresponds to the EK-FAC accelerated version of Algorithms \ref{alg:1}-\ref{alg:3}  (refer to Algorithms \ref{alg:4}-\ref{alg:6} in Appendix).
%including an accelerated version of data level CBM-IF
%\textit{IF}: Influence Function(IF) was originally designed for end-to-end models and is not suitable for all three levels of modification in CBMs. Thus, we choose to freeze the concept predictor network and apply IF to the label predictor. Notably, at the concept level, the output dimension change from deleting the concept predictor was resolved by setting the corresponding output to 00.

\noindent{\bf Evaluation Metric.} We utilize two primary evaluation metrics to assess our models: the F1 score and runtime (RT). The \textit{F1 score} measures the model's performance by balancing precision and recall. \textit{Runtime}, measured in seconds, evaluates the running time of each method to update the model.  

\noindent{\bf Implementation Details.} Our experiments utilized an Intel Xeon CPU and an RTX 3090 GPU. For utility evaluation, at the concept level, one concept was randomly removed for the OAI dataset and repeated while ten concepts were randomly removed for the CUB dataset, with five different seeds. At the data level, 3\% of the data points were randomly deleted and repeated 10 times with different seeds. At the concept-label level, we randomly selected 3\% of the data points and modified one  concept of each data randomly, repeating this 10 times for consistency across iterations. %Furthermore, in the study of editing multiple samples on the CUB dataset tested the resilience of ECBMs. We removed 1\% to 10\% of the concepts sequentially at the concept level and altered or deleted 1\% to 10\% of the data points at the concept-label level and data level in 1\% increments. \di{Rewirte the setting for these three settings}. Each setup was repeated ten times with different seeds. 


\subsection{Evaluation of Utility and Editing Efficiency}
Our experimental results, as illustrated in Table \ref{tab:results}, demonstrate the effectiveness of ECBMs compared to traditional retraining and CBM-IF, particularly emphasizing computational efficiency without compromising accuracy. Specifically, ECBMs achieved F1 scores close to those of retraining (0.8808 vs. 0.8825) while significantly reducing the runtime from 31.44 seconds to 8.29 seconds. This pattern is consistent in the CUB dataset, where the runtime was decreased from 27.88 seconds for retraining to 7.03 seconds for ECBMs, with a negligible difference in the F1 score (0.7971 to 0.7963). These results highlight the potential of ECBMs to provide substantial time savings—approximately 22-30\% of the computational time required for retraining—while maintaining comparable accuracy. Compared to CBM-IF, ECBM also showed a slight reduction in runtime and a significant improvement in F1 score. The former verifies the effective acceleration of our algorithm by EK-FAC. This efficiency is particularly crucial in scenarios where frequent updates to model annotations are needed, confirming the utility of ECBMs in dynamic environments where running time and accuracy are critical. 

We can also see that the original version of ECBM, i.e., CBM-IF, also has a lower runtime than retraining but a lower F1 score than ECBM. Such results may be due to different reasons. For example, 
our original theorems depend on the inverse of the Hessian matrices, which may not be well-defined for non-convex loss. Moreover, these Hessian matrices may be ill-conditioned or singular, which makes calculating their inverse imprecise and unstable.  

%Moreover, due to the excessively high computational complexity of the IHVP problem, we applied a linear approximation to the activation function, which can also lead to a decrease in the F1 score. 

\input{tabs/tab_t}

%The Influence Function, limited to single-instance modifications, was not applicable at the concept level, reinforcing the need for more scalable solutions like Editable CBMs in handling multiple data corrections efficiently.
%Additionally, to ensure the accuracy of our approximations using the Neumann series for inverse Hessian-vector products, a subset of 300 samples from the OAI dataset was used to directly compute the Hessian matrix to confirm that our approximations did not introduce significant errors. However, due to computational constraints, direct computation of the Hessian matrix is often impractical in larger datasets.


\noindent {\bf Editing Multiple Samples.}
To comprehensively evaluate the editing capabilities of ECBM in various scenarios, we conducted experiments on the performance with multiple samples that need to be removed. Specifically, for the concept label/data levels, we consider the different ratios of samples (1-10\%) for edit, while for the concept level, we consider removing different numbers of concepts $\in \{2, 4, 6,\cdots, 20\}$.  We compared the performance of retraining, CBM-IF, and ECBM methods. As shown in Figure \ref{fig:hyperpara}, except for certain cases at the concept level, the F1 score of the ECBM method is generally around \rebuttal{$0.0025$} lower than that of the retrain method, which is significantly better than the corresponding results of the CBM-IF method. Recalling Table \ref{tab:results}, the speed of ECBM is more than three times faster than that of retraining. Consequently, ECBM is an editing method that achieves a trade-off between speed and effectiveness. % We also provide our running time for multiple samples editing in Figure ???????????????????????????\ref{} in the appendix. Results indicate that our method is not affected by the samples of editing.
\input{figs/fig3}


\subsection{Results on Interpretability}
%Since CBM is an explainable model, in this section, we aim to evaluate the interpretability of our ECBM (compared to the retraining). Specifically, we will focus on the concept level edit. 

\noindent{\bf Influence function in ECBM can measure the importance of concepts.} 
The original motivation of the influence function is to calculate the importance score of each sample. Here, we will show that the influence function for the concept level in Theorem \ref{thm:4.3} can be used to calculate the importance of each concept in CBMs, which provides an explainable tool for CBMs. In detail, we conduct our experiments on the CUB dataset. We first select 1-10 most influential and 1-10 least influential concepts by our influence function. Then, we will remove these concepts and update the model via retraining or our ECBM and analyze the change (F1 Score Difference) w.r.t. the original CBM before removal. 

%\noindent{\bf Positive Perturbation and Negative Perturbation. \di{why it is called perturbation? You do not have any perturbations!}} We also report the results of negative and positive perturbation tests (concept removal) by measuring the F1 score obtained by retraining and ECBM method after removing 1-10 most influential and 1-10 least influential concepts, which are selected by the ECBM method.  This serves as an indicator of the interpretability performance of ECBM in identifying influential concepts. We refer to the change in F1 score under these perturbation tests as D-F1. For negative perturbations, a higher D-F1 score indicates more faithful explanations, as a good explanation should maintain accuracy after removing irrelevant concepts. Conversely, for positive perturbations, we expect to observe a sharp decline in performance after removing concepts identified as influential. Besides, the gap value of D-F1 between retraining and editing CBM is a measure of how close ECBM is to the fundamental truth of retraining. We plot the D-F1 bar charts under the removal of concepts. 

The results in Figure \ref{fig:positive} demonstrate that when we remove the \rebuttal{1-10} most influential concepts identified by the ECBM method, the F1 score decreases by more than \rebuttal{0.025} compared to the CBM before removal. In contrast, Figure \ref{fig:negative} shows that the change in the F1 score remains consistently below 0.005 when removing the least influential concepts. These findings strongly indicate that the influence function in ECBM can successfully determine the importance of concepts. Furthermore, we observe that the gap between the F1 score of retraining and ECBM is consistently smaller than 0.005, and even smaller in the case of least important concepts. This further suggests that when ECBM edits various concepts, its performance is very close to the ground truth.
%\warn{The following picture need to be replaced}
\input{figs/fig2}
\\
\noindent{\bf ECBMs can erase data influence.}
For the data level,  ECBMs aim to facilitate an efficient removal of samples. We perform membership inference attacks (MIAs) to provide direct evidence that ECBMs can indeed erase data influence. MIA is a privacy attack that aims to infer whether a specific data sample was part of the training dataset used to train a model. The attacker exploits the model's behavior, such as overconfidence or overfitting, to distinguish between \textit{training (member)} and \textit{non-training (non-member)} data points. In MIAs, the attacker typically queries the model with a data sample and observes its prediction confidence or loss values, which tend to be higher for members of the training set than non-members~\citep{shokri2017membership}.

To quantify the success of these edits, we calculate the RMIA (Removed Membership Inference Attack) score for each category. The RMIA score is defined as the model's confidence in classifying whether a given sample belongs to the training set. Lower RMIA values indicate that the sample behaves more like a test set (non-member) sample~\cite{zarifzadeh2024low}. This metric is especially crucial for edited samples, as a successful ECBM should make the removed members behave similarly to non-members, reducing their membership vulnerability. See Appendix \ref{sec:appendix:exp} for its definition. 

We conducted experiments by randomly selecting 200 samples from the training set (members) and 200 samples from the test set (non-members) of the CUB dataset. We calculated the RMIA scores for these samples and plotted their frequency distributions, as shown in Figure \ref{fig:rmia-1}. The mean RMIA score for non-members was 0.049465, while members had a mean score of 0.063505. Subsequently, we applied ECBMs to remove the 200 training samples from the model, updated the model parameters, and then recalculated the RMIA scores. After editing, the mean RMIA score for the removed-members decreased to 0.052105, significantly closer to the non-members' mean score. This shift in RMIA values demonstrates the effectiveness of ECBMs in editing the model, as the removed members now exhibit behavior closer to that of non-members. The post-editing RMIA score distributions are shown in Figure \ref{fig:rmia-2}. These results provide evidence of the effectiveness of ECBMs in editing the model's knowledge about specific samples.
%\warn{mu {members}:0.063505, mu {nonmembers}:0.049465, mu {removedmembers}:0.052105}
\input{figs/figMIA}

\noindent{\bf Visualization.} Since CBM is an explainable model, we aim to evaluate the interpretability of our ECBM (compared to the retraining). We will present some visualization results for the concept-level edit. Figure~\ref{fig:vertical_images} presents the top \rebuttal{10} most influential concepts and their corresponding predicted concept labels obtained by our ECBM and the retrain method after randomly deleting concepts for the CUB dataset. {\rebuttal{Detailed explanation can be found in Appendix \ref{app:explain}.}}
Our ECBM can provide explanations for which concepts are crucial and how they \rebuttal{assist the prediction}.
Specifically, among the top 10 most important concepts in the ground truth (retraining), ECBM can accurately recognize 9 \rebuttal{within them}. 
For instance, we correctly identify "has\_upperparts\_color::orange", "has\_upper\_tail\_color::red", and "has\_breast\_color::black" as some of the most important concepts when predicting categories. Additional visualization results under data level and concept-label level on OAI and CUB datasets are included in Appendix \ref{app:visual}.
\input{figs/fig4}








==> section/6_conclusion.tex <==
\vspace{-0.2in}
\section{Conclusion}
\vspace{-0.2in}
\label{sec:conclusion}
In this paper, we propose Editable Concept Bottleneck Models (ECBMs). ECBMs can address issues of removing/inserting some training data or new concepts from trained CBMs for different reasons, such as privacy concerns, data mislabelling, spurious concepts, and concept annotation errors retraining from scratch. Furthermore, to improve computational efficiency, we present streamlined versions integrating EK-FAC. Experimental results show our ECBMs are efficient and effective.

%It is important to acknowledge that the ECBM approach is essentially an approximation of the model that would be obtained by retraining with the edited data. This paper does not provide a mathematical quantification of the estimation error associated with this approximation, which could be a potential area for future research.

==> section/accelerate_for_data_level.tex <==
It is worth noting that in theorem \ref{thm:data-level:f}, $H_{\bar{f}^*_{-z_G}}$ serves as an estimate for $H_{\Tilde{f}_{-z_G}}$ which is defined by
\begin{equation*}
    H_{\Tilde{f}_{-z_G}} = \nabla_{\Tilde{f}}\sum_{i\in[n]-G}L_{Y_i}\left(\Tilde{f}_{-z_G}, \hat{g}\right).
\end{equation*}
However, the computation of  $H_{\bar{f}^*_{-z_G}}$ is relatively complex. If the EK-FAC method is further applied to accelerate the process based on this approximation, it will introduce additional errors. Therefore, we can employ a more computationally efficient method with tolerable error to estimate $H_{\Tilde{f}_{-z_G}}$.
% It is worth noting that in theorem, the computation of Hˉf∗−zGH_{\bar{f}^*_{-z_G}} is relatively complex, and the role of Hˉf∗−zGH_{\bar{f}^*_{-z_G}} here is to serve as an estimate of H\Tildef−zGH_{\Tilde{f}_{-z_G}} which is defined by
% \begin{equation*}
%     \nabla_{\Tilde{f}}\sum_{i\in[n]-G}L_{Y_i}\left(\Tilde{f}_{-z_G}, \hat{g}\right).
% \end{equation*}
% If the EK-FAC method is further applied to accelerate the process based on this approximation, it will introduce additional errors. Therefore, considering the high error tolerance when calculating Hˉf∗−zGH_{\bar{f}^*_{-z_G}}, we can employ numerical methods to provide two effective estimates of H\Tildef−zGH_{\Tilde{f}_{-z_G}}.
\begin{theorem}
We can estimate $H_{\Tilde{f}_{-z_G}}$ by the following two ways:
    \begin{align*}
        &H_{\Tilde{f}_{-z_G}} \approx \frac{\|\nabla_{\hat{f}} L_{Y_G}  \| }{\| H_{\hat{f}} \cdot \nabla_{\hat{f}} L_{Y_G} \|} \cdot \left(I - 2 \cdot \frac{C\cdot \nabla_{\hat{f}} L_{Y_G} \cdot {\nabla_{\hat{f}} L_{Y_G}}^{\mathrm{T}} \cdot C }{{\nabla_{\hat{f}} L_{Y_G}}^{\mathrm{T}} \cdot C^2 {\nabla_{\hat{f}} L_{Y_G}}} \right)\\
        &H_{\Tilde{f}_{-z_G}} \approx \nabla_{\hat{f}} L_{Y_G} \cdot {\nabla_{\hat{f}} L_{Y_G}}^{\mathrm{T}} \cdot \left( \nabla_{\hat{f}} L_{Y_G} \cdot {\nabla_{\hat{f}}  L_{Y_G}}^{\mathrm{T}} + \alpha I \right) ^{-1} \cdot H_{\hat{f}},
    \end{align*}
    where $\nabla_{\hat{f}} L_{Y_G}\triangleq\nabla_{\hat{f}} \sum_{r\in G}L_{Y_r} ( \hat{f}, \hat{g})$, and $C\triangleq \frac{H_{\hat{f}}}{\|H_{\hat{f}}\nabla_{\hat{f}} L_{Y_G}\|} - \frac{I}{\|\nabla_{\hat{f}} L_{Y_G}\|}$.
\end{theorem}





\begin{breakablealgorithm}
\caption{Accelerated Data-level ECBM \label{alg:3-1}}
\begin{algorithmic}[1]
    \STATE {\bf Input:} Dataset $\mathcal{D} = \{ (x_i, y_i, c_i) \}_{i=1}^{N}$, original concept predictor $\hat{f}$, label predictor $\hat{g}$, and the to be removed data index set $G$.
    \STATE For $r\in G$, remove the $r$-th data $(x_r, y_r, c_r)$ from $\mathcal{D}$ and define the new dataset as $\mathcal{S}$.
    \STATE Compute the Hessian matrix of the loss function for $\hat{g}$:
    $$H_{\hat{g}} = \nabla^2_{\hat{g}}  \sum_{i,j}  L_{C_j}(\hat{g}^j(x_i),c_i^j).$$
    \STATE Update concept predictor $\Tilde{g}$:
    \begin{equation*}
        \Tilde{g} = \hat{g} + H^{-1}_{\hat{g}} \cdot  \sum_{r\in G}\nabla_{g} L_{C} (\hat{g}(x_r), c_r)
    \end{equation*}
    \STATE Update label predictor $\Tilde{f}$.
    Compute the Hessian matrix of the loss function to $\hat{f}$:
$$H_{\hat{f}} = \nabla^2_{\hat{f}}  \sum_{i=1}^n  L_Y(\hat{f}(\hat{g}(x_i), y_i).$$
\STATE   Compute $A$ as:
    \begin{equation*}
           A =  H^{-1}_{\hat{f}} \cdot  \sum_{i\in [n]-G} \nabla_{\hat{f}} L_{Y}\left(\hat{f}(\hat{g}(x_i)), y_i\right)
    \end{equation*}

\STATE Obtain $\bar{f}$ as 
    \begin{equation*}
        \bar{f} = \hat{f} + A
    \end{equation*}
\STATE Compute the Hessian matrix $H^{\prime}$:

Obtain $$\nabla_{\hat{f}} L_{Y_G}=\nabla_{\hat{f}} \sum_{r\in G}L_Y ( \hat{f} ( \hat{g} (x_r) ), y_r),$$ 
\begin{itemize}
    \item {\bf Method 1}:
    
    Compute $$C=\frac{H_{\hat{f}}}{\|H_{\hat{f}}\nabla_{\hat{f}} L_{Y_G}\|} - \frac{I}{\|\nabla_{\hat{f}} L_{Y_G}\|}$$
    Obtain $H^{\prime}$ as
    \begin{equation*}
        H^{\prime} = \frac{\|\nabla_{\hat{f}} L_{Y_G}  \| }{\| H_{\hat{f}} \cdot \nabla_{\hat{f}} L_{Y_G} \|} \cdot \left(I - 2 \cdot \frac{C\cdot \nabla_{\hat{f}} L_{Y_G} \cdot {\nabla_{\hat{f}} L_{Y_G}}^{\mathrm{T}} \cdot C }{{\nabla_{\hat{f}} L_{Y_G}}^{\mathrm{T}} \cdot C^2 {\nabla_{\hat{f}} L_{Y_G}}} \right)
    \end{equation*}
    \item {\bf Method 2}:

    Obtain $H^{\prime}$ as 
    \begin{equation*}
        H^{\prime} = \nabla_{\hat{f}} L_{Y_G} \cdot {\nabla_{\hat{f}} L_{Y_G}}^{\mathrm{T}} \cdot \left( \nabla_{\hat{f}} L_{Y_G} \cdot {\nabla_{\hat{f}}  L_{Y_G}}^{\mathrm{T}} + \alpha I \right) ^{-1} \cdot H_{\hat{f}}
    \end{equation*}
\end{itemize}


\STATE Compute $B$ as
    \begin{equation*}
        B = -{H^{\prime}}^{-1}\cdot \sum_{i\in [n]-G}\nabla_{\hat{f}}\left(    L_Y(\bar{f}(\Tilde{g}(x_i)), y_i) - L_Y(\bar{f}(\hat{g}(x_i)), y_i)\right)
    \end{equation*}
\STATE Update the label predictor $\Tilde{f}$ as: $\Tilde{f} =  \hat{f} + A + B.$
    \STATE {\bf Return: $\Tilde{f}$, $\Tilde{g}$}.  
\end{algorithmic}
\end{breakablealgorithm}


\begin{lemma}\label{approx:H:1}
\cite{hildebrand1987introduction} If we have an equation $A\cdot x = y$, where $x$ and $y$are known and $A$ is unknown. Then, the solution $A$ will not be unique. We can use a scaled Householder transformation to estimate $A$. If $x$ and $y$ are non-zero vectors with $\hat{x}=\frac{x}{\|x\|}$ and $\hat{y}=\frac{y}{\|y\|}$, then we can take  
\begin{equation*}
A=\left\{\begin{array}{ll}  
\frac{\|y\|}{\|x\|}\cdot\left(I-2 \frac{v v^{T}}{v^{T} v}\right) & \hat{x} \neq \hat{y} \\  
\frac{\|y\|}{\|x\|}\cdot I & \hat{x}=\hat{y}  
\end{array}\right.  
\end{equation*} 
where $v=\hat{x}-\hat{y}$.
\end{lemma}

\begin{proof}
Suppose we are given a unit vector $\hat{x}$ and we want to find a reflection that transforms $\hat{x}$ into a direction parallel to another given vector $\hat{y}$, which is not equal to $\hat{x}$, then the right reflection is through a hyperplane that bisects the angle between $\hat{x}$ and $\hat{y}$, which can be constructed by taking the hyperplane normal to $\|\hat{x} - \hat{y}\|$, that is, letting $v = \hat{x} -\hat{y}$,
\begin{align*}
\left (I - 2 \frac{v \cdot v^{\mathrm{T}}}{v^{\mathrm{T}} v} \right )\cdot \hat{x} - \hat{y} 
= & \frac{\hat{x} - \hat{y}}{\|\hat{x} - \hat{y}\|_{2}^{2}}\left(\|\hat{x} - \hat{y}\|_{2}^{2}-2(\hat{x} - \hat{y})^{t} \hat{x}\right) \\ 
= & \frac{\hat{x} - \hat{y}}{\|\hat{x} - \hat{y}\|_{2}^{2}}\left((\hat{x} - \hat{y})^{t}(\hat{x} - \hat{y})-2(\hat{x} - \hat{y})^{t} \hat{x}\right)  \\ 
= & \frac{\hat{x} - \hat{y}}{\|\hat{x} - \hat{y}\|_{2}^{2}}\left(\hat{x}^{t} \hat{x}-\hat{x}^{t} \hat{y}-\hat{y}^{t} \hat{x}+\hat{y}^{t} \hat{y} -2 \hat{x}^{t} \hat{x}+2 \hat{y}^{t} \hat{x}\right) = 0.
\end{align*}

Denote $\Tilde{A} = I - 2 \frac{v\cdot v^{\mathrm{T}}}{v^{\mathrm{T}} v}$, then we have $\Tilde{A} \hat{x} = \hat{y}$, that is $ \frac{\|y\|}{\|x\|} \cdot \Tilde{A} x = y$. If we choose $A$ to be $\frac{\|y\|}{\|x\|} \cdot \left(I - 2 \frac{v v^{\mathrm{T}}}{v^{\mathrm{T}} v}\right )$, then we have $A x = y$. 

If $x = y$, then we set $\Tilde{A} = I$, and we have $A = \frac{\|y\|}{\|x\|} \cdot I$.
\end{proof}

\begin{lemma}\label{approx:H:2}
\cite{boyd2004convex} If we frame solving equation $A\cdot x = y$ for $A$ as the following optimization problem:
\begin{equation*}
    \min_{A}\frac{1}{2}\|A\cdot x-y\|_{F}^{2}+\frac{\alpha}{2}\|A\|_{F}^{2},
\end{equation*}
where 
\begin{equation*}
    \|A\|_F=\left(\sum_{i=1}^n \sum_{j=1}^n a_{i, j}^2\right)^{\frac{1}{2}}=\operatorname{trace}\left[A^{\top} A\right]^{\frac{1}{2}}
\end{equation*} is the  Frobenius norm, and $\alpha$ is a regularization parameter. Then $A$ can be approximated by
\begin{equation*}
 A = yx^T\left(xx^T + \alpha I\right)^{-1}.
\end{equation*}
\end{lemma}

\begin{proof}
The objective function can be written as 
$$\frac{1}{2}\operatorname{tr}\left[\left(Ax - y\right)^T\left(Ax - y\right)\right] + \frac{\alpha}{2}\operatorname{tr}\left[A^TA\right].$$ 
If $A$ is perturbed in any direction $H$, the derivative of the objective function at $A$ should be zero. That is 
\begin{align*} 
0 &= \frac{d}{dA}\left(\frac{1}{2}\operatorname{tr}\left[\left(Ax -y\right)^T\left(Ax - y\right)\right] + \frac{\alpha}{2}\operatorname{tr}\left[A^TA\right]\right) \cdot H \\ 
&=\operatorname{tr}\left[\left(Hx\right)^T\left(Ax - y\right)\right]+\alpha\operatorname{tr}\left[H^TA\right] \\ 
&= \operatorname{tr}\left[H^T\left(\left(Ax - y\right)x^T + \alpha A\right)\right]. 
\end{align*}
Where $\operatorname{tr}$ is the trace of matrix defined as $\operatorname{tr}(A) = A_{1,1} + A_{2,2} + \cdots + A_{n,n}$.

Since this must hold for all perturbations $H$, we must have $$0 = \left(Ax - y\right)x^T + \alpha A.$$ 
which we may solve to find 
$A = yx^T \left( xx^T + \alpha I \right)^{-1}.$
% Using the Woodbury formula we have 
% (xxT+αI)−1=1α(I−x(αI+xTx)−1xT)\left(xx^T + \alpha I\right)^{-1} = \frac{1}{\alpha}\left( I - x\left(\alpha I + x^Tx\right)^{-1}x^T\right)
% and therefore 
%A=1αyxT−1αyxTx(αI+xTx)−1xT.A = \frac{1}{\alpha}yx^T - \frac{1}{\alpha}yx^T x\left(\alpha I + x^Tx\right)^{-1}x^T.
\end{proof}


\begin{theorem}
    Observing the complexity of computing $H_{\Tilde{f}_{-z_G}}$, we consider the method from lemma \ref{approx:H:1} and \ref{approx:H:2} to approximate the Hessian matrix avoid of iHVP problem. And $H_{\Tilde{f}}$ can be estimated by
    \begin{align*}
        &H_{\Tilde{f}_{-z_G}} \approx \frac{\|\nabla_{\hat{f}} L_{Y_G}  \| }{\| H_{\hat{f}} \cdot \nabla_{\hat{f}} L_{Y_G} \|} \cdot \left(I - 2 \cdot \frac{C\cdot \nabla_{\hat{f}} L_{Y_G} \cdot {\nabla_{\hat{f}} L_{Y_G}}^{\mathrm{T}} \cdot C }{{\nabla_{\hat{f}} L_{Y_G}}^{\mathrm{T}} \cdot C^2 {\nabla_{\hat{f}} L_{Y_G}}} \right)\\
        &H_{\Tilde{f}_{-z_G}} \approx \nabla_{\hat{f}} L_{Y_G} \cdot {\nabla_{\hat{f}} L_{Y_G}}^{\mathrm{T}} \cdot \left( \nabla_{\hat{f}} L_{Y_G} \cdot {\nabla_{\hat{f}}  L_{Y_G}}^{\mathrm{T}} + \alpha I \right) ^{-1} \cdot H_{\hat{f}},
    \end{align*}
    where $\nabla_{\hat{f}} L_{Y_G}\triangleq\nabla_{\hat{f}} \sum_{r\in G}L_Y ( \hat{f} ( \hat{g} (x_r) ), y_r)$, and $C\triangleq \frac{H_{\hat{f}}}{\|H_{\hat{f}}\nabla_{\hat{f}} L_{Y_G}\|} - \frac{I}{\|\nabla_{\hat{f}} L_{Y_G}\|}$.
\end{theorem}
\begin{proof}
The computational complexity of $H_{\Tilde{f}_{-z_G}}$ in theorem \ref{3-esti-f} is relatively high, so we try to estimate it. We rewrite the format of $\Tilde{f}_{-z_G}$ and $\hat{f}$ and define a new symbol $\hat{f}_{\epsilon}$. When $\epsilon \rightarrow 1$, $\hat{f}_{\epsilon} \rightarrow \hat{f}$, When $\epsilon \rightarrow 0$, $\hat{f}_{\epsilon}\rightarrow \Tilde{f}_{-z_G}$.
\begin{equation*}
\left \{
\begin{aligned}
 \Tilde{f}_{-z_G} = \argmin_f \sum_{i \in S}^{n} L_Y \left(  f \left(  \hat{g} (x_i) \right),y_i  \right) \quad \text{ \textcircled{1} } \\
\hat{f}_{\epsilon} = \argmin_f \sum_{i \in S}^{n} L_Y \left(  f (\hat{g}(x_i)), y_i  \right) +  \epsilon \cdot \sum_{r\in G}L_Y \left( f ( \hat{g} (x_r) ) , y_r   \right) \quad \text{ \textcircled{2} }
\end{aligned}
\right.
\end{equation*}

For the \textcircled{2} equation, we use Taylor expansion:
\begin{equation*}
    \nabla_{\hat{f}_{\epsilon}} \sum_{i \in S }^{n} L_Y \left(  \hat{f}_{\epsilon} (\hat{g}(x_i)), y_i  \right) +  \epsilon \cdot \nabla_{\hat{f}_{\epsilon}} \sum_{r\in G}L_Y \left( \hat{f}_{\epsilon} ( \hat{g} (x_r) ) , y_r   \right) = 0.
\end{equation*}

If we expand in $\Tilde{f}_{-z_G}$, then we have,
\begin{align*}
&   \nabla_{\Tilde{f}_{-z_G}} \sum_{i\in S}^{n} L_Y \left(  \Tilde{f}_{-z_G} (\hat{g}(x_i)), y_i  \right) +  \epsilon \cdot \nabla_{\Tilde{f}_{-z_G}}\sum_{r\in G} L_Y \left( \Tilde{f}_{-z_G} ( \hat{g} (x_r) ) , y_r   \right)  \\
& + \left[ \nabla^{2}_{\Tilde{f}_{-z_G}} \sum_{i\in S}^{n} L_Y \left(  \Tilde{f}_{-z_G} (\hat{g}(x_i)), y_i  \right) +  \epsilon \cdot \nabla^{2}_{\Tilde{f}_{-z_G}}\sum_{r\in G} L_Y \left( \Tilde{f}_{-z_G} ( \hat{g} (x_r) ) , y_r   \right) \right] ( \hat{f}_{\epsilon} - \Tilde{f}_{-z_G} ) = 0.
\end{align*}

We know that $\nabla_{\Tilde{f}_{-z_G}} \sum_{i\in S}^{n} L_Y \left(  \Tilde{f}_{-z_G} (\hat{g}(x_i)), y_i  \right) = 0$, and $\nabla^{2}_{\Tilde{f}_{-z_G}} \sum_{i\in S}^{n} L_Y \left(  \Tilde{f}_{-z_G} (\hat{g}(x_i)), y_i  \right)$ is the $H_{\Tilde{f}_{-z_G}}$ which we want to estimate. 

Then, we expand $\nabla_{\Tilde{f}_{-z_G}} \sum_{r\in G}L_Y \left( \Tilde{f}_{-z_G} ( \hat{g} (x_r) ) , y_r   \right)$ in the $\hat{f}_{\epsilon}$, we have,
\begin{equation*}
   H_{\Tilde{f}_{-z_G}} \cdot \left[ \hat{f}_{\epsilon} - \Tilde{f}_{-z_G}   \right] 
 = -\epsilon \cdot \nabla_{\Tilde{f}_{-z_G}}\sum_{r\in G} L_Y ( \Tilde{f}_{-z_G} ( \hat{g} (x_r) ), y_r ).
\end{equation*}

\begin{equation*}
    \Rightarrow
   H_{\Tilde{f}_{-z_G}} \cdot \frac{   \left[ \hat{f}_{\epsilon} - \Tilde{f}_{-z_G}   \right] } {\epsilon}
 = (-1) \sum_{r\in G}\cdot \left[ \nabla_{\hat{f}_{\epsilon}} L_Y ( \hat{f}_{\epsilon} ( \hat{g} (x_r) ), y_r )     + \nabla^{2}_{\hat{f}_{\epsilon}}  L_Y ( \hat{f}_{\epsilon} ( \hat{g} (x_r) ), y_r ) \cdot ( \Tilde{f}_{-z_G} - \hat{f}  )   \right].
\end{equation*}
\begin{equation*}
    \Rightarrow
   H_{\Tilde{f}_{-z_G}} \cdot \frac{   \left[ \hat{f}_{\epsilon} - \Tilde{f}_{-z_G}   \right] } {\epsilon}
 \approx (-1)\sum_{r\in G} \cdot \nabla_{\hat{f}_{\epsilon}} L_Y ( \hat{f}_{\epsilon} ( \hat{g} (x_r) ), y_r ).  
\end{equation*}

We estimate it using the value $\epsilon = 1$,
\begin{equation*}\label{approxH}
 H_{\Tilde{f}_{-z_G}} \cdot ( \hat{f} - \Tilde{f}_{-z_G} ) 
\approx (-1) \sum_{r\in G}\cdot \nabla_{\hat{f}} L_Y ( \hat{f} ( \hat{g} (x_r) ), y_r).
\end{equation*}

Substituting equation \ref{ap:approx:f_piao} into the above equation and we have
\begin{equation}\label{app:aprox:H_piao}
    H_{\Tilde{f}_{-z_G}} \cdot \left (H_{\hat{f}} \cdot \nabla_{\hat{f}} \sum_{r\in G}L_Y ( \hat{f} ( \hat{g} (x_r) ), y_r )  \right )= \nabla_{\hat{f}} \sum_{r\in G}L_Y ( \hat{f} ( \hat{g} (x_r) ), y_r ).  
\end{equation}

Estimating $H_{\Tilde{f}_{-z_G}}$ from the above equation is an ill-posed problem, and we give an estimation by directly substituting \eqref{app:aprox:H_piao} into lemma \ref{approx:H:1} and \ref{approx:H:2}:
\begin{align*}
        &H_{\Tilde{f}_{-z_G}} = \frac{\|\nabla_{\hat{f}} L_{Y_G}  \| }{\| H_{\hat{f}} \cdot \nabla_{\hat{f}} L_{Y_G} \|} \cdot \left(I - 2 \cdot \frac{C\cdot \nabla_{\hat{f}} L_{Y_G} \cdot {\nabla_{\hat{f}} L_{Y_G}}^{\mathrm{T}} \cdot C }{{\nabla_{\hat{f}} L_{Y_G}}^{\mathrm{T}} \cdot C^2 {\nabla_{\hat{f}} L_{Y_G}}} \right)\\
        &H_{\Tilde{f}_{-z_G}} = \nabla_{\hat{f}} L_{Y_G} \cdot {\nabla_{\hat{f}} L_{Y_G}}^{\mathrm{T}} \cdot \left( \nabla_{\hat{f}} L_{Y_G} \cdot {\nabla_{\hat{f}}  L_{Y_G}}^{\mathrm{T}} + \alpha I \right) ^{-1} \cdot H_{\hat{f}},
    \end{align*}
    where $\nabla_{\hat{f}} L_{Y_G}\triangleq\nabla_{\hat{f}} \sum_{r\in G}L_Y ( \hat{f} ( \hat{g} (x_r) ), y_r)$, and $C\triangleq \frac{H_{\hat{f}}}{\|H_{\hat{f}}\nabla_{\hat{f}} L_{Y_G}\|} - \frac{I}{\|\nabla_{\hat{f}} L_{Y_G}\|}$.
\end{proof}




==> section/app_notation_table.tex <==
\section{\rebuttal{Notation Table}}
\begin{table}[ht]  
    \centering  
    \begin{tabular}{@{}ll@{}}  
        \toprule  
        Symbol & Description \\ \midrule  
        ${c} = \{p_1, \ldots, p_k\}$ & Set of concepts provided by experts or LLMs. \\
        $\mathcal{D} = \{ z_i \}_{i=1}^{n}$ & Training dataset, where $z_i = (x_i, y_i, {c_i})$. \\
        $x_i \in \mathbb{R}^m$ & Feature vector for the $i$-th sample. \\
        $y_i \in \mathbb{R}^{d_z}$ & Label for the $i$-th sample, with $d_z$ being the number of classes. \\
        $c_i = (c_i^1, \ldots, c_i^k) \in \mathbb{R}^k$ & Concept vector for the $i$-th sample. \\
        $\tilde{c}_w^r$ & Corrected concept label for the $w$-th sample and $r$-th concept. \\
        $c_i^j$ & Weight of the concept $p_j$ in the concept vector $c_i$. \\
        $g: \mathbb{R}^m \to \mathbb{R}^k$ & Concept predictor mapping input space to concept space. \\
        $f: \mathbb{R}^k \to \mathbb{R}^{d_z}$ & Label predictor mapping concept space to prediction space. \\
        $L_{C}(g^j(x),c^j)$ & Loss function for the $j$-th concept predictor. \\
        $L_{C_j}(g(x),c)$ & Loss function for the $j$-th concept predictor(for simplicity). \\
        $L_{Y}(f(\hat{g}(x)), y)$ & Loss function from concept space to output space. \\
        $L_{Y_i}(f, \hat{g})$ & Loss function for the $i$-th input based on ${f}$, $\hat{g}$(for simplicity). \\
        $H_{\hat{\theta}}$ & Hessian matrix of the loss function with respect to $\hat{\theta}$. \\
        $G_{\hat{\theta}}$ & Fisher information matrix of model $\hat{\theta}$. \\
        $\lambda$ & Damping term for ensuring positive definiteness of the Hessian. \\
        $\hat{g}$ & Estimated concept predictor. \\
        $\hat{f}$ & Estimated label predictor. \\
        $\hat{g}_{e}$ & Retrained concept predictor after correcting erroneous data. \\
        $\hat{f}_{e}$ & Retrained label predictor after correcting erroneous data. \\
        $\hat{g}_{-p_M}$ & Retrained concept predictor after removing concepts indexed by $M$. \\
        $\hat{g}^{*}_{-p_M}$ & Mapped concept predictor with the same dimensionality as $\hat{g}$. \\
        $\bar{g}_{-p_M}$ & Approximation of the retrained concept predictor $\hat{g}_{-p_M}$. \\
        $\hat{f}_{p_M=0}$ & Label predictor after setting the $r$-th concept to zero for $r \in M$. \\
        $\bar{f}_{p_M=0}$ & Approximation of the label predictor $\hat{f}_{p_M=0}$. \\
        $H_{\hat{g}}$ & Hessian matrix of the loss function with respect to $\hat{g}$. \\
        $H_{\hat{f}}$ & Hessian matrix of the loss function with respect to $\hat{f}$. \\
        $M \subset [k]$ & Set of erroneous concept indices to be removed. \\
        $G \subset [n]$ & Set of indices of samples to be removed from the dataset. \\
        $z_r = (x_r, y_r, c_r)$ & Data sample to be removed, where $r \in G$. \\
        $\hat{g}_{-z_G}$ & Retrained concept predictor after removing samples indexed by $G$. \\
        $\bar{g}_{-z_G}$ & Approximation of the retrained concept predictor $\hat{g}_{-z_G}$. \\
        $\Tilde{f}_{-z_G}$ & Intermediate label predictor. \\
        $\bar{f}_{-z_G}$ & Final edited label predictor after removing samples indexed by $G$. \\
        \bottomrule  
    \end{tabular}  
\caption{\rebuttal{Notation Table}}
    \label{tab:notation}  
\end{table}

==> section/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}
\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our main claims made in the abstract and introduction accurately reflect the paper's contributions and scope. See in Section \ref{sec:intro} and Abstract.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Section \ref{sec:limitation}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide the full set of assumptions and a complete (and correct) proof. See Section \ref{sec:further}, Section \ref{sec:appendix:b}, Section \ref{sec:appendix:c}, and Section \ref{sec:appendix:d} in the Appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Section \ref{sec:exp} and Section \ref{sec:appendix:exp}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, we will provide the code.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Section \ref{sec:exp} and Section \ref{sec:appendix:exp}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Section \ref{sec:exp} and Section \ref{sec:appendix:exp}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Section \ref{sec:exp} and Section \ref{sec:appendix:exp}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Section \ref{sec:impacts}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected. See Section \ref{sec:exp} and Section \ref{sec:appendix:exp}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}


==> section/extra_stuff.tex <==
%\section{More Related Work}
%\label{sec:app:related work}
%\paragraph{Concept Bottleneck Models.} 
%CBM \cite{koh2020concept} stands out as an innovative deep-learning approach for image classification and visual reasoning. It introduces a concept bottleneck layer into deep neural networks, enhancing model generalization and interpretability by learning specific concepts. However, CBM faces two primary challenges: its performance often lags behind that of original models lacking the concept bottleneck layer, attributed to incomplete information extraction from the original data to bottleneck features. Additionally, CBM relies on laborious dataset annotation. Researchers have explored solutions to these challenges. \cite{chauhan2023interactive} extend CBM into interactive prediction settings, introducing an interaction policy to determine which concepts to label, thereby improving final predictions. \cite{oikarinen2023label} address CBM limitations and propose a novel framework called Label-free CBM. This innovative approach enables the transformation of any neural network into an interpretable CBM without requiring labeled concept data, all while maintaining high accuracy. Post-hoc Concept Bottleneck models \cite{yuksekgonul2022post} can be applied to various neural networks without compromising model performance, preserving interpretability advantages. CBMs work on the image field also includes \cite{havasi2022addressing,kim2023probabilistic,keser2023interpretable,sawada2022concept,sheth2023auxiliary}. For the graph concept field, \cite{magister2021gcexplainer} provides a global interpretation for Graph Neural Networks (GNN). They begin by mapping graphs into a concept space through clustering and subsequently offer a human-in-the-loop evaluation. \cite{xuanyuan2023global, Barbiero2023interpretable} extends this approach by incorporating global and local explanations. For local explanations, they define a concept set, with each neuron represented as a vector with Boolean values indicating concept activation. 

%Despite many works on CBMs, we are the first to investigate the interactive influence between concepts through influence functions. Our research endeavors to bridge this gap by utilizing influence functions in CBMs, thereby deciphering the interaction of concept models and providing an adaptive solution to concept editing.

%\noindent {\bf Influence Function.} The influence function, initially a staple in robust statistics \cite{cook2000detection,cook1980characterizations}, has seen extensive adoption within machine learning since \cite{koh2017understanding} introduced it to the field. Its versatility spans various applications, including detecting mislabeled data, interpreting models, addressing model bias, and facilitating machine unlearning tasks. In the domain of machine unlearning, several studies leverage influence functions for approximate unlearning, offering closed-form updates of model parameters and tracing the impact of unlearning on recalled data samples. Notable works in this area encompass unlearning features and labels \cite{warnecke2021machine}, minimax unlearning \cite{liu2024certified}, forgetting a subset of image data for training deep neural networks \cite{golatkar2020eternal,golatkar2021mixed}, graph unlearning involving nodes, edges, and features. Recent advancements, such as the LiSSA method \cite{agarwal2017second,kwon2023datainf} and kNN-based techniques \cite{guo2021fastif}, have been proposed to enhance computational efficiency. These methods enable faster computation of the inverse Hessian in influence functions, facilitating the identification of influential examples and mislabeled data in large-scale models. Various studies have applied influence functions to interpret models across different domains, including natural language processing \cite{han2020explaining} and image classification \cite{basu2021influence}, while also addressing biases in classification models \cite{wang2019repairing}, word embeddings \cite{brunet2019understanding}, and finetuned models \cite{chen2020multi}. 

%Despite numerous studies on influence functions, we are the first to utilize them to construct the editable CBM. This offers valuable insights into removing mislabeled concepts and interpreting data influence within CBMs. Moreover, compared to traditional neural networks, CBMs are more complicated in their influence function. Because we only need to change the predicted output in the traditional influence function. While in CBMs, we should first remove the true concept, then we need to approximate the predicted concept in order to approximate the output. Bridging the gap between the true and predicted concepts poses a significant theoretical challenge in our proof.








#######  Extra stuff ######

We then introduce an important lemma across all three scenarios,
\begin{lemma}
    For the concept bottleneck model, if the bottleneck layer C\mathcal{C} utilize linear transformations of the θTc\theta^{T} c, then we have θ∗pj=0\theta^{*}_{p_j=0} = θ∗−pj\theta^{*}_{-p_j}. 
\end{lemma}

\begin{proof}
It is evident that for the dot product, θTc\theta^{T} c is irrelevant whether a dimension of cc is missing or equals zero in the linear transformation
\begin{equation*}
    \sum_{k:k \neq j} \theta[k] c[k] = \sum_k \theta[j] \mathbb{I} \{ k \notin j \} c[k].
\end{equation*}
Thus, the loss ℓ(z,θ)=ℓ(θTˆc,y;θ)\ell (z,\theta) = \ell(\theta^T \hat{c}, y; \theta) of both models is the same for every sample in the second stage. Thus, L(θ;D)L(\theta;\mathcal{D}) is also equal for both models with the same model parameters.
\end{proof}




\noindent{\bf Second Stage.} 
We first focus on the difference between ˆf\hat{f} and ˆfpr=0\hat{f}_{p_r=0}. The influence function can be defined as :
\begin{equation*}
\mathcal{I}(z) \stackrel{\text { def }}{=} \frac{d \hat{\theta}_{\epsilon, z}}{d \epsilon}|_{\epsilon=0}=-H_{\hat{\theta}}^{-1} \nabla_{\hat{\theta}} L(z, \hat{\theta}),  
\end{equation*}

We can linearly approximate the parameter change by the following equation,

\begin{equation}
\label{eq:1}
    \hat{f}_{p_r=0} = -H_{\hat{f}}^{-1} \cdot  \left( \nabla_{\hat{f}} \sum_{i=1}^n \ell \left( \hat{f}\left(\hat{g}\left(x_{i}\right), y_{i}\right)\right)-\nabla_{\hat{f}} \sum_{i=1}^n\ell\left(\hat{f}\left(\hat{g}_{-p_r}^{*}\left(x_{i}\right), y_{i}\right)\right)\right).
\end{equation}

Because $\hat{f}$ is the minimizer of the label loss of the original dataset, the first term in the above equation equals zero.

\noindent{\bf First Stage.}
Now, we come to the problem of approximating ˆg∗−pr∈T0={wfinal=0}⊆T\hat{g}^{*}_{-p_r} \in T_0 = \{ w_{\text{final}} = 0 \}  \subseteq T, where wfinalw_{\text{final}} is the parameter of the final layer of neural network. And ˆg∈T\hat{g} \in T. We use ˆgϵ\hat{g}_{\epsilon} to approximate ˆg∗−pr\hat{g}^{*}_{-p_r}. Similar to the original idea of defining the influence function, we define the following:
\begin{equation}
    \hat{g}_{-p_r}^{*}=\underset{g \in \Gamma_0}\argmin \sum_{\substack{j=1, j \neq p_r}}^{k}\sum_{i=1}^{n} \ell\left(g^j\left(x_{i}\right), c^{j}_i\right).
\end{equation}
\begin{equation}
    \hat{g}=\underset{g \in T}\argmin \sum_{\substack{j=1, j \neq p_r}}^{k} \sum_{i=1}^{n} \ell\left(g^{j}\left(x_{i}\right), c_i^j\right)
    +\sum_{i=1}^n \ell\left(g^p_r(x_i), c_i^{p_r}\right).
\end{equation}
\begin{equation}
    \hat{g}_{\epsilon} \triangleq \underset{g \in T}\argmin \sum_{\substack{j=1, j \neq p_r}}^{k} \sum_{i=1}^{n}\ell\left(g^{j}\left(x_{i}\right), c^{j}_i\right)+\epsilon \cdot \sum_{i=1}^{n} \ell\left(g^{p_r}\left(x_{i}\right), c^{p_r}_i\right).
\end{equation}
When ϵ→0\epsilon \rightarrow 0, ˆgϵ→ˆg∗−pr\hat{g}_{\epsilon} \rightarrow \hat{g}_{-p_r}^{*}, by the condition of the minimizer, we can obtain:
\begin{equation}
    \nabla_{g}\sum_{\substack{j=1, j \neq p_r}}^{k} \sum_{i=1}^{n} \ell\left(\hat{g}_{-p_r}^{*j}\left(x_{i}\right), c^{j}_i\right)=0
\end{equation}
Perform a Taylor expansion of the above equation at ˆgϵ\hat{g}_{\epsilon}, we can obtain

\begin{equation*}
    \nabla_{\hat{f}} \sum_{i=1}^{n} \ell ( \hat{f}( \hat{g}^{*}_{-p_r} (x_{i})), y_{i})
= -\nabla_{\hat{f}} \sum_{i=1}^{n} \ell \left( \hat{f} \left( \hat{g} (x_i) - H^{-1}_{\hat{g}} \cdot \nabla_{\hat{g}} \sum_{j=1, j \neq r}^{k} \sum_{i=1}^{n} \ell ( \hat{g}_{j} (x_i), c_j) \right) , y_i \right).
\end{equation*}

Substitute $\nabla_{\hat{f}} \sum_{i=1}^{n} \ell ( \hat{f}( \hat{g}^{*}_{-p_r} (x_{i})), y_{i})$ to equation \ref{eq:1}, we get the final closed-form influence function:

\begin{equation}
    \hat{f}_{-p_r}
= -H_{\hat{f}}^{-1} \cdot   \nabla_{\hat{f}} \sum_{i=1}^{n} \ell \left( \hat{f} \left( \hat{g} (x_i) - H^{-1}_{\hat{g}} \cdot \nabla_{\hat{g}} \sum_{j=1, j \neq r}^{k} \sum_{i=1}^{n} \ell ( \hat{g}_{j} (x_i), c_j) \right) , y_i \right).
\end{equation}

\noindent{\bf First Stage.}
To obtain the approximation of the parameters change. Motivated by \cite{koh2017understanding}, we do a derivation and definition of the influence function.
\begin{equation}
    \hat{g}_{\epsilon, -z_r} = \argmin \sum_{i \neq r} \ell(g(x_i), c_i) + \epsilon \cdot \ell\left(g(x_r), c_r\right).
\end{equation}
Then, when $\epsilon \to 0$, $\hat{g}_{\epsilon, -z_r} \to \hat{g}$.
\begin{equation}
    \mathcal{I}(z_r) \stackrel{\text { def }}{=} \frac{d \hat{g}_{\epsilon, -z_r}}{d \epsilon}|_{\epsilon=0}=-H_{\hat{g}}^{-1} \nabla_{\hat{g}} \sum \ell\left(\hat{g}(x_i),c_i\right),  
\end{equation}
Then, we can linearly approximate $\hat{g}_{-z_r}$ by computing $\hat{g} - 1 \cdot \mathcal{I}(z_r)$.

\noindent{\bf Second Stage.} Now we approximate $\hat{f}_{-z_r}$.
\begin{equation}
    \hat{f}_{-z_r} = \argmin_{f}\sum_{\substack{i = 1}}^{n} \ell(f\left(\hat{g}_{-z_r}(x_{i})\right), y_{i}) - \ell\left(f(\hat{g}_{-z_r}(x_r)), y_r\right)
\end{equation}
\begin{equation}
    \hat{f}_{-z_r}^* = \argmin_{f}\sum_{\substack{i = 1}}^{n} \ell(f\left(\hat{g}(x_{i})\right), y_{i})- \ell\left(f(\hat{g}(x_r)), y_r\right)
\end{equation}
We can evaluate the difference between $\hat{f}^*_{-z_r}$ and $\hat{f}$, and then approximate $\hat{f}_{-z_r} - \hat{f}^*_{-z_r}$ use the method similar to Appendix \ref{ap1}. Finally, we get the closed-form solution,

\begin{align*}
&\hat{f}_{-z_r} = \hat{f} + H^{-1}_{\hat{f}}  \left(  
\nabla_{\hat{f}} \sum_{i=1}^{n} \ell \left(   \hat{f} ( \hat{g} (x_i) ) , y_i   \right) \right) \\
& \cdot \left(  1  -  \left( \nabla_{\hat{f}} \ell \left( 
\hat{f} ( \hat{g} (x_r) ),y_r \right) \cdot \left( 
\nabla_{\hat{f}} \sum_{i=1,i \neq r}^{n} \ell \left(   \hat{f} ( \hat{g} (x_i) ) , y_i   \right)  -  \nabla_{\hat{f}} \sum_{i=1, i \neq r }^{n} \ell \left( 
\hat{f} ( \hat{g} (x_i) ),y_i \right) \right) \right) \right).
\end{align*}

Similar to previous practice, we approximate the retrained concept predicting model first and obtain the approximation of $\hat{g}_{c_w^r = 0}$ as 
\begin{equation}\label{4.4-1}
    \hat{g}_{c^r_w=0} \approx \hat{g} -H^{-1}_{\hat{g}} \cdot \nabla_g \sum_{j=1}^k \sum_{i=1}^n  \ell ( \hat{g}^j(x_i), c^j_i)
\end{equation}
On the other hand, we estimate $\hat{f}_{c_w^r = 0}$ as:
\begin{equation}\label{4.4-2}
    \hat{f}_{c_w^r = 0} \approx \hat{f}  -H^{-1}_{\hat{f}}\cdot\sum_{i=1}^n\nabla_f  \left( \ell \left( \hat{f} \left( \hat{g}_{\epsilon, c^r_w=0} \left(x_{i} \right) \right), y_{i}\right)-  \ell \left(  \hat{f}\left(\hat{g}\left(x_{i} \right) \right), y_{i} \right) \right),
\end{equation}
Substituting equation \ref{4.4-2} into equation \ref{4.4-1}, we have
\begin{align}
     \hat{f}_{c_w^r = 0} &= \hat{f} + H^{-1}_{\hat{f}} \cdot \nabla_f \sum_{i=1}^n \ell \left(   \hat{f} \left( \hat{g} ( x_{i} ) 
 \right) , y_{i} \right) \notag \\
     & - H^{-1}_{\hat{f}} \cdot \nabla_f \sum_{i=1}^n \left( \ell \left( \hat{f} \left( \hat{g} (x_{i} )
    - H^{-1}_{\hat{g}} \cdot \nabla_g \sum_{j=1}^k\sum_{i=1}^n \ell ( \hat{g}^j(x_i), c^j_i) ( x_i ) \right) , y_{i_c} \right) \right).
\end{align}

\begin{algorithm}[h]
\caption{Concept-level ECBM \label{alg:2}}
\begin{algorithmic}[1]
    \State {\bf Input:} Dataset $\mathcal{D} = \{ (x_i, y_i, c_i) \}_{i=1}^{N}$, original concept predictor $\hat{f}$, and label predictor $\hat{g}$.
    \State Set $p_r = 0$ for all $\mathcal{D}$.
    \For {$i=1,\cdots, k$} \quad \quad \quad   \# Update concept predictor
    \If {$i=r$}
        \State Update $\Tilde{g}^{r}$:
    \begin{equation*}
        \Tilde{g}^{r} \approx \hat{g} (x_i) - H^{-1}_{\hat{g}} \cdot \nabla_{\hat{g}} \sum_{j=1, j \neq r}^{k} \sum_{i=1}^{n} \ell ( \hat{g}_{j} (x_i), c_j).
    \end{equation*}
    \Else
        \State Update other concept predictors:
        $\Tilde{g}^i=\hat{g}^i$.
    \EndIf
    \EndFor 
    \State Update label predictor $\Tilde{f}$:
    \begin{equation*}
    \hat{f}_{-p_r}
    \approx \hat{f}-H_{\hat{f}}^{-1} \cdot   \nabla_{\hat{f}} \sum_{i=1}^{n} \ell \left( \hat{f} \left( \hat{g} (x_i) - H^{-1}_{\hat{g}} \cdot \nabla_{\hat{g}} \sum_{j=1, j \neq r}^{k} \sum_{i=1}^{n} \ell ( \hat{g}_{j} (x_i), c_j) \right) , y_i \right).
    \end{equation*}
    \State {\bf Return: $\Tilde{f}$, $\Tilde{g}$}.  
\end{algorithmic}
\end{algorithm}





% The gradients on parameters θl=(W,b)\theta_{l} = \left(W, b \right) is 
% \begin{equation*}
%     \nabla_{\theta} = \frac{\partial L}{\partial \theta} = \mathrm{vec}\left(h \delta^{\mathrm{T}}\right).  
% \end{equation*}
% The Kronecker factored approximation of corresponding $G^{l}$ is 
% \begin{align*}
% G^{l}  = & \mathbb{E} \left[ \nabla_{\theta} \nabla_{\theta}^{\mathrm{T}} \right]\\
% \approx &  \mathbb{E} \left[h h^{\mathrm{T}} \right] \otimes \mathbb{E} \left[ \delta \delta^{\mathrm{T}}\right]
% \end{align*}
% Plugging the notation for convolution layer, we have 
% \begin{equation*}
%     {G^{(l)}} \approx {A} \otimes {B} 
% \end{equation*}
% where
% \begin{align*}
% A=\mathbb{E}\left[\sum_{t, t^{\prime}\in\mathcal{T} } h^{t} h^{t^{\prime} \top}\right], B=\mathbb{E}\left[\sum_{t, t^{\prime}\in \mathcal{T}} \delta^{t} \delta^{t^{\prime} \top}\right] 
% \end{align*}
% and hth^{t} is flattened input subtensor (receptive field) at position tt, δt\delta^{t} is the gradient of LL w.r.t. output of filter at position tt.



% \begin{array}{l}  
 
% A=\mathbb{E}\left[\sum_{\left(s, s^{\prime}\right)} h^{s} h^{s^{\prime} \top}\right], B=\mathbb{E}\left[\sum_{\left(s, s^{\prime}\right)} \delta^{s} \delta^{s^{\prime} \top}\right] \\  
% \end{array}  
% $$  
% $s \in \mathcal{S}, s^{\prime} \in \mathcal{S}$ : spatial positions iterated over by the filter $h^{s}$ : flattened input subtensor (receptive field) at position $s$ $\delta^{s}$ : gradient of $\ell$ w.r.t. output of filter at position $s$

% $\underset{\left(n_{\text {in }} n_{\text {out }} k_{w} k_{h}\right)^{2}}$
% $\underset{\left(n_{\text {in }} k_{w} k_{h}\right)^{2}}$


% And this layer is parameterized by a set of weights $w_{i, j, \delta}$ and biases $b_{i}$, where $i \in\{1, \ldots, I\}$ indexes the output map, $j$ indexes the input map, and $\delta \in \Delta$ indexes the spatial offset (from the center of the filter). If the filters are of size $(2 R+1) \times(2 R+1)$, then we would have $\Delta=\{-R, \ldots, R\} \times\{-R, \ldots, R\}$. We denote the numbers of spatial locations and spatial offsets as $|\mathcal{T}|$ and $|\Delta|$, respectively. The convolution layer computes a set of pre-activations $\left\{s_{i, t}\right\}$ as follows:  




% To this end, consider the $l$-th layer of $\hat{g}$ which takes $\left\{a_{j, t}\right\}$ as input. And this layer is parameterized by a set of weights $w_{i, j, \delta}$ and biases $b_{i}$, where $i \in\{1, \ldots, I\}$ indexes the output map, $j$ indexes the input map, and $\delta \in \Delta$ indexes the spatial offset (from the center of the filter). If the filters are of size $(2 R+1) \times(2 R+1)$, then we would have $\Delta=\{-R, \ldots, R\} \times\{-R, \ldots, R\}$. We denote the numbers of spatial locations and spatial offsets as $|\mathcal{T}|$ and $|\Delta|$, respectively. The convolution layer computes a set of pre-activations $\left\{s_{i, t}\right\}$ as follows:  
% $$  
% s_{i, t}=\sum_{\delta \in \Delta} w_{i, j, \delta} a_{j, t+\delta}+b_{i},  
% $$  


% %----------------
% $$  
% \begin{array}{l}  
% \underset{\left(n_{\text {in }} n_{\text {out }} k_{w} k_{h}\right)^{2}}{G^{(l)}} \approx \underset{\left(n_{\text {in }} k_{w} k_{h}\right)^{2}}{A} \otimes \underset{\left(n_{\text {out }}\right)^{2}}{B} \\  
% A=\mathbb{E}\left[\sum_{\left(s, s^{\prime}\right)} h^{s} h^{s^{\prime} \top}\right], B=\mathbb{E}\left[\sum_{\left(s, s^{\prime}\right)} \delta^{s} \delta^{s^{\prime} \top}\right] \\  
% \end{array}  
% $$  
% $s \in \mathcal{S}, s^{\prime} \in \mathcal{S}$ : spatial positions iterated over by the filter $h^{s}$ : flattened input subtensor (receptive field) at position $s$ $\delta^{s}$ : gradient of $\ell$ w.r.t. output of filter at position $s$

% %----------------



% the parameters $\theta_{l}$ for $l$-th layer includes input, weights, bias and outputs are denoted a layer of activation $\left\{a_{j, t}\right\}$, where $j \in\{1, \ldots, J\}$ indexes the input map and $t \in \mathcal{T}$ indexes the spatial location which is typically a 2-D grid. Assume convolution is performed with a stride of 1 and padding equal to $R$, so that the set of spatial locations is shared between the input and output feature maps.


% where $b_{i}$ denotes the bias parameter. The activations are defined to take the value 0 outside of $\mathcal{T}$. The pre-activations are passed through a nonlinearity such as ReLU to compute the output layer activations, but we have no need to refer to this explicitly when analyzing a single layer. (For simplicity, we assume operations such as pooling and response normalization are implemented as separate layers.)  
  
% Pre-activation derivatives $\mathcal{D} s_{i, t}$ are computed during backpropagation. One then computes weight derivatives as:  
% \begin{equation}\label{con_layer}
%     \mathcal{D} w_{i, j, \delta}=\sum_{t \in \mathcal{T}} a_{j, t+\delta} \mathcal{D} s_{i, t}.
% \end{equation}






% \section{EK-FAC acceleration}
% Noting that all the theorems in our work requires computing an inverse-Hessian-vector product(IHVP), i.e., $H^{-1}v$ for some vector $v$. 
% This is a computational bottleneck for large models, since each dimension of this matrix, $H$, is equal to the number of model parameters phases. 
% In this section, we utilize Eigenvalue Kronecker-Factored Approximate Curvature(EK-FAC) method to the Fisher information matrix(FIM) to approximate IHVP.
% And the FIM is defined as follows:
% \begin{equation*}
%     F = \mathbb{E}_{x \sim p_{\text{data}}, y \sim P_{y \mid x}(\theta)} \left[ \nabla_{{\theta}} \log p (y \mid \theta, x) {\nabla_{{\theta}} \log p (y \mid \theta, x)}^{\mathrm{T}}\right].
% \end{equation*}
% where $p_{\text{data}}$ is the data distribution and $P_{y \mid x}(\theta)$ is the model's output distribution over $y$. And $y$ is sampled from the output distribution, we use the training labels instead yields the empirical Fisher matrix as an alternative.
% \subsection{EK-FAC for Convolution Layer}
% In our CBM model, the label predictor is a single linear layer and the cost for Hessian computing is affordable. However, the concept predictor is based on Resnet-18, which has much more parameters. Therefore, we perform a EK-FAC for $\hat{g}$.
% \begin{equation*}
%     \hat{g} = \argmin_g \sum_{j=1}^{k}  L_{C_j} = \argmin_g \sum_{j=1}^k\sum_{i=1}^n \ell(g^j(x_i),c_i^j),
% \end{equation*}
% we define $H_{\hat{g}} = \nabla^2_{\hat{g}}L_{C_j}$ as the Hessian matrix of the loss function with respect to the parameters. The Gauss-Newton Hessian (GNH),  serves as an estimate of $H$ that approximates the linearization of the parameter-output relationship of the network around its current parameters(\cite{martens2020new}), and is denoted as 
% \begin{equation*}
%     G=\mathbb{E}\left[J^{\top} H_{y} J\right]
% \end{equation*}
% where $J = \frac{\mathrm{d}y}{\mathrm{d}{\hat{g}}}$, $H_{y} = \nabla_{y}^2 L_{C_j}$ is the Hessian of the loss with respect to the network’s outputs, and the expectation is with respect to the empirical distribution.
% %index ref{martens2020new}

% \cite{martens2020new} shows that there is quite general equivalence between FIM and GNH, especially for several common loss functions like cross-entropy and squared error. Therefore, we can use FIM instead of GNH as an estimate of $H_{\hat{g}}$.

% % On the other hand, EK-FAC method provides a parameterized estimate of FIM for a neural network, facilitating efficient inversion. Although initially developed for optimization tasks with considerations like step size selection, our attention here is solely on the fundamental FIM approximation. 
% We provide the EK-FAC method for approximating the Hessian matrix for the concept predictor here.


% \subsection{Convolution layer}
% The block-diagonal version of K-FAC is based on two approximations to F which together make it tractable to invert. Firstly, it is assumed that the weight derivatives in various layers are independent, leading to the block diagonal structure of F, where each layer corresponds to a separate block:
% \begin{equation*}
%     F \approx\left(\begin{array}{ccc}E\left[\operatorname{vec}\left(\mathcal{D} \overline{W}_{1}\right) \operatorname{vec}\left(\mathcal{D} \overline{W}_{1}\right)^{\top}\right] & & \mathbf{0} \\ & \ddots & \\ \mathbf{0} & & \mathbb{E}\left[\operatorname{vec}\left(\mathcal{D} \overline{W}_{L}\right) \operatorname{vec}\left(\mathcal{D} \overline{W}_{L}\right)^{\top}\right]\end{array}\right)
% \end{equation*}
% This approximation alone is inadequate, as each of the blocks could still be significantly large. We perform the second approximation in the following part.

% Consider the ll-th layer of ˆg\hat{g} which takes as input 
% input, weights, bias and outputs are denoted a layer of activations $\left\{a_{j, t}\right\}$, where $j \in\{1, \ldots, J\}$ indexes the input map and $t \in \mathcal{T}$ indexes the spatial location which is typically a 2-D grid. Assume convolution is performed with a stride of 1 and padding equal to $R$, so that the set of spatial locations is shared between the input and output feature maps.
% This layer is parameterized by a set of weights $w_{i, j, \delta}$ and biases $b_{i}$, where $i \in\{1, \ldots, I\}$ indexes the output map, $j$ indexes the input map, and $\delta \in \Delta$ indexes the spatial offset (from the center of the filter). If the filters are of size $(2 R+1) \times(2 R+1)$, then we would have $\Delta=\{-R, \ldots, R\} \times\{-R, \ldots, R\}$. We denote the numbers of spatial locations and spatial offsets as $|\mathcal{T}|$ and $|\Delta|$, respectively. The convolution layer computes a set of pre-activations $\left\{s_{i, t}\right\}$ as follows:  
% $$  
% s_{i, t}=\sum_{\delta \in \Delta} w_{i, j, \delta} a_{j, t+\delta}+b_{i},  
% $$  
% where $b_{i}$ denotes the bias parameter. The activations are defined to take the value 0 outside of $\mathcal{T}$. The pre-activations are passed through a nonlinearity such as ReLU to compute the output layer activations, but we have no need to refer to this explicitly when analyzing a single layer. (For simplicity, we assume operations such as pooling and response normalization are implemented as separate layers.)  
  
% Pre-activation derivatives $\mathcal{D} s_{i, t}$ are computed during backpropagation. One then computes weight derivatives as:  
% \begin{equation}\label{con_layer}
%     \mathcal{D} w_{i, j, \delta}=\sum_{t \in \mathcal{T}} a_{j, t+\delta} \mathcal{D} s_{i, t}.
% \end{equation}

% \subsection{K-FAC for convolution layer}
% Recall the definition of FIM and plug equation \ref{con_layer} in, then we have
% \begin{equation*}
%     \mathbb{E}\left[\mathcal{D} w_{i, j, \delta} \mathcal{D} w_{i^{\prime}, j^{\prime}, \delta^{\prime}}\right]=\mathbb{E}\left[\left(\sum_{t \in \mathcal{T}} a_{j, t+\delta} \mathcal{D} s_{i, t}\right)\left(\sum_{t^{\prime} \in \mathcal{T}} a_{j^{\prime}, t^{\prime}+\delta^{\prime}} \mathcal{D} s_{i^{\prime}, t^{\prime}}\right)\right]
% \end{equation*}
% Before the approximation, we need to recall the following three assumptions proposed in \cite{grosse2016kronecker}:
% \begin{itemize}
% \item Independent activations and derivatives (IAD). The activations are independent of the pre-activation derivatives, i.e. $\left\{a_{j, t}\right\}\perp\left\{\mathcal{D} s_{i, t^{\prime}}\right\}$. 
% \item Spatial homogeneity (SH). The first-order statistics of the activations are independent of spatial location. The second-order statistics of the activations and pre-activation derivatives at any two spatial locations $t$ and $t^{\prime}$ depend only on $t^{\prime}-t$. This implies there are functions $M, \Omega$ and $\Gamma$ such that:  
% $$  
% \begin{aligned}  
% \mathbb{E}\left[a_{j, t}\right] & =M(j) \\  
% \mathbb{E}\left[a_{j, t} a_{j^{\prime}, t^{\prime}}\right] & =\Omega\left(j, j^{\prime}, t^{\prime}-t\right) \\  
% \mathbb{E}\left[\mathcal{D} s_{i, t} \mathcal{D} s_{i^{\prime}, t^{\prime}}\right] & =\Gamma\left(i, i^{\prime}, t^{\prime}-t\right) .  
% \end{aligned}  
% $$  
% Note that $\mathbb{E}\left[\mathcal{D} s_{i, t}\right]=0$ under the model's distribution, so 
% \begin{equation*}
% \operatorname{Cov}\left(\mathcal{D} s_{i, t}, \mathcal{D} s_{i^{\prime}, t^{\prime}}\right)=\mathbb{E}\left[\mathcal{D} s_{i, t} \mathcal{D} s_{i^{\prime}, t^{\prime}}\right].
% \end{equation*}
% \item Spatially uncorrelated derivatives (SUD). The pre-activation derivatives at any two distinct spatial locations are uncorrelated, i.e. $\Gamma\left(i, i^{\prime}, \delta\right)=0$ for $\delta \neq 0$.
% \end{itemize}
% Let $\hat{F_{\ell}} \approx \mathbb{E}\left[\operatorname{vec}\left(\mathcal{D} \overline{W}_{\ell}\right) \operatorname{vec}\left(\mathcal{D} \overline{W}_{\ell}\right)^{\top}\right]$ denote the block of the approximate Fisher for layer $\ell$. Because the data are two-dimensional, the offsets can be parameterized with indices $\delta=\left(\delta_{1}, \delta_{2}\right)$ and $\delta^{\prime}=\left(\delta_{1}^{\prime}, \delta_{2}^{\prime}\right)$, and denote the dimensions of the activations map as $\left(T_{1}, T_{2}\right)$. 
% Theorem 1 in \cite{grosse2016kronecker} yields our KFC factorization of $\hat{{F}}_{\ell}$ into a Kronecker product of smaller factors:
% \begin{equation*}
% \hat{F}_{\ell}={\Omega}_{\ell-1} \otimes {\Gamma}_{\ell}
% \end{equation*}
% where
% \begin{equation*}
%     \begin{aligned} 
% {\left[{\Omega}_{\ell-1}\right]_{j|\Delta|+\delta, j^{\prime}|\Delta|+\delta^{\prime}} } & \triangleq \beta\left(\delta, \delta^{\prime}\right) \Omega\left(j, j^{\prime}, \delta^{\prime}-\delta\right) \\ {\left[{\Omega}_{\ell-1}\right]_{j|\Delta|+\delta, 0}=\left[{\Omega}_{\ell-1}\right]_{0, j|\Delta|+\delta} } & \triangleq \beta(\delta) M(j) \\ {\left[{\Omega}_{\ell-1}\right]_{0,0} } & \triangleq|\mathcal{T}| \\ {\left[{\Gamma}_{\ell}\right]_{i, i^{\prime}} } & \triangleq \Gamma\left(i, i^{\prime}, 0\right) .
% \end{aligned}
% \end{equation*}
% and
% \begin{equation*}
% \begin{aligned} 
% \beta(\delta) & \triangleq\left(T_{1}-\left|\delta_{1}\right|\right)\left(T_{2}-\left|\delta_{2}\right|\right) \\
% \beta\left(\delta, \delta^{\prime}\right) & \triangleq\left(T_{1}-\max \left(\delta_{1}, \delta_{1}^{\prime}, 0\right)+\min \left(\delta_{1}, \delta_{1}^{\prime}, 0\right)\right) \cdot\left(T_{2}-\max \left(\delta_{2}, \delta_{2}^{\prime}, 0\right)+\min \left(\delta_{2}, \delta_{2}^{\prime}, 0\right)\right)
% \end{aligned}
% \end{equation*}
% Recall the Theorem 2 in \cite{grosse2016kronecker}, Under assumption SH, we estimate each $\Omega$ and $\Gamma$ directly by the following fact:
% \begin{equation}
%     \begin{aligned}  
% {\Omega}_{\ell} & =\mathbb{E}\left[ \llbracket {{A}}_{\ell} \rrbracket_{H}^{\mathrm{T}} \llbracket {{A}}_{\ell} \rrbracket_{H} \right] \\  
% {\Gamma}_{\ell} & =\frac{1}{|\mathcal{T}|} \mathbb{E}\left[\mathcal{D} {S}_{\ell}^{\top} \mathcal{D} {S}_{\ell}\right]  
% \end{aligned} 
% \end{equation}
% where  $\llbracket \tilde{\mathbf{A}}_{\ell} \rrbracket$ is the expanded activation as
% \begin{equation}\label{expand_op}
%     \llbracket \tilde{\mathbf{A}}_{\ell} \rrbracket_{t M+m, j|\Delta|+\delta}=[\tilde{\mathbf{A}}_{\ell}]_{(t+\delta) M+m, j}=a_{j, t+\delta}^{(m)},
% \end{equation}
% for all entries such that t+δ∈Tt+\delta \in \mathcal{T}. All other entries are defined to be 0 . Here, mm indexes the data instance within the mini-batch.

% The extension operators is an operator used to overcome the problem of poor convolutional memory localisation and thus efficiently implemented, denoted as \llbracket⋅\rrbracket\llbracket\cdot\rrbracket, which extracts patches around each spatial location and flattens them into vectors, and these vectors become the rows of a matrix. For instance, M×|T|×JM \times|\mathcal{T}| \times J array ˜Aℓ\tilde{{A}}_{\ell}, where MM is the mini-batch size, |T||\mathcal{T}| is the number of spatial locations, and JJ is the number of feature maps. Then, \llbracket˜Aℓ\rrbracket\llbracket \tilde{\mathbf{A}}_{\ell} \rrbracket is a M|T|×J|Δ|M |\mathcal{T}| \times J |\Delta| matrix, defined as equation ???\ref{expand_op}.

% Using this result, we define the empirical statistics for a given mini-batch:  
% $$  
% \begin{aligned}  
% \hat{{\Omega}}_{\ell-1} & =\frac{1}{M} \llbracket \tilde{{A}}_{\ell-1} \rrbracket_{H}^{\top} \llbracket \tilde{{A}}_{\ell-1} \rrbracket_{H} \\  
% \hat{{\Gamma}}_{\ell} & =\frac{1}{M|\mathcal{T}|} \mathcal{D} \tilde{{S}}_{\ell}^{\top} \mathcal{D} \tilde{{S}}_{\ell}  
% \end{aligned}  
% $$
% Since subsequent inverse operations are required and the current approximation for FIM or GNH  is PSD, we actually use a damped version for FIM as ˆF=F+γI\hat{F} = F + \gamma I, 

% \subsection{EK-FAC for convolution layer}
% In this part, for the sake of simplicity, we drop the layer subscript and aproxiamate hat.

% The K-FAC approximation also allows for efficient computation of eigendecomposition. In particular, eigendecomposition can be distributed across Kronecker products. That is, if ˆΩ\mathbf{\hat{\Omega}} and ˆΓ\mathbf{\hat{\Gamma}} have eigendecomposition 
% \mathbf{Q}_{\mathbf{\Omega}} \boldsymbol{\Lambda}_{\mathbf{\Omega}} \mathbf{Q}_{\mathbf{\Omega}}^{\top}\mathbf{Q}_{\mathbf{\Omega}} \boldsymbol{\Lambda}_{\mathbf{\Omega}} \mathbf{Q}_{\mathbf{\Omega}}^{\top}\mathbf{Q}_{\mathbf{\Omega}} \boldsymbol{\Lambda}_{\mathbf{\Omega}} \mathbf{Q}_{\mathbf{\Omega}}^{\top}\mathbf{Q}_{\mathbf{\Omega}} \boldsymbol{\Lambda}_{\mathbf{\Omega}} \mathbf{Q}_{\mathbf{\Omega}}^{\top} and \mathbf{Q}_{\mathbf{\Gamma}} \boldsymbol{\Lambda}_{\mathbf{\Gamma}} \mathbf{Q}_{\mathbf{\Gamma}}^{\top}\mathbf{Q}_{\mathbf{\Gamma}} \boldsymbol{\Lambda}_{\mathbf{\Gamma}} \mathbf{Q}_{\mathbf{\Gamma}}^{\top}\mathbf{Q}_{\mathbf{\Gamma}} \boldsymbol{\Lambda}_{\mathbf{\Gamma}} \mathbf{Q}_{\mathbf{\Gamma}}^{\top}\mathbf{Q}_{\mathbf{\Gamma}} \boldsymbol{\Lambda}_{\mathbf{\Gamma}} \mathbf{Q}_{\mathbf{\Gamma}}^{\top}, respectively, then the eigendecomposition of \mathbf{\Omega} \otimes \mathbf{\Gamma}\mathbf{\Omega} \otimes \mathbf{\Gamma} can be written as: 
% $$  
% \begin{aligned}  
% \mathbf{\Omega} \otimes \mathbf{\Gamma} & =\mathbf{Q}_{\mathbf{\Omega}} \boldsymbol{\Lambda}_{\mathbf{\Omega}} \mathbf{Q}_{\mathbf{\Omega}}^{\top} \otimes \mathbf{Q}_{\mathbf{\Gamma}} \boldsymbol{\Lambda}_{\mathbf{\Gamma}} \mathbf{Q}_{\mathbf{\Gamma}}^{\top} \\  
% & =\left(\mathbf{Q}_{\mathbf{\Omega}} \otimes \mathbf{Q}_{\mathbf{\Gamma}}\right)\left(\boldsymbol{\Lambda}_{\mathbf{\Omega}} \otimes \mathbf{\Lambda}_{\mathbf{\Gamma}}\right)\left(\mathbf{Q}_{\mathbf{\Omega}} \otimes \mathbf{Q}_{\mathbf{\Gamma}}\right)^{\top}  
% \end{aligned}  
% $$



% %_-------------

% 2.2.3 Eigenvalue-Corrected Kronecker-Factored Approximate Curvature  
  
% The K-FAC approximation admits not only efficient IHVP computation but also efficient eigendecomposition. Specifically, eigendecompositions distribute over Kronecker products, so if the factors A\mathbf{A} and S\mathbf{S} (we drop the layer subscripts to avoid clutter) have eigendecomposition \mathbf{Q}_{\mathbf{A}} \boldsymbol{\Lambda}_{\mathbf{A}} \mathbf{Q}_{\mathbf{A}}^{\top}\mathbf{Q}_{\mathbf{A}} \boldsymbol{\Lambda}_{\mathbf{A}} \mathbf{Q}_{\mathbf{A}}^{\top} and \mathbf{Q}_{\mathbf{S}} \boldsymbol{\Lambda}_{\mathbf{S}} \mathbf{Q}_{\mathbf{S}}^{\top}\mathbf{Q}_{\mathbf{S}} \boldsymbol{\Lambda}_{\mathbf{S}} \mathbf{Q}_{\mathbf{S}}^{\top}, respectively, then the eigendecomposition of \mathbf{A} \otimes \mathbf{S}\mathbf{A} \otimes \mathbf{S} can be written as:  
% $$  
% \begin{aligned}  
% \mathbf{A} \otimes \mathbf{S} & =\mathbf{Q}_{\mathbf{A}} \boldsymbol{\Lambda}_{\mathbf{A}} \mathbf{Q}_{\mathbf{A}}^{\top} \otimes \mathbf{Q}_{\mathbf{S}} \boldsymbol{\Lambda}_{\mathbf{S}} \mathbf{Q}_{\mathbf{S}}^{\top} \\  
% & =\left(\mathbf{Q}_{\mathbf{A}} \otimes \mathbf{Q}_{\mathbf{S}}\right)\left(\boldsymbol{\Lambda}_{\mathbf{A}} \otimes \mathbf{\Lambda}_{\mathbf{S}}\right)\left(\mathbf{Q}_{\mathbf{A}} \otimes \mathbf{Q}_{\mathbf{S}}\right)^{\top}  
% \end{aligned}  
% $$
  
% Observe that \boldsymbol{\Lambda}_{\mathbf{A}}\boldsymbol{\Lambda}_{\mathbf{A}} and \boldsymbol{\Lambda}_{\mathbf{S}}\boldsymbol{\Lambda}_{\mathbf{S}} are (M+1) \times(M+1)(M+1) \times(M+1) and P \times PP \times P diagonal matrices, and their Kronecker product is a (M+1) P \times(M+1) P(M+1) P \times(M+1) P diagonal matrix. Because this larger diagonal matrix \boldsymbol{\Lambda}_{\mathbf{A}} \otimes \boldsymbol{\Lambda}_{\mathbf{S}}\boldsymbol{\Lambda}_{\mathbf{A}} \otimes \boldsymbol{\Lambda}_{\mathbf{S}} has only (M+1) P(M+1) P entries, we can afford to fit and store the diagonal entries individually rather than assuming the Kronecker structure.  
  
% The Eigenvalue-corrected K-FAC (EK-FAC) (George et al., 2018) approximation does exactly this. After computing the eigendecomposition of the original Kronecker factors, it fits a more accurate GNH approximation such that:  
% $$  
% \mathbf{G} \approx\left(\mathbf{Q}_{\mathbf{A}} \otimes \mathbf{Q}_{\mathbf{s}}\right) \mathbf{\Lambda}\left(\mathbf{Q}_{\mathbf{A}} \otimes \mathbf{Q}_{\mathbf{s}}\right)^{\top}  
% $$  
% where \boldsymbol{\Lambda}\boldsymbol{\Lambda} is diagonal matrix of dimension (M+1) P(M+1) P defined as:  
% $$  
% \boldsymbol{\Lambda}_{i i}=\mathbb{E}\left[\left(\left(\mathbf{Q}_{\mathbf{A}} \otimes \mathbf{Q}_{\mathbf{S}}\right) \mathcal{D} \boldsymbol{\theta}\right)_{i}^{2}\right]  
% $$



==> section/rebuttal.tex <==
\section{Additional Experiment}

\subsection{Improvement via Harmful Data Removal}

We conducted addition experiments on CUB datasets with synthetically introduced noisy concepts or labels. Firstly, we introduce noises under three levels. In concept level, we choose 10\% of the concepts and flip these concept labels for a portion of the data. In data level, we choose 10\% of the data and flip their labels. In concept-label level, we choose 10\% of the total concepts and flip them. Then we conduct the following experiments.

We introduce noises into the three levels and train the model. After that, we remove the noise and obtain the retrained mdoel, which is the ground truth(gt) of this harmful data removal task. In contrast, we use ECBM to remove the harmful data. 
\begin{figure}[ht]
    \centering
    \begin{tabular}{c}
        \includegraphics[width=0.95\linewidth]{images/harmful_removal.png} 
    \end{tabular}
    \caption{Model performance after the removal of harmful data.}
    \label{hramful_removal}
\end{figure}

From figure \ref{hramful_removal}, it can be observed that the model performance improves across all three settings after noise removal and subsequent retraining or ECBM editing. This confirms that the performance of ECBM is nearly equivalent to retraining in various experimental scenarios, further providing evidence of the robustness of our method.


\noindent {\bf Model Unlearning.} 
Model unlearning has gained significant attention in recent years, with various methods~\citep{bourtoule2021machine,brophy2021machine,cao2015towards, chen2022recommendation,chen2022graph} proposed to efficiently remove the influence of certain data from trained machine learning models. Existing approaches can be broadly categorized into exact and approximate unlearning methods. Exact unlearning methods aim to replicate the results of retraining by selectively updating only a portion of the dataset, thereby avoiding the computational expense of retraining on the entire dataset~\citep{sekhari2021remember, chowdhury2024towards}. Approximate unlearning methods, on the other hand, seek to adjust model parameters to approximately satisfy the optimality condition of the objective function on the remaining data~\citep{golatkar2020eternal,guo2019certified,izzo2021approximate}. These methods are further divided into three subcategories: (1) Newton step-based updates that leverage Hessian-related terms [22, 26, 31, 34, 40, 43, 49], often incorporating Gaussian noise to mitigate residual data influence. To reduce computational costs, some works approximate the Hessian using the Fisher information matrix~\citep{golatkar2020eternal} or small Hessian blocks~\citep{mehta2022deep}. (2) Neural tangent kernel (NTK)-based unlearning approximates training as a linear process, either by treating it as a single linear change~\citep{golatkar2020forgetting}. (3) SGD path tracking methods, such as DeltaGrad~\citep{wu2020deltagrad} and unrollSGD~\citep{thudi2022unrolling}, reverse the optimization trajectory of stochastic gradient descent during training. 
Despite their advancements, these methods fail to handle the special architecture of CBMs. Moreover, given the high cost of obtaining data, we sometimes prefer to correct the data rather than remove it, which model unlearning is unable to achieve.

==> tabs/tab1.tex <==
\begin{table}[ht]
    \centering
    \caption{Performance comparison of different methods on the three datasets.}
    \label{tab:results}
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{llcccccc}
        \toprule
        \multirow{2}{*}{\textbf{Edit Level}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{OAI}} & \multicolumn{2}{c}{\textbf{CUB}} & \multicolumn{2}{c}{\textbf{CelebA}}\\
        \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8}
        & & \textbf{F1 score} & \textbf{RT (second)} & \textbf{F1 score} & \textbf{RT (second)} & \textbf{F1 score} & \textbf{RT (second)}\\
        \midrule
        \multirow{3}{*}{Concept Label} & Retrain & 0.8825$\pm$0.0054 & 31.44 & 0.7971$\pm$0.0066 & 27.88 & 0.3827$\pm$0.0272	& 57.60 \\
        & CBM-IF(Ours) & 0.8639$\pm$0.0033 & 16.31 & 0.7699$\pm$0.0035 & 14.39 & 0.3561$\pm$0.0134	& 34.93\\
        & ECBM(Ours) & \textbf{0.8808$\pm$0.0039} & \textbf{8.29} & \textbf{0.7963$\pm$0.0050} & \textbf{7.03} & \textbf{0.3845$\pm$0.0327} & \textbf{15.67}\\
        \midrule
        \multirow{3}{*}{Concept} & Retrain & 0.8448$\pm$0.0191 & 27.33 & 0.7811$\pm$0.0047 & 28.41 & 0.3776$\pm$0.0350 & 68.94\\
        & CBM-IF(Ours) & 0.8214$\pm$0.0071 & 17.38 & 0.7579$\pm$0.0065 & 15.70 & 0.3609$\pm$0.0202 & 35.56\\
        & ECBM(Ours) & \textbf{0.8403$\pm$0.0090} & \textbf{8.30} & \textbf{0.7787$\pm$0.0058} & \textbf{6.43} & \textbf{0.3761$\pm$0.0280} & \textbf{15.99} \\
        \midrule
        \multirow{3}{*}{Data} & Retrain & 0.8811$\pm$0.0065 & 33.72 & 0.7838$\pm$0.0051 & 28.08 & 0.3797$\pm$0.0375 & 65.60\\
        & CBM-IF(Ours) & 0.8472$\pm$0.0046 & 17.84 & 0.7623$\pm$0.0031 & 15.86 & 0.3536$\pm$0.0166 & 40.08 \\
        & ECBM(Ours) & \textbf{0.8797$\pm$0.0038} & \textbf{8.81} & \textbf{0.7827$\pm$0.0088} & \textbf{7.11} & \textbf{0.3748$\pm$0.0347} & \textbf{16.75} \\
        \bottomrule
    \end{tabular}}
\end{table}

==> tabs/tab_t.tex <==
\begin{table*}[ht]
    \centering
    \caption{Performance comparison of different methods on the three datasets.}
    \label{tab:results}
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{llcccccc}
        \toprule
        \multirow{2}{*}{\textbf{Edit Level}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{OAI}} & \multicolumn{2}{c}{\textbf{CUB}} & \multicolumn{2}{c}{\textbf{CelebA}}\\
        \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8}
        & & \textbf{F1 score} & \textbf{RT (second)} & \textbf{F1 score} & \textbf{RT (second)} & \textbf{F1 score} & \textbf{RT (second)}\\
        \midrule
        \multirow{3}{*}{Concept Label} & Retrain & 0.8825$\pm$0.0054 & 31.44 & 0.7971$\pm$0.0066 & 27.88 & 0.3827$\pm$0.0272	& 57.60 \\
        & CBM-IF(Ours) & 0.8639$\pm$0.0033 & 16.31 & 0.7699$\pm$0.0035 & 14.39 & 0.3561$\pm$0.0134	& 34.93\\
        & ECBM(Ours) & \textbf{0.8808$\pm$0.0039} & \textbf{8.29} & \textbf{0.7963$\pm$0.0050} & \textbf{7.03} & \textbf{0.3845$\pm$0.0327} & \textbf{15.67}\\
        \midrule
        \multirow{3}{*}{Concept} & Retrain & 0.8448$\pm$0.0191 & 27.33 & 0.7811$\pm$0.0047 & 28.41 & 0.3776$\pm$0.0350 & 68.94\\
        & CBM-IF(Ours) & 0.8214$\pm$0.0071 & 17.38 & 0.7579$\pm$0.0065 & 15.70 & 0.3609$\pm$0.0202 & 35.56\\
        & ECBM(Ours) & \textbf{0.8403$\pm$0.0090} & \textbf{8.30} & \textbf{0.7787$\pm$0.0058} & \textbf{6.43} & \textbf{0.3761$\pm$0.0280} & \textbf{15.99} \\
        \midrule
        \multirow{3}{*}{Data} & Retrain & 0.8811$\pm$0.0065 & 33.72 & 0.7838$\pm$0.0051 & 28.08 & 0.3797$\pm$0.0375 & 65.60\\
        & CBM-IF(Ours) & 0.8472$\pm$0.0046 & 17.84 & 0.7623$\pm$0.0031 & 15.86 & 0.3536$\pm$0.0166 & 40.08 \\
        & ECBM(Ours) & \textbf{0.8797$\pm$0.0038} & \textbf{8.81} & \textbf{0.7827$\pm$0.0088} & \textbf{7.11} & \textbf{0.3748$\pm$0.0347} & \textbf{16.75} \\
        \bottomrule
    \end{tabular}}
\end{table*}
